Reproducibility Issues for BERT-based Evaluation Metrics

Reproducibility is of utmost concern in machine learning and natural language processing (NLP). In the field of natural language generation (especially machine translation), the seminal paper of Post (2018) has pointed out problems of reproducibility of the dominant metric, BLEU, at the time of publication. Nowadays, BERT-based evaluation metrics considerably outperform BLEU. In this paper, we ask whether results and claims from four recent BERT-based metrics can be reproduced. We find that reproduction of claims and results often fails because of (i) heavy undocumented preprocessing involved in the metrics, (ii) missing code and (iii) reporting weaker results for the baseline metrics. (iv) In one case, the problem stems from correlating not to human scores but to a wrong column in the csv file, inflating scores by 5 points. Motivated by the impact of preprocessing, we then conduct a second study where we examine its effects more closely (for one of the metrics). We find that preprocessing can have large effects, especially for highly inflectional languages. In this case, the effect of preprocessing may be larger than the effect of the aggregation mechanism (e.g., greedy alignment vs. Word Mover Distance).

==> structure/figure.tex <==

\begin{figure}[h]
    \centering
    \includegraphics[width=0.85\textwidth]{figures/sum cv sw.png}
    \caption{\emph{Sensitivity to Stopwords}: Coefficients of variations of the correlations on TAC2008-2009.}
    \label{fig:sum cv sw}
\end{figure}



\begin{figure}[h]
    \centering
    \subfigure[MT: segment-level]{\includegraphics[height=0.4\textheight,width=0.27\textwidth]{figures/17-1-segment-pearson.png}}
    \subfigure[MT: system-level]{\includegraphics[height=0.4\textheight,width=0.27\textwidth]{figures/17-1-system-pearson.png}}
    \subfigure[Summrization]{\includegraphics[height=0.4\textheight,width=0.3\textwidth]{figures/2008-pearson.png}}
    
    
    \caption{\emph{Sensitivity to Stopwords}: (a) segment-level Pearson correlation of MoverScore-1 on WMT17; (b) system-level Pearson correlation of MoverScore-1 on WMT17; (C) summary-level Pearson correlation of MoverScore-1/2 on TAC2008.}
    \label{fig:example stopwords}
    
\end{figure}


\begin{figure}[h]

    \centering
    \includegraphics[width=0.8\textwidth]{figures/pie_sw.png}
    \caption{\emph{Sensitivity to Stopwords}: Distribution of the best stopword setting of each evaluation metric on each evaluation task. The rings from the inside to the outside represent MoverScore-1, MoverScore-2 and BERTScore-F1. For MT, I regard each language pair in WMT datasets as a test case for MT, resulting in 21 test cases (3 datasets times 7 language pairs). For summarization tasks, I regard each type of correlation as a test case for each criterion, resulting in 6 test cases (3 correlations times 2 datasets).}
    
    \label{fig:sw distribution}
\end{figure}

\begin{figure}[h]
    \centering
    \subfigure[Segment-level]{
    \includegraphics[width=\textwidth]{figures/rd_ori_dis_segment.png}
    }
    \subfigure[System-level]{
    \includegraphics[width=\textwidth]{figures/rd_ori_dis_system.png}
    }
    \caption{\emph{Sensitivity to IDF-weighting}: Relative differences of correlations from using original IDF-weighting to disabling IDF-weighting (RDs(dis-ori)) on WMT17-19. Negative values indicate original IDF-weighting works better.}
    \label{fig:rd dis ori wmt}
\end{figure}



\begin{figure}[hp]

    \includegraphics[width=\textwidth]{figures/rd idf sum.png}
    \caption{\emph{Sensitivity to IDF-weighting}: Relative differences of correlations from using original IDF-weighting to disabling IDF-weighting (RDs(dis-ori)) on TAC2008-2009. Negative values indicate original IDF-weighting works better.}
    \label{fig:rd idf sum}
\end{figure}



\begin{figure*}[hp]
%\addtocounter{subfigure}{-1}
\centering
\subfigure[MoverScore-1]{

\includegraphics[width=\textwidth]{figures/MoverScore-1segment_rd.png}

}
\subfigure[MoverScore-2]{

\includegraphics[width=\textwidth]{figures/MoverScore-2segment_rd.png}

}
\subfigure[BERTScore-F1]{

\includegraphics[width=\textwidth]{figures/BERTScore-F1segment_rd.png}

}
\caption{\emph{Sensitivity to IDF-weighting}: Left column: relative differences of segment-level correlations on WMT17-19 from using idf-ori to disabling IDF-weighting (RD(dis-ori)); negative values indicate idf-ori works better. Middle column: relative differences of segment-level correlations on WMT17-19 from using idf-random to disabling IDF-weighting (RD(random-dis); positive values indicate idf-random works better. Right column: relative differences of segment-level correlations on WMT17-19 from using idf-random to idf-ori (RD(random-ori)); negative values indicate idf-ori performs better.}
\label{fig:idf rd wmt seg}
\end{figure*}



\begin{figure}[H]
    \centering
    %\subfigure[MT]{\includegraphics[width=0.8\textwidth]{figures/punc keep.png}}
    %\subfigure[Summarization]{\includegraphics[width=0.75\textwidth]{figures/PUNC sum.png}}
    \includegraphics[width=0.9\textwidth]{figures/punc en.png}
    \caption{\emph{Sensitivity to Punctuation}: Relative differences of correlations of evaluation metrics from removing to keeping punctuations on WMT17-19 and TAC2008-2009 (RD(keep)). Positive values indicate positive impacts of punctuation removal.}
    \label{fig:punc rd wmt}
\end{figure}



\begin{figure}[H]
    \centering
    
    \includegraphics[width=0.9\textwidth]{figures/sub en.png}
    
    
    \caption{\emph{Sensitivity to Subword Selection}: Coefficients of variation of correlations of evaluation metrics using \emph{first}, \emph{all}, \emph{ave-all} subwords on WMT17-19 and TAC2008-2009.}
    
    \label{fig:sub rd wmt}
\end{figure}



\begin{figure}[hp]
    \centering
    \includegraphics[width=\textwidth]{figures/pie_sub_punc.png}
    \caption{\emph{Sensitivity to Subword Selection and Punctuation Removal}: Distribution of the best configuration of subword selection and punctuation removal for MoverScore-1 on machine translation (WMT17-19) and summarization (TAC2008-2009) evaluation tasks. I mark the default setting of MoverScore with $*$.}
    \label{fig:sub punc best}
\end{figure}


\begin{figure}[hp]
    \centering
    \subfigure[Segment-level]{\includegraphics[width=0.95\textwidth]{figures/comparison-segment.png}}
    \subfigure[System-level]{\includegraphics[width=0.95\textwidth]{figures/comparison-system.png}}
    \caption{\emph{Comparison among Evaluated Languages}: Average statistics over WMT17-19 datasets for MoverScore-1 and BERTScore-F1 in the evaluation of Czech, German, Finnish, Russian, Turkish, Chinese and English. CV-stopwords represents the coefficient of variation regarding different stopword settings. CV-idf represents the coefficient of variation regarding different IDF-weighting. RD-idf represents the relative performance change from using original IDF-weighting to disabling IDF-weighting; negative values indicate positive impact of original IDF-weighting. CV-subwords refers to the coefficient of variation regarding subword selection. RD-punctuation represents the relative performance change from removing to keeping punctuations; positive values indicate positive impact of punctuation removal.}
    
    \label{fig:all}
\end{figure}


\begin{figure}[h]
    \centering
    \subfigure[WMT18]{
    \includegraphics[width=0.3\textwidth]{figures/noisy18.jpg}
    }
    \subfigure[WMT19]{
    \includegraphics[width=0.3\textwidth]{figures/noisy19.jpg}
    }
    
    \caption{\emph{Noisy Alignment Rermoval}: Segment-level Kendall's $\tau$ of MoverScore-1 on WMT18-19. Dropout rate 0 denotes disabling noisy alignment removal. The best result for each language pair is marked with black triangle. The best results that are not obtained from noisy alignment removal are marked with red boxes.}
    \label{fig:noisy 18 19}
\end{figure}


\begin{figure*}[h]

\centering
\includegraphics[width=\textwidth]{figures/idf rd seg all.png}

\caption{\emph{Comparison among Evaluated Languages}: Relative change of segment-level correlations of MoverScore-1 on WMT17-19 from using original IDF-weighting to disabling IDF-weighting in the evaluation for tested languages. Negative values indicate positive impact of original IDF-weighting. 
The maximum, minimum, mean RDs in English evaluation are marked with red lines.}

\label{fig:idf rd all languages}
\end{figure*}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\textwidth]{figures/pun seg all.png}
    
    \caption{\emph{Comparison among Evaluated Languages}: Relative change of segment-level correlations of MoverScore-1 on WMT17-19 from removing to keeping punctuations in the evaluation for tested languages. The maximum, minimum, mean values in English evaluation are marked with red lines.}
    \label{fig:punc sub all}
\end{figure}

==> structure/full_tables.tex <==
%\clearpage
\subsection{Stopwords tables}\label{sec:stop}


\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccc|cccccc@{}}
\toprule
\multirow{3}{*}{metric} & \multicolumn{6}{c|}{TAC2008} & \multicolumn{6}{c}{TAC2009} \\
 & \multicolumn{3}{c}{pyramid} & \multicolumn{3}{c|}{responsiveness} & \multicolumn{3}{c}{pyramid} & \multicolumn{3}{c}{responsiveness} \\
 & Peason & Spearman & Kendall & Peason & Spearman & Kendall & Peason & Spearman & Kendall & Peason & Spearman & Kendall \\ \midrule
Mover-1 & 0.7581 & 0.6709 & 0.5167 & \textbf{0.7369} & \textbf{0.6071} & \textbf{0.5000} & 0.8296 & 0.6996 & 0.5448 & \textbf{0.7542} & 0.5908 & 0.4807 \\
Mover-1+153 & \textbf{0.7602} & \textbf{0.6721} & \textbf{0.5187} & 0.7363 & 0.6040 & 0.4972 & \textbf{0.8305} & \textbf{0.6998} & \textbf{0.5504} & 0.7538 & \textbf{0.5926} & \textbf{0.4820} \\
Mover-1+179 & \textbf{0.7602} & \textbf{0.6721} & \textbf{0.5187} & 0.7363 & 0.6040 & 0.4972 & \textbf{0.8305} & \textbf{0.6998} & \textbf{0.5504} & 0.7538 & \textbf{0.5926} & \textbf{0.4820} \\
Mover-1+326 & 0.7590 & 0.6682 & 0.5154 & 0.7353 & 0.6018 & 0.4955 & 0.8296 & 0.6976 & 0.5482 & 0.7539 & 0.5909 & 0.4806 \\ \midrule
\multicolumn{1}{c}{range} & 0.0021 & 0.0040 & 0.0034 & 0.0016 & 0.0053 & 0.0045 & 0.0009 & 0.0022 & 0.0055 & 0.0004 & 0.0018 & 0.0014 \\
\multicolumn{1}{c}{CV} & 0.13\% & 0.28\% & 0.32\% & 0.09\% & 0.36\% & 0.38\% & 0.06\% & 0.15\% & 0.48\% & 0.03\% & 0.17\% & 0.16\% \\ \midrule
Mover-2 & \textbf{0.7521} & \textbf{0.6623} & \textbf{0.5100} & \textbf{0.7338} & \textbf{0.6002} & \textbf{0.4939} & \textbf{0.8246} & \textbf{0.6934} & \textbf{0.5448} & \textbf{0.5855} & 0.7530 & \textbf{0.4754} \\
Mover-2 +153 & 0.7463 & 0.6503 & 0.4983 & 0.7300 & 0.5873 & 0.4824 & 0.8190 & 0.6811 & 0.5340 & 0.5794 & \textbf{0.7530} & 0.4703 \\
Mover-2 +179 & 0.7463 & 0.6503 & 0.4983 & 0.7300 & 0.5873 & 0.4824 & 0.8191 & 0.6811 & 0.5340 & 0.5790 & \textbf{0.7530} & 0.4703 \\
Mover-2 +326 & 0.7448 & 0.6452 & 0.4930 & 0.7286 & 0.5846 & 0.4797 & 0.8172 & 0.6771 & 0.5303 & 0.5772 & 0.7528 & 0.4678 \\ \midrule
\multicolumn{1}{c}{range} & 0.0073 & 0.0172 & 0.0171 & 0.0052 & 0.0156 & 0.0143 & 0.0075 & 0.0163 & 0.0145 & 0.0083 & 0.0002 & 0.0076 \\
\multicolumn{1}{c}{CV} & 0.43\% & 1.11\% & 1.44\% & 0.31\% & 1.19\% & 1.31\% & 0.39\% & 1.04\% & 1.17\% & 0.62\% & 0.01\% & 0.68\% \\ \midrule
BERT-F1 & \textbf{0.7502} & \textbf{0.6498} & \textbf{0.4977} & \textbf{0.5966} & \textbf{0.7249} & \textbf{0.4905} & \textbf{0.8378} & \textbf{0.7208} & \textbf{0.5701} & \textbf{0.7488} & \textbf{0.6014} & \textbf{0.4891} \\
BERT-F1+153 & 0.6913 & 0.5478 & 0.4107 & 0.5086 & 0.6824 & 0.4127 & 0.7754 & 0.6113 & 0.4676 & 0.7206 & 0.5398 & 0.4314 \\
BERT-F1+179 & 0.6913 & 0.5478 & 0.4107 & 0.5086 & 0.6824 & 0.4127 & 0.7754 & 0.6113 & 0.4676 & 0.7206 & 0.5398 & 0.4314 \\
BERT-F1+326 & 0.6864 & 0.5379 & 0.4015 & 0.5037 & 0.6785 & 0.4074 & 0.7687 & 0.6010 & 0.4594 & 0.7157 & 0.5314 & 0.4247 \\ \midrule
\multicolumn{1}{c}{range} & 0.0639 & 0.1119 & 0.0961 & 0.0929 & 0.0464 & 0.0831 & 0.0691 & 0.1198 & 0.1107 & 0.0330 & 0.0700 & 0.0644 \\
\multicolumn{1}{c}{CV} & 4.31\% & 9.26\% & 10.51\% & 8.48\% & 3.18\% & 9.25\% & 4.11\% & 8.91\% & 10.74\% & 2.07\% & 5.86\% & 6.78\% \\ \bottomrule
\end{tabular}%
}
\caption{Correlations with summary-level human judgements on TAC2008-2009 for stopwords tests.}
\label{tab:stopwords tac}
\end{table*}


\begin{table*}[htbp]
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccc}
\hline
\multicolumn{9}{c}{segment-level}                                                                                                                                         \\
metric                    & cs-en           & de-en           & fi-en           & lv-en           & ru-en           & tr-en           & zh-en           & average         \\ \hline
Mover-1                   & \textbf{0.6698} & \textbf{0.7083} & \textbf{0.8214} & \textbf{0.7174} & \textbf{0.7379} & \textbf{0.7618} & \textbf{0.7442} & \textbf{0.7373} \\
Mover-1+153               & 0.6615          & 0.6818          & 0.7817          & 0.7056          & 0.7071          & 0.7293          & 0.7301          & 0.7139          \\
Mover-1+179               & 0.6615          & 0.6818          & 0.7817          & 0.7056          & 0.7071          & 0.7293          & 0.7301          & 0.7139          \\
Mover-1+326               & 0.6385          & 0.6595          & 0.7710          & 0.6967          & 0.6969          & 0.7133          & 0.7294          & 0.7008          \\ \hline
\multicolumn{1}{c}{range} & 0.0313          & 0.0487          & 0.0505          & 0.0207          & 0.0409          & 0.0486          & 0.0148          & 0.0365          \\
\multicolumn{1}{c}{CV}    & 2.04\%          & 2.92\%          & 2.82\%          & 1.20\%          & 2.49\%          & 2.78\%          & 0.98\%          & 2.18\%          \\ \hline
Mover-2                   & \textbf{0.6786} & \textbf{0.7092} & \textbf{0.8145} & \textbf{0.7157} & \textbf{0.7357} & \textbf{0.7622} & \textbf{0.7380} & \textbf{0.7363} \\
Mover-2 +153              & 0.6605          & 0.6775          & 0.7766          & 0.7095          & 0.7065          & 0.7342          & 0.7318          & 0.7138          \\
Mover-2 +179              & 0.6605          & 0.6775          & 0.7766          & 0.7095          & 0.7065          & 0.7342          & 0.7318          & 0.7138          \\
Mover-2 +326              & 0.6375          & 0.6536          & 0.7672          & 0.7046          & 0.6943          & 0.7174          & 0.7317          & 0.7009          \\ \hline
\multicolumn{1}{c}{range} & 0.0411          & 0.0555          & 0.0473          & 0.0111          & 0.0414          & 0.0448          & 0.0064          & 0.0354          \\
\multicolumn{1}{c}{CV}    & 2.55\%          & 3.35\%          & 2.68\%          & 0.64\%          & 2.48\%          & 2.52\%          & 0.43\%          & 2.09\%          \\ \hline
BERT-F1                   & \textbf{0.6553} & \textbf{0.6816} & \textbf{0.8230} & \textbf{0.7127} & \textbf{0.7254} & \textbf{0.7180} & \textbf{0.7121} & \textbf{0.7183} \\
BERT-F1+153               & 0.5790          & 0.5662          & 0.7294          & 0.6142          & 0.6124          & 0.6001          & 0.6216          & 0.6175          \\
BERT-F1+179               & 0.5790          & 0.5662          & 0.7294          & 0.6142          & 0.6124          & 0.6001          & 0.6216          & 0.6175          \\
BERT-F1+326               & 0.5676          & 0.5274          & 0.6929          & 0.6043          & 0.6034          & 0.5719          & 0.5973          & 0.5950          \\ \hline
\multicolumn{1}{c}{range} & 0.0877          & 0.1542          & 0.1301          & 0.1084          & 0.1220          & 0.1460          & 0.1148          & 0.1233          \\
\multicolumn{1}{c}{CV}    & 6.79\%          & 11.40\%         & 7.48\%          & 8.03\%          & 9.11\%          & 10.44\%         & 7.93\%          & 8.74\%          \\ \hline
\multicolumn{9}{c}{system-level}                                                                                                                                          \\
metric                    & cs-en           & de-en           & fi-en           & lv-en           & ru-en           & tr-en           & zh-en           & average         \\ \hline
Mover-1                   & 0.9989          & \textbf{0.9794} & \textbf{0.9731} & 0.9712          & 0.9737          & \textbf{0.9912} & \textbf{0.9510} & \textbf{0.9769} \\
Mover-1+153               & 0.9967          & 0.9720          & 0.9671          & \textbf{0.9626} & \textbf{0.9754} & 0.9795          & 0.9386          & 0.9703          \\
Mover-1+179               & 0.9967          & 0.9720          & 0.9671          & \textbf{0.9626} & \textbf{0.9754} & 0.9795          & 0.9386          & 0.9703          \\
Mover-1+326               & \textbf{0.9992} & 0.9656          & 0.9631          & 0.9619          & 0.9729          & 0.9771          & 0.9364          & 0.9680          \\ \hline
\multicolumn{1}{c}{range} & 0.0024          & 0.0138          & 0.0099          & 0.0093          & 0.0025          & 0.0141          & 0.0146          & 0.0089          \\
\multicolumn{1}{c}{CV}    & 0.13\%          & 0.58\%          & 0.42\%          & 0.46\%          & 0.13\%          & 0.64\%          & 0.71\%          & 0.44\%          \\ \hline
Mover-2                   & 0.9994          & \textbf{0.9812} & \textbf{0.9762} & \textbf{0.9724} & 0.9715          & 0.9954          & \textbf{0.9558} & \textbf{0.9789} \\
Mover-2 +153              & 0.9984          & 0.9789          & 0.9734          & 0.9706          & \textbf{0.9739} & \textbf{0.9956} & 0.9548          & 0.9780          \\
Mover-2 +179              & 0.9984          & 0.9789          & 0.9734          & 0.9706          & \textbf{0.9739} & \textbf{0.9956} & 0.9548          & 0.9780          \\
Mover-2 +326              & \textbf{0.9998} & 0.9744          & 0.9707          & 0.9702          & 0.9717          & 0.9945          & 0.9533          & 0.9764          \\ \hline
\multicolumn{1}{c}{range} & 0.0014          & 0.0068          & 0.0055          & 0.0022          & 0.0024          & 0.0010          & 0.0026          & 0.0025          \\
\multicolumn{1}{c}{CV}    & 0.07\%          & 0.29\%          & 0.23\%          & 0.10\%          & 0.14\%          & 0.05\%          & 0.11\%          & 0.14\%          \\ \hline
BERT-F1                   & 0.9915          & 0.9674          & 0.9946          & \textbf{0.9914} & 0.9595          & \textbf{0.9958} & 0.9528          & 0.9790          \\
BERT-F1+153               & \textbf{0.9980} & 0.9695          & \textbf{0.9974} & 0.9893          & 0.9620          & 0.9947          & 0.9564          & 0.9810          \\
BERT-F1+179               & \textbf{0.9980} & 0.9695          & \textbf{0.9974} & 0.9893          & 0.9620          & 0.9947          & 0.9564          & 0.9810          \\
BERT-F1+326               & 0.9968          & \textbf{0.9708} & 0.9966          & 0.9890          & \textbf{0.9620} & 0.9942          & \textbf{0.9582} & \textbf{0.9811} \\ \hline
\multicolumn{1}{c}{range} & 0.0064          & 0.0034          & 0.0029          & 0.0025          & 0.0026          & 0.0016          & 0.0055          & 0.0021          \\
\multicolumn{1}{c}{CV}    & 0.31\%          & 0.14\%          & 0.14\%          & 0.11\%          & 0.13\%          & 0.07\%          & 0.24\%          & 0.16\%          \\ \hline
\end{tabular}%
}
\caption{Segment-level Pearson's $r$ and system-level Pearson's $r$ on WMT17 for stopwords tests. Bold values indicate the best performances.}
\label{tab:wmt17 stopwords}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccc}
\hline
\multicolumn{9}{c}{segment-level}                                                                                                                                         \\
metric                    & cs-en           & de-en           & et-en           & fi-en           & ru-en           & tr-en           & zh-en           & average         \\ \hline
Mover-1                   & \textbf{0.3726} & \textbf{0.5414} & \textbf{0.3944} & \textbf{0.2917} & \textbf{0.3414} & 0.2847          & \textbf{0.2591} & \textbf{0.3550} \\
Mover-1+153               & 0.3550          & 0.5328          & 0.3890          & 0.2805          & 0.3272          & \textbf{0.2856} & 0.2492          & 0.3456          \\
Mover-1+179               & 0.3550          & 0.5328          & 0.3890          & 0.2805          & 0.3272          & \textbf{0.2856} & 0.2492          & 0.3456          \\
Mover-1+326               & 0.3460          & 0.5227          & 0.3817          & 0.2767          & 0.3270          & 0.2755          & 0.2498          & 0.3399          \\ \hline
\multicolumn{1}{c}{range} & 0.0266          & 0.0187          & 0.0127          & 0.0150          & 0.0144          & 0.0101          & 0.0100          & 0.0151          \\
\multicolumn{1}{c}{CV}    & 3.12\%          & 1.44\%          & 1.34\%          & 2.29\%          & 2.16\%          & 1.73\%          & 1.94\%          & 2.00\%          \\ \hline
Mover-2                   & \textbf{0.3738} & \textbf{0.5416} & \textbf{0.3911} & \textbf{0.2891} & \textbf{0.3351} & \textbf{0.2957} & \textbf{0.2543} & \textbf{0.3544} \\
Mover-2 +153              & 0.3597          & 0.5334          & 0.3851          & 0.2731          & 0.3243          & 0.2823          & 0.2489          & 0.3438          \\
Mover-2 +179              & 0.3597          & 0.5334          & 0.3851          & 0.2731          & 0.3243          & 0.2823          & 0.2489          & 0.3438          \\
Mover-2 +326              & 0.3476          & 0.5236          & 0.3801          & 0.2705          & 0.3237          & 0.2758          & 0.2495          & 0.3387          \\ \hline
\multicolumn{1}{c}{range} & 0.0262          & 0.0179          & 0.0109          & 0.0187          & 0.0113          & 0.0199          & 0.0055          & 0.0157          \\
\multicolumn{1}{c}{CV}    & 2.98\%          & 1.38\%          & 1.16\%          & 3.09\%          & 1.68\%          & 2.95\%          & 1.05\%          & 2.04\%          \\ \hline
BERT-F1                   & \textbf{0.3714} & \textbf{0.5372} & 0.3920 & \textbf{0.2958} & \textbf{0.3414} & \textbf{0.2884} & \textbf{0.2450} & \textbf{0.3530} \\
BERT-F1+153               & 0.3182          & 0.4872          & 0.3422          & 0.2372          & 0.3058          & 0.2319          & 0.2125          & 0.3050          \\
BERT-F1+179               & 0.3182          & 0.4872          & 0.3422          & 0.2372          & 0.3058          & 0.2319          & 0.2125          & 0.3050          \\
BERT-F1+326               & 0.3112          & 0.4822          & 0.3400          & 0.2299          & 0.2960          & 0.2408          & 0.2225          & 0.3032          \\ \hline
\multicolumn{1}{c}{range} & 0.0603          & 0.0551          & 0.0521          & 0.0658          & 0.0454          & 0.0565          & 0.0325          & 0.0498          \\
\multicolumn{1}{c}{CV}    & 8.49\%          & 5.21\%          & 7.15\%          & 12.27\%         & 6.39\%          & 10.92\%         & 6.87\%          & 8.18\%          \\ \hline
\multicolumn{9}{c}{system-level}                                                                                                                                          \\
metric                    & cs-en           & de-en           & et-en           & fi-en           & ru-en           & tr-en           & zh-en           & average         \\ \hline
Mover-1                   & \textbf{0.9889} & \textbf{0.9959} & \textbf{0.9846} & \textbf{0.9938} & 0.9926          & 0.9823          & \textbf{0.9861} & \textbf{0.9892} \\
Mover-1+153               & 0.9798          & 0.9941          & 0.9826          & 0.9914          & \textbf{0.9933} & 0.9895          & 0.9846          & 0.9879          \\
Mover-1+179               & 0.9798          & 0.9941          & 0.9826          & 0.9914          & \textbf{0.9933} & 0.9895          & 0.9846          & 0.9879          \\
Mover-1+326               & 0.9880          & 0.9934          & 0.9824          & 0.9898          & 0.9922          & \textbf{0.9900} & 0.9841          & 0.9885          \\ \hline
\multicolumn{1}{c}{range} & 0.0091          & 0.0025          & 0.0022          & 0.0040          & 0.0011          & 0.0077          & 0.0020          & 0.0013          \\
\multicolumn{1}{c}{CV}    & 0.51\%          & 0.11\%          & 0.11\%          & 0.17\%          & 0.06\%          & 0.37\%          & 0.09\%          & 0.20\%          \\ \hline
Mover-2                   & 0.9888          & \textbf{0.9962} & \textbf{0.9852} & \textbf{0.9931} & 0.9914          & 0.9798          & 0.9869          & 0.9888          \\
Mover-2 +153              & 0.9836          & 0.9956          & 0.9837          & 0.9929          & \textbf{0.9925} & 0.9896          & \textbf{0.9871} & 0.9893          \\
Mover-2 +179              & 0.9836          & 0.9956          & 0.9837          & 0.9929          & \textbf{0.9925} & 0.9896          & \textbf{0.9871} & 0.9893          \\
Mover-2 +326              & \textbf{0.9893} & 0.9951          & 0.9834          & 0.9918          & 0.9912          & \textbf{0.9916} & 0.9868          & \textbf{0.9899} \\ \hline
\multicolumn{1}{c}{range} & 0.0057          & 0.0012          & 0.0018          & 0.0012          & 0.0013          & 0.0117          & 0.0003          & 0.0011          \\
\multicolumn{1}{c}{CV}    & 0.32\%          & 0.05\%          & 0.08\%          & 0.06\%          & 0.07\%          & 0.54\%          & 0.01\%          & 0.16\%          \\ \hline
BERT-F1                   & 0.9809          & 0.9953          & 0.9832          & \textbf{0.9947} & 0.9881          & 0.9936          & 0.9814          & \textbf{0.9882} \\
BERT-F1+153               & 0.9858          & \textbf{0.9959} & 0.9872          & 0.9914          & 0.9904          & 0.9580          & \textbf{0.9821} & 0.9844          \\
BERT-F1+179               & 0.9858          & \textbf{0.9959} & 0.9872          & 0.9914          & 0.9904          & 0.9580          & \textbf{0.9821} & 0.9844          \\
BERT-F1+326               & \textbf{0.9881} & 0.9957          & \textbf{0.9872} & 0.9910          & \textbf{0.9908} & \textbf{0.9354} & 0.9818          & 0.9815          \\ \hline
\multicolumn{1}{c}{range} & 0.0072          & 0.0006          & 0.0040          & 0.0036          & 0.0027          & 0.0581          & 0.0006          & 0.0067          \\
\multicolumn{1}{c}{CV}    & 0.31\%          & 0.03\%          & 0.20\%          & 0.17\%          & 0.12\%          & 2.50\%          & 0.03\%          & 0.48\%          \\ \hline
\end{tabular}%
}
\caption{Segment-level Kendall's $\tau$ and system-level Pearson's $r$ on WMT18 for stopwords tests. Bold values indicate the best performances.}
\label{tab:wmt18 stopwords}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccc}
\hline
\multicolumn{9}{c}{segment-level}                                                                                                                                         \\
metric                    & de-en           & fi-en           & gu-en           & kk-en           & lt-en           & ru-en           & zh-en           & average         \\ \hline
Mover-1                   & \textbf{0.2224} & \textbf{0.3436} & \textbf{0.3105} & \textbf{0.4479} & \textbf{0.3682} & \textbf{0.2183} & \textbf{0.4223} & \textbf{0.3333} \\
Mover-1+153               & 0.2126          & 0.3358          & 0.3072          & 0.4419          & 0.3641          & 0.2119          & 0.4201          & 0.3277          \\
Mover-1+179               & 0.2126          & 0.3358          & 0.3072          & 0.4419          & 0.3641          & 0.2119          & 0.4201          & 0.3277          \\
Mover-1+326               & 0.2071          & 0.3346          & 0.3031          & 0.4357          & 0.3571          & 0.2075          & 0.4202          & 0.3236          \\ \hline
\multicolumn{1}{c}{range} & 0.0153          & 0.0090          & 0.0074          & 0.0122          & 0.0111          & 0.0108          & 0.0023          & 0.0097          \\
\multicolumn{1}{c}{CV}    & 2.98\%          & 1.22\%          & 0.98\%          & 1.13\%          & 1.26\%          & 2.10\%          & 0.26\%          & 1.42\%          \\ \hline
Mover-2                   & \textbf{0.2200} & \textbf{0.3427} & \textbf{0.3095} & \textbf{0.4450} & \textbf{0.3682} & \textbf{0.2231} & \textbf{0.4242} & \textbf{0.3333} \\
Mover-2 +153              & 0.2071          & 0.3327          & 0.3053          & 0.4391          & 0.3593          & 0.2092          & 0.4176          & 0.3243          \\
Mover-2 +179              & 0.2071          & 0.3327          & 0.3053          & 0.4391          & 0.3593          & 0.2092          & 0.4176          & 0.3243          \\
Mover-2 +326              & 0.2009          & 0.3293          & 0.3013          & 0.4334          & 0.3544          & 0.2048          & 0.4169          & 0.3201          \\ \hline
\multicolumn{1}{c}{range} & 0.0191          & 0.0134          & 0.0083          & 0.0117          & 0.0138          & 0.0183          & 0.0073          & 0.0131          \\
\multicolumn{1}{c}{CV}    & 3.85\%          & 1.74\%          & 1.11\%          & 1.08\%          & 1.60\%          & 3.76\%          & 0.82\%          & 1.99\%          \\ \hline
BERT-F1                   & \textbf{0.1524} & \textbf{0.3365} & \textbf{0.2997} & \textbf{0.4454} & \textbf{0.3715} & \textbf{0.2055} & \textbf{0.4051} & \textbf{0.3166} \\
BERT-F1+153               & 0.1234          & 0.3002          & 0.2788          & 0.4198          & 0.3290          & 0.1835          & 0.3651          & 0.2857          \\
BERT-F1+179               & 0.1234          & 0.3002          & 0.2788          & 0.4198          & 0.3290          & 0.1835          & 0.3651          & 0.2857          \\
BERT-F1+326               & 0.1253          & 0.2916          & 0.2706          & 0.4104          & 0.3226          & 0.1833          & 0.3564          & 0.2800          \\ \hline
\multicolumn{1}{c}{range} & 0.0290          & 0.0449          & 0.0291          & 0.0350          & 0.0489          & 0.0222          & 0.0487          & 0.0366          \\
\multicolumn{1}{c}{CV}    & 10.85\%         & 6.51\%          & 4.41\%          & 3.55\%          & 6.67\%          & 5.83\%          & 5.85\%          & 6.24\%          \\ \hline
\multicolumn{9}{c}{system-level}                                                                                                                                          \\
metric                    & de-en           & fi-en           & gu-en           & kk-en           & lt-en           & ru-en           & zh-en           & average         \\ \hline
Mover-1                   & 0.9247          & 0.9940          & 0.9132          & \textbf{0.9839} & \textbf{0.9634} & 0.9771          & 0.9686          & 0.9607          \\
Mover-1+153               & \textbf{0.9260} & 0.9958          & 0.9201          & 0.9821          & 0.9616          & 0.9780          & 0.9697          & 0.9619          \\
Mover-1+179               & \textbf{0.9260} & 0.9958          & 0.9201          & 0.9821          & 0.9616          & 0.9780          & 0.9697          & 0.9619          \\
Mover-1+326               & 0.9241          & \textbf{0.9962} & \textbf{0.9238} & 0.9828          & 0.9612          & \textbf{0.9781} & \textbf{0.9698} & \textbf{0.9623} \\ \hline
\multicolumn{1}{c}{range} & 0.0019          & 0.0023          & 0.0107          & 0.0018          & 0.0022          & 0.0010          & 0.0013          & 0.0016          \\
\multicolumn{1}{c}{CV}    & 0.09\%          & 0.09\%          & 0.42\%          & 0.07\%          & 0.09\%          & 0.04\%          & 0.05\%          & 0.12\%          \\ \hline
Mover-2                   & \textbf{0.9242} & 0.9942          & 0.9137          & 0.9847          & \textbf{0.9631} & \textbf{0.9753} & 0.9661          & 0.9602          \\
Mover-2 +153              & 0.9227          & 0.9956          & 0.9271          & 0.9871          & 0.9577          & 0.9730          & 0.9659          & 0.9613          \\
Mover-2 +179              & 0.9227          & 0.9956          & 0.9271          & 0.9871          & 0.9577          & 0.9730          & 0.9659          & 0.9613          \\
Mover-2 +326              & 0.9208          & \textbf{0.9962} & \textbf{0.9319} & \textbf{0.9875} & 0.9575          & 0.9732          & \textbf{0.9663} & \textbf{0.9619} \\ \hline
\multicolumn{1}{c}{range} & 0.0034          & 0.0020          & 0.0183          & 0.0027          & 0.0056          & 0.0023          & 0.0003          & 0.0017          \\
\multicolumn{1}{c}{CV}    & 0.13\%          & 0.07\%          & 0.74\%          & 0.11\%          & 0.25\%          & 0.10\%          & 0.01\%          & 0.20\%          \\ \hline
BERT-F1                   & \textbf{0.9272} & 0.9871          & 0.9305          & 0.9973          & 0.9695          & \textbf{0.9771} & \textbf{0.9633} & \textbf{0.9646} \\
BERT-F1+153               & 0.9263          & \textbf{0.9920} & 0.9387          & 0.9964          & 0.9707          & 0.9765          & 0.9446          & 0.9636          \\
BERT-F1+179               & 0.9263          & \textbf{0.9920} & 0.9387          & 0.9964          & 0.9707          & 0.9765          & 0.9446          & 0.9636          \\
BERT-F1+326               & 0.9238          & 0.9917          & \textbf{0.9399} & \textbf{0.9966} & \textbf{0.9711} & 0.9756          & 0.9453          & 0.9634          \\ \hline
\multicolumn{1}{c}{range} & 0.0033          & 0.0049          & 0.0094          & 0.0008          & 0.0016          & 0.0015          & 0.0188          & 0.0011          \\
\multicolumn{1}{c}{CV}    & 0.13\%          & 0.21\%          & 0.40\%          & 0.03\%          & 0.06\%          & 0.06\%          & 0.84\%          & 0.25\%          \\ \hline
\end{tabular}%
}
\caption{Segment-level Kendall's $\tau$ and system-level Pearson's $r$ on WMT19 for stopwords tests. Bold values indicate the best performances.}

\label{tab:wmt19 stopwords}
\end{table*}



\subsection{IDF tables}\label{sec:idf}
\begin{table*}[htbp]
\centering
\resizebox{0.79\textwidth}{!}{%
\begin{tabular}{lcccccccc}
\hline
\multicolumn{9}{c}{segment-level} \\
metric & cs-en & de-en & fi-en & lv-en & ru-en & tr-en & zh-en & average \\ \hline
Mover-1+idf$_{ori}$ & 0.6698 & \textbf{0.7083} & \textbf{0.8214} & 0.7174 & \textbf{0.7379} & 0.7618 & \textbf{0.7442} & 0.7373 \\
Mover-1+idf$_{dis}$ & 0.6487 & 0.6765 & 0.8101 & 0.6994 & 0.7177 & 0.7581 & 0.7363 & 0.7210 \\
Mover-1+idf$_{rand}$ & 0.6696 & 0.7064 & 0.8199 & \textbf{0.7195} & 0.7385 & 0.7615 & 0.7423 & 0.7368 \\
Mover-1+idf$_{rand}$ & \textbf{0.6702} & 0.7072 & 0.8200 & 0.7187 & 0.7389 & \textbf{0.7635} & 0.7432 & \textbf{0.7374} \\
Mover-1+idf$_{rand}$ & 0.6682 & 0.7054 & 0.8202 & 0.7187 & 0.7378 & 0.7619 & 0.7432 & 0.7365 \\
Mover-1+idf$_{rand}$ & 0.6692 & 0.7071 & 0.8187 & 0.7190 & 0.7370 & 0.7594 & 0.7437 & 0.7363 \\ \hline
\multicolumn{1}{c}{range(ori+rand)} & 0.0021 & 0.0029 & 0.0027 & 0.0021 & 0.0019 & 0.0041 & 0.0019 & 0.0011 \\
\multicolumn{1}{c}{CV(ori+rand)} & 0.12\% & 0.15\% & 0.12\% & 0.11\% & 0.10\% & 0.19\% & 0.09\% & 0.13\% \\
\multicolumn{1}{c}{AD(dis-ori)} & -0.0211 & -0.0317 & -0.0114 & -0.0180 & -0.0202 & -0.0038 & -0.0079 & -0.0163 \\
\multicolumn{1}{c}{RD(dis-ori)} & -3.15\% & -4.48\% & -1.38\% & -2.51\% & -2.73\% & -0.49\% & -1.06\% & -2.26\% \\ \hline
Mover-2+idf$_{ori}$ & \textbf{0.6786} & \textbf{0.7092} & \textbf{0.8145} & 0.7157 & \textbf{0.7357} & \textbf{0.7622} & 0.7380 & \textbf{0.7363} \\
Mover-2+idf$_{dis}$ & 0.6552 & 0.6757 & 0.8005 & 0.6986 & 0.7067 & 0.7587 & 0.7326 & 0.7183 \\
Mover-2+idf$_{rand}$ & 0.6716 & 0.7016 & 0.8108 & 0.7116 & 0.7337 & 0.7587 & 0.7305 & 0.7312 \\
Mover-2+idf$_{rand}$ & 0.6705 & 0.7005 & 0.8109 & 0.7118 & 0.7320 & 0.7571 & 0.7296 & 0.7303 \\
Mover-2+idf$_{rand}$ & 0.6734 & 0.6990 & 0.8035 & 0.7029 & 0.7272 & 0.7540 & 0.7260 & 0.7266 \\
Mover-2+idf$_{rand}$ & 0.6577 & 0.6945 & 0.8040 & \textbf{0.7215} & 0.7236 & 0.7605 & \textbf{0.7418} & 0.7291 \\ \hline
\multicolumn{1}{c}{range(ori+rand)} & 0.0209 & 0.0147 & 0.0110 & 0.0185 & 0.0121 & 0.0082 & 0.0158 & 0.0097 \\
\multicolumn{1}{c}{CV(ori+rand)} & 1.15\% & 0.76\% & 0.59\% & 0.95\% & 0.68\% & 0.42\% & 0.89\% & 0.78\% \\
\multicolumn{1}{c}{AD(dis-ori)} & -0.0234 & -0.0335 & -0.0140 & -0.0171 & -0.0291 & -0.0035 & -0.0055 & -0.0180 \\
\multicolumn{1}{c}{RD(dis-ori)} & -3.44\% & -4.72\% & -1.71\% & -2.39\% & -3.95\% & -0.46\% & -0.74\% & -2.49\% \\ \hline
BERT-F1+idf$_{ori}$ & 0.6553 & \textbf{0.6816} & \textbf{0.8230} & 0.7127 & \textbf{0.7254} & 0.7180 & 0.7121 & \textbf{0.7183} \\
BERT-F1+idf$_{dis}$ & 0.6542 & 0.6711 & 0.8105 & 0.6918 & 0.7071 & \textbf{0.7306} & \textbf{0.7139} & 0.7113 \\
BERT-F1+idf$_{rand}$ & \textbf{0.6649} & 0.6806 & 0.8202 & 0.7130 & 0.7242 & 0.7162 & 0.7085 & 0.7182 \\
BERT-F1+idf$_{rand}$ & 0.6645 & 0.6791 & 0.8205 & \textbf{0.7133} & 0.7246 & 0.7169 & 0.7091 & 0.7183 \\
BERT-F1+idf$_{rand}$ & 0.6628 & 0.6789 & 0.8209 & 0.7132 & 0.7238 & 0.7156 & 0.7091 & 0.7178 \\
BERT-F1+idf$_{rand}$ & 0.6629 & 0.6811 & 0.8200 & 0.7131 & 0.7246 & 0.7150 & 0.7085 & 0.7179 \\ \hline
\multicolumn{1}{c}{range(ori+rand)} & 0.0096 & 0.0027 & 0.0030 & 0.0006 & 0.0016 & 0.0030 & 0.0036 & 0.0005 \\
\multicolumn{1}{c}{CV(ori+rand)} & 0.59\% & 0.18\% & 0.15\% & 0.03\% & 0.08\% & 0.16\% & 0.21\% & 0.20\% \\
\multicolumn{1}{c}{AD(dis-ori)} & -0.0011 & -0.0105 & -0.0125 & -0.0209 & -0.0183 & 0.0126 & 0.0018 & -0.0070 \\
\multicolumn{1}{c}{RD(dis-ori)} & -0.16\% & -1.54\% & -1.51\% & -2.94\% & -2.52\% & 1.75\% & 0.25\% & -0.95\% \\ \hline
\multicolumn{9}{c}{system-level} \\
metric & cs-en & de-en & fi-en & lv-en & ru-en & tr-en & zh-en & average \\ \hline
Mover-1+idf$_{ori}$ & \textbf{0.9989} & \textbf{0.9794} & 0.9731 & 0.9711 & \textbf{0.9736} & 0.9911 & 0.9511 & 0.9769 \\
Mover-1+idf$_{dis}$ & 0.9963 & 0.9770 & \textbf{0.9743} & \textbf{0.9790} & 0.9577 & \textbf{0.9975} & \textbf{0.9630} & \textbf{0.9778} \\
Mover-1+idf$_{rand}$ & 0.9985 & 0.9754 & 0.9734 & 0.9705 & 0.9726 & 0.9903 & 0.9518 & 0.9761 \\
Mover-1+idf$_{rand}$ & 0.9985 & 0.9756 & 0.9736 & 0.9706 & 0.9729 & 0.9901 & 0.9515 & 0.9761 \\
Mover-1+idf$_{rand}$ & 0.9985 & 0.9753 & 0.9734 & 0.9703 & 0.9728 & 0.9900 & 0.9509 & 0.9759 \\
Mover-1+idf$_{rand}$ & 0.9986 & 0.9755 & 0.9733 & 0.9704 & 0.9726 & 0.9903 & 0.9516 & 0.9760 \\ \hline
\multicolumn{1}{c}{range(ori+rand)} & 0.0004 & 0.0040 & 0.0005 & 0.0008 & 0.0010 & 0.0012 & 0.0009 & 0.0010 \\
\multicolumn{1}{c}{CV(ori+rand)} & 0.01\% & 0.18\% & 0.02\% & 0.03\% & 0.04\% & 0.05\% & 0.04\% & 0.05\% \\
\multicolumn{1}{c}{AD(dis-ori)} & -0.0025 & -0.0024 & 0.0012 & 0.0078 & -0.0159 & 0.0063 & 0.0119 & 0.0009 \\
\multicolumn{1}{c}{RD(dis-ori)} & -0.25\% & -0.24\% & 0.13\% & 0.81\% & -1.63\% & 0.64\% & 1.25\% & 0.10\% \\ \hline
Mover-2+idf$_{ori}$ & \textbf{0.9994} & \textbf{0.9812} & 0.9762 & 0.9724 & \textbf{0.9714} & 0.9954 & 0.9559 & \textbf{0.9788} \\
Mover-2+idf$_{dis}$ & 0.9963 & 0.9753 & 0.9773 & \textbf{0.9821} & 0.9548 & 0.9959 & \textbf{0.9643} & 0.9780 \\
Mover-2+idf$_{rand}$ & 0.9973 & 0.9731 & 0.9760 & 0.9696 & 0.9706 & 0.9926 & 0.9561 & 0.9765 \\
Mover-2+idf$_{rand}$ & 0.9973 & 0.9726 & 0.9757 & 0.9691 & 0.9710 & 0.9919 & 0.9554 & 0.9762 \\
Mover-2+idf$_{rand}$ & 0.9982 & 0.9721 & 0.9759 & 0.9687 & 0.9705 & 0.9922 & 0.9555 & 0.9762 \\
Mover-2+idf$_{rand}$ & 0.9953 & 0.9754 & \textbf{0.9790} & 0.9744 & 0.9653 & \textbf{0.9972} & 0.9620 & 0.9784 \\ \hline
\multicolumn{1}{c}{range(ori+rand)} & 0.0041 & 0.0091 & 0.0033 & 0.0057 & 0.0060 & 0.0053 & 0.0066 & 0.0027 \\
\multicolumn{1}{c}{CV(ori+rand)} & 0.15\% & 0.38\% & 0.14\% & 0.25\% & 0.26\% & 0.23\% & 0.30\% & 0.25\% \\
\multicolumn{1}{c}{AD(dis-ori)} & -0.0032 & -0.0059 & 0.0010 & 0.0097 & -0.0166 & 0.0005 & 0.0083 & -0.0008 \\
\multicolumn{1}{c}{RD(dis-ori)} & -0.32\% & -0.60\% & 0.11\% & 1.00\% & -1.71\% & 0.05\% & 0.87\% & -0.08\% \\ \hline
BERT-F1+idf$_{ori}$ & 0.9915 & 0.9674 & \textbf{0.9946} & \textbf{0.9914} & 0.9595 & \textbf{0.9958} & 0.9528 & 0.9790 \\
BERT-F1+idf$_{dis}$ & 0.9869 & 0.9608 & 0.9791 & 0.9909 & 0.9367 & 0.9907 & 0.9535 & 0.9712 \\
BERT-F1+idf$_{rand}$ & 0.9954 & 0.9686 & 0.9945 & 0.9903 & 0.9598 & 0.9953 & 0.9537 & 0.9797 \\
BERT-F1+idf$_{rand}$ & 0.9951 & 0.9686 & 0.9946 & 0.9903 & 0.9601 & 0.9952 & 0.9537 & 0.9796 \\
BERT-F1+idf$_{rand}$ & \textbf{0.9953} & \textbf{0.9688} & 0.9944 & 0.9902 & \textbf{0.9602} & 0.9953 & \textbf{0.9535} & \textbf{0.9797} \\
BERT-F1+idf$_{rand}$ & 0.9950 & 0.9686 & 0.9944 & 0.9904 & 0.9599 & 0.9953 & 0.9537 & 0.9796 \\ \hline
\multicolumn{1}{c}{range(ori+rand)} & 0.0039 & 0.0013 & 0.0002 & 0.0012 & 0.0007 & 0.0006 & 0.0010 & 0.0007 \\
\multicolumn{1}{c}{CV(ori+rand)} & 0.16\% & 0.06\% & \textbf{0.01\%} & \textbf{0.05\%} & \textbf{0.03\%} & 0.02\% & 0.04\% & 0.05\% \\
\multicolumn{1}{c}{AD(dis-ori)} & -0.0046 & -0.0066 & -0.0155 & -0.0005 & -0.0228 & -0.0051 & 0.0007 & -0.0078 \\
\multicolumn{1}{c}{RD(dis-ori)} & -0.47\% & -0.69\% & -1.56\% & -0.05\% & -2.37\% & -0.51\% & 0.07\% & -0.80\% \\ \hline
\end{tabular}%
}
\caption{Segment-level Pearson's $r$ and system-level Pearson's $r$ on WMT17 for IDF-weighting tests. Bold values indicate the best performances.}
\label{tab:wmt17 idf}
\end{table*}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[htbp]
\centering
\resizebox{0.79\textwidth}{!}{%
\begin{tabular}{lcccccccc}
\hline
\multicolumn{9}{c}{segment-level} \\
metric & cs-en & de-en & et-en & fi-en & ru-en & tr-en & zh-en & average \\ \hline
Mover-1+idf$_{ori}$ & 0.3726 & \textbf{0.5414} & 0.3944 & \textbf{0.2917} & \textbf{0.3414} & 0.2847 & \textbf{0.2591} & \textbf{0.3550} \\
Mover-1+idf$_{dis}$ & 0.3483 & 0.5255 & 0.3895 & 0.2818 & 0.3258 & 0.2755 & 0.2528 & 0.3428 \\
Mover-1+idf$_{rand}$ & 0.3734 & 0.5365 & 0.3926 & 0.2882 & 0.3372 & 0.2802 & 0.2521 & 0.3515 \\
Mover-1+idf$_{rand}$ & \textbf{0.3738} & 0.5369 & 0.3935 & 0.2867 & 0.3353 & 0.2847 & 0.2542 & 0.3521 \\
Mover-1+idf$_{rand}$ & 0.3730 & 0.5385 & \textbf{0.3954} & 0.2851 & 0.3370 & 0.2861 & 0.2520 & 0.3524 \\
Mover-1+idf$_{rand}$ & 0.3773 & 0.5372 & 0.3946 & 0.2874 & 0.3368 & \textbf{0.2868} & 0.2544 & 0.3535 \\ \hline
\multicolumn{1}{c}{range(ori+rand)} & 0.0047 & 0.0049 & 0.0028 & 0.0065 & 0.0062 & 0.0066 & 0.0071 & 0.0036 \\
\multicolumn{1}{c}{CV(ori+rand)} & 0.51\% & 0.37\% & 0.27\% & 0.84\% & 0.68\% & 0.90\% & 1.13\% & 0.67\% \\
\multicolumn{1}{c}{AD(dis-ori)} & -0.0243 & -0.0159 & -0.0049 & -0.0098 & -0.0156 & -0.0091 & -0.0064 & -0.0122 \\
\multicolumn{1}{c}{RD(dis-ori)} & -6.51\% & -2.93\% & -1.23\% & -3.37\% & -4.56\% & -3.21\% & -2.45\% & -3.47\% \\ \hline
Mover-2+idf$_{ori}$ & 0.3738 & \textbf{0.5416} & 0.3911 & 0.2891 & 0.3351 & \textbf{0.2957} & \textbf{0.2543} & \textbf{0.3544} \\
Mover-2+idf$_{dis}$ & 0.3499 & 0.5255 & 0.3831 & 0.2784 & 0.3270 & 0.2755 & 0.2458 & 0.3407 \\
Mover-2+idf$_{rand}$ & \textbf{0.3773} & 0.5298 & \textbf{0.3926} & \textbf{0.2921} & \textbf{0.3391} & 0.2889 & 0.2501 & 0.3528 \\
Mover-2+idf$_{rand}$ & 0.3656 & 0.5328 & 0.3881 & 0.2814 & 0.3326 & 0.2842 & 0.2511 & 0.3480 \\
Mover-2+idf$_{rand}$ & 0.3644 & 0.5329 & 0.3876 & 0.2826 & 0.3310 & 0.2823 & 0.2507 & 0.3474 \\
Mover-2+idf$_{rand}$ & 0.3769 & 0.5355 & 0.3923 & 0.2881 & 0.3312 & 0.2929 & 0.2508 & 0.3525 \\ \hline
\multicolumn{1}{c}{range(ori+rand)} & 0.0129 & 0.0118 & 0.0050 & 0.0106 & 0.0081 & 0.0134 & 0.0043 & 0.0070 \\
\multicolumn{1}{c}{CV(ori+rand)} & 1.67\% & 0.83\% & 0.60\% & 1.57\% & 1.01\% & 1.95\% & 0.66\% & 1.19\% \\
\multicolumn{1}{c}{AD(dis-ori)} & -0.0239 & -0.0161 & -0.0079 & -0.0107 & -0.0081 & -0.0202 & -0.0085 & -0.0136 \\
\multicolumn{1}{c}{RD(dis-ori)} & -6.39\% & -2.97\% & -2.03\% & -3.71\% & -2.41\% & -6.82\% & -3.35\% & -3.95\% \\ \hline
BERT-F1+idf$_{ori}$ & 0.3714 & 0.5372 & 0.3920 & \textbf{0.2958} & \textbf{0.3414} & 0.2884 & 0.2450 & 0.3530 \\
BERT-F1+idf$_{dis}$ & 0.3718 & 0.5311 & 0.3848 & 0.2863 & 0.3410 & 0.2669 & 0.2433 & 0.3465 \\
BERT-F1+idf$_{rand}$ & \textbf{0.3753} & \textbf{0.5377} & 0.3926 & 0.2946 & 0.3356 & 0.2894 & \textbf{0.2457} & 0.3530 \\
BERT-F1+idf$_{rand}$ & 0.3738 & 0.5361 & \textbf{0.3928} & 0.2912 & 0.3381 & 0.2894 & 0.2447 & 0.3523 \\
BERT-F1+idf$_{rand}$ & 0.3734 & 0.5368 & 0.3920 & 0.2947 & 0.3374 & 0.2884 & 0.2452 & 0.3526 \\
BERT-F1+idf$_{rand}$ & 0.3753 & 0.5371 & 0.3926 & 0.2950 & 0.3391 & \textbf{0.2899} & 0.2448 & \textbf{0.3534} \\ \hline
\multicolumn{1}{c}{range(ori+rand)} & 0.0039 & 0.0016 & 0.0008 & 0.0046 & 0.0058 & 0.0014 & 0.0010 & 0.0011 \\
\multicolumn{1}{c}{CV(ori+rand)} & 0.43\% & 0.11\% & 0.10\% & 0.61\% & 0.63\% & 0.22\% & 0.16\% & 0.32\% \\
\multicolumn{1}{c}{AD(dis-ori)} & 0.0004 & -0.0061 & -0.0072 & -0.0095 & -0.0004 & -0.0216 & -0.0017 & -0.0066 \\
\multicolumn{1}{c}{RD(dis-ori)} & 0.11\% & -1.14\% & -1.83\% & -3.20\% & -0.11\% & -7.48\% & -0.69\% & -2.05\% \\ \hline
\multicolumn{9}{c}{system-level} \\
metric & cs-en & de-en & et-en & fi-en & ru-en & tr-en & zh-en & average \\ \hline
Mover-1+idf$_{ori}$ & \textbf{0.9889} & \textbf{0.9959} & 0.9846 & 0.9938 & \textbf{0.9926} & 0.9823 & 0.9861 & 0.9892 \\
Mover-1+idf$_{dis}$ & 0.9877 & 0.9940 & \textbf{0.9878} & 0.9926 & 0.9888 & 0.9352 & \textbf{0.9891} & 0.9822 \\
Mover-1+idf$_{rand}$ & 0.9879 & 0.9945 & 0.9837 & \textbf{0.9947} & 0.9917 & 0.9857 & 0.9868 & 0.9893 \\
Mover-1+idf$_{rand}$ & 0.9881 & 0.9947 & 0.9837 & 0.9945 & 0.9919 & 0.9842 & 0.9866 & 0.9891 \\
Mover-1+idf$_{rand}$ & 0.9883 & 0.9945 & 0.9837 & 0.9946 & 0.9918 & \textbf{0.9859} & 0.9866 & \textbf{0.9894} \\
Mover-1+idf$_{rand}$ & 0.9883 & 0.9944 & 0.9837 & 0.9947 & 0.9917 & 0.9850 & 0.9867 & 0.9892 \\ \hline
\multicolumn{1}{c}{range(ori+rand)} & 0.0010 & 0.0015 & 0.0009 & 0.0010 & 0.0009 & 0.0036 & 0.0007 & 0.0003 \\
\multicolumn{1}{c}{CV(ori+rand)} & 0.04\% & 0.06\% & 0.04\% & 0.04\% & 0.04\% & 0.15\% & 0.03\% & 0.06\% \\
\multicolumn{1}{c}{AD(dis-ori)} & -0.0011 & -0.0019 & 0.0031 & -0.0012 & -0.0037 & -0.0471 & 0.0030 & -0.0070 \\
\multicolumn{1}{c}{RD(dis-ori)} & -0.11\% & -0.19\% & 0.32\% & -0.12\% & -0.38\% & -4.79\% & 0.31\% & -0.71\% \\ \hline
Mover-2+idf$_{ori}$ & 0.9888 & \textbf{0.9962} & 0.9852 & 0.9931 & \textbf{0.9914} & 0.9798 & 0.9869 & 0.9888 \\
Mover-2+idf$_{dis}$ & 0.9865 & 0.9934 & \textbf{0.9884} & 0.9913 & 0.9876 & 0.8787 & \textbf{0.9890} & 0.9736 \\
Mover-2+idf$_{rand}$ & \textbf{0.9897} & 0.9916 & 0.9830 & \textbf{0.9946} & 0.9893 & \textbf{0.9906} & 0.9882 & \textbf{0.9896} \\
Mover-2+idf$_{rand}$ & 0.9848 & 0.9942 & 0.9841 & 0.9938 & 0.9884 & 0.9869 & 0.9870 & 0.9884 \\
Mover-2+idf$_{rand}$ & 0.9840 & 0.9943 & 0.9840 & 0.9941 & 0.9880 & 0.9884 & 0.9867 & 0.9885 \\
Mover-2+idf$_{rand}$ & 0.9882 & 0.9925 & 0.9842 & 0.9943 & 0.9898 & 0.9883 & 0.9885 & 0.9894 \\ \hline
\multicolumn{1}{c}{range(ori+rand)} & 0.0058 & 0.0047 & 0.0022 & 0.0015 & 0.0034 & 0.0108 & 0.0018 & 0.0011 \\
\multicolumn{1}{c}{CV(ori+rand)} & 0.26\% & 0.18\% & 0.08\% & 0.06\% & 0.14\% & 0.42\% & 0.08\% & 0.17\% \\
\multicolumn{1}{c}{AD(dis-ori)} & -0.0023 & -0.0028 & 0.0032 & -0.0018 & -0.0039 & -0.1011 & 0.0021 & -0.0152 \\
\multicolumn{1}{c}{RD(dis-ori)} & -0.23\% & -0.28\% & 0.32\% & -0.18\% & -0.39\% & -10.32\% & 0.21\% & -1.55\% \\ \hline
BERT-F1+idf$_{ori}$ & 0.9809 & 0.9953 & 0.9832 & \textbf{0.9947} & \textbf{0.9881} & 0.9936 & 0.9814 & 0.9882 \\
BERT-F1+idf$_{dis}$ & 0.9815 & 0.9938 & \textbf{0.9833} & 0.9859 & 0.9849 & 0.9502 & \textbf{0.9839} & 0.9805 \\
BERT-F1+idf$_{rand}$ & 0.9817 & 0.9954 & 0.9825 & 0.9947 & 0.9879 & 0.9935 & 0.9814 & 0.9882 \\
BERT-F1+idf$_{rand}$ & 0.9817 & \textbf{0.9955} & 0.9825 & 0.9947 & 0.9880 & \textbf{0.9936} & 0.9815 & 0.9882 \\
BERT-F1+idf$_{rand}$ & \textbf{0.9819} & 0.9954 & 0.9825 & 0.9948 & 0.9881 & 0.9935 & \textbf{0.9814} & \textbf{0.9882} \\
BERT-F1+idf$_{rand}$ & 0.9819 & 0.9954 & 0.9825 & 0.9948 & 0.9879 & 0.9935 & 0.9814 & 0.9882 \\ \hline
\multicolumn{1}{c}{range(ori+rand)} & 0.0010 & \textbf{0.0002} & 0.0007 & 0.0002 & 0.0002 & 0.0002 & 0.0001 & 0.0001 \\
\multicolumn{1}{c}{CV(ori+rand)} & 0.04\% & 0.01\% & \textbf{0.03\%} & \textbf{0.01\%} & \textbf{0.01\%} & 0.01\% & 0.00\% & 0.02\% \\
\multicolumn{1}{c}{AD(dis-ori)} & 0.0006 & -0.0014 & 0.0001 & -0.0087 & -0.0033 & -0.0433 & 0.0025 & -0.0076 \\
\multicolumn{1}{c}{RD(dis-ori)} & 0.06\% & -0.14\% & 0.01\% & -0.88\% & -0.33\% & -4.36\% & 0.25\% & -0.77\% \\ \hline
\end{tabular}%
}
\caption{Segment-level Kendall's $\tau$ and system-level Pearson's $r$ on WMT18 for IDF-weighting tests. Bold values indicate the best performances.}
\label{tab:wmt18 idf}
\end{table*}


\begin{table*}[htbp]
\centering
\resizebox{0.79\textwidth}{!}{%
\begin{tabular}{lcccccccc}
\hline
\multicolumn{9}{c}{segment-level} \\
metric & de-en & fi-en & gu-en & kk-en & lt-en & ru-en & zh-en & average \\ \hline
Mover-1+idf$_{ori}$ & \textbf{0.2224} & \textbf{0.3436} & 0.3105 & 0.4479 & \textbf{0.3682} & \textbf{0.2183} & \textbf{0.4223} & \textbf{0.3333} \\
Mover-1+idf$_{dis}$ & 0.1462 & 0.3404 & 0.3024 & \textbf{0.4526} & 0.3619 & 0.1990 & 0.4095 & 0.3160 \\
Mover-1+idf$_{rand}$ & 0.1700 & 0.3405 & 0.3155 & 0.4503 & 0.3659 & 0.2149 & 0.4097 & 0.3238 \\
Mover-1+idf$_{rand}$ & 0.1701 & 0.3423 & 0.3187 & 0.4493 & 0.3670 & 0.2118 & 0.4122 & 0.3245 \\
Mover-1+idf$_{rand}$ & 0.1704 & 0.3410 & \textbf{0.3195} & 0.4496 & 0.3670 & 0.2087 & 0.4096 & 0.3237 \\
Mover-1+idf$_{rand}$ & 0.1714 & 0.3422 & 0.3165 & 0.4492 & 0.3678 & 0.2097 & 0.4111 & 0.3240 \\ \hline
\multicolumn{1}{c}{range(ori+rand)} & 0.0524 & 0.0030 & 0.0090 & 0.0024 & 0.0023 & 0.0096 & 0.0127 & 0.0096 \\
\multicolumn{1}{c}{CV(ori+rand)} & 12.84\% & 0.35\% & 1.12\% & 0.19\% & 0.24\% & 1.86\% & 1.29\% & 2.56\% \\
\multicolumn{1}{c}{AD(dis-ori)} & -0.0762 & -0.0031 & -0.0082 & 0.0047 & -0.0063 & -0.0193 & -0.0128 & -0.0173 \\
\multicolumn{1}{c}{RD(dis-ori)} & -34.26\% & -0.91\% & -2.63\% & 1.05\% & -1.71\% & -8.85\% & -3.03\% & -7.19\% \\ \hline
Mover-2+idf$_{ori}$ & \textbf{0.2200} & \textbf{0.3427} & 0.3095 & 0.4450 & \textbf{0.3682} & \textbf{0.2231} & \textbf{0.4242} & \textbf{0.3333} \\
Mover-2+idf$_{dis}$ & 0.1410 & 0.3341 & 0.2961 & 0.4421 & 0.3539 & 0.1981 & 0.4021 & 0.3096 \\
Mover-2+idf$_{rand}$ & 0.1533 & 0.3379 & \textbf{0.3188} & 0.4415 & 0.3604 & 0.2080 & 0.4088 & 0.3184 \\
Mover-2+idf$_{rand}$ & 0.1533 & 0.3379 & \textbf{0.3188} & 0.4415 & 0.3604 & 0.2080 & 0.4088 & 0.3184 \\
Mover-2+idf$_{rand}$ & 0.1513 & 0.3370 & 0.3121 & 0.4426 & 0.3609 & 0.2021 & 0.4111 & 0.3167 \\
Mover-2+idf$_{rand}$ & 0.1560 & 0.3437 & 0.3182 & \textbf{0.4452} & 0.3657 & 0.2090 & 0.4105 & 0.3212 \\ \hline
\multicolumn{1}{c}{range(ori+rand)} & 0.0687 & 0.0067 & 0.0092 & 0.0037 & 0.0079 & 0.0210 & 0.0154 & 0.0165 \\
\multicolumn{1}{c}{CV(ori+rand)} & 17.87\% & 0.91\% & 1.38\% & 0.41\% & 1.00\% & 3.71\% & 1.58\% & 3.84\% \\
\multicolumn{1}{c}{AD(dis-ori)} & -0.0790 & -0.0086 & -0.0135 & -0.0030 & -0.0144 & -0.0250 & -0.0221 & -0.0236 \\
\multicolumn{1}{c}{RD(dis-ori)} & -35.91\% & -2.50\% & -4.36\% & -0.66\% & -3.90\% & -11.20\% & -5.22\% & -9.11\% \\ \hline
BERT-F1+idf$_{ori}$ & 0.1524 & 0.3365 & 0.2997 & \textbf{0.4454} & \textbf{0.3715} & 0.2055 & 0.4051 & 0.3166 \\
BERT-F1+idf$_{dis}$ & 0.1504 & 0.3385 & 0.2873 & 0.4345 & 0.3630 & 0.2003 & 0.4026 & 0.3110 \\
BERT-F1+idf$_{rand}$ & 0.1538 & 0.3394 & 0.2987 & 0.4438 & 0.3687 & 0.2067 & \textbf{0.4077} & \textbf{0.3170} \\
BERT-F1+idf$_{rand}$ & \textbf{0.1554} & 0.3391 & 0.2991 & 0.4431 & 0.3665 & \textbf{0.2070} & 0.4075 & 0.3168 \\
BERT-F1+idf$_{rand}$ & 0.1548 & 0.3393 & \textbf{0.3007} & 0.4426 & 0.3678 & 0.2064 & 0.4073 & 0.3170 \\
BERT-F1+idf$_{rand}$ & 0.1548 & \textbf{0.3403} & 0.2991 & 0.4412 & 0.3677 & 0.2066 & 0.4065 & 0.3166 \\ \hline
\multicolumn{1}{c}{range(ori+rand)} & 0.0030 & 0.0039 & 0.0020 & 0.0042 & 0.0050 & 0.0015 & 0.0026 & 0.0004 \\
\multicolumn{1}{c}{CV(ori+rand)} & 0.76\% & 0.43\% & 0.26\% & 0.35\% & 0.51\% & 0.27\% & 0.26\% & 0.41\% \\
\multicolumn{1}{c}{AD(dis-ori)} & -0.0020 & 0.0020 & -0.0124 & -0.0109 & -0.0085 & -0.0052 & -0.0024 & -0.0056 \\
\multicolumn{1}{c}{RD(dis-ori)} & -1.29\% & 0.59\% & -4.14\% & -2.45\% & -2.29\% & -2.51\% & -0.60\% & -1.81\% \\ \hline
\multicolumn{9}{c}{system-level} \\
metric & de-en & fi-en & gu-en & kk-en & lt-en & ru-en & zh-en & average \\ \hline
Mover-1+idf$_{ori}$ & 0.9247 & 0.9940 & 0.9132 & 0.9839 & 0.9634 & \textbf{0.9771} & \textbf{0.9686} & 0.9607 \\
Mover-1+idf$_{dis}$ & 0.9234 & 0.9904 & 0.9200 & \textbf{0.9903} & \textbf{0.9637} & 0.9712 & 0.9590 & 0.9597 \\
Mover-1+idf$_{rand}$ & 0.9252 & 0.9945 & 0.9308 & 0.9895 & 0.9620 & 0.9753 & 0.9677 & 0.9636 \\
Mover-1+idf$_{rand}$ & \textbf{0.9258} & 0.9945 & 0.9307 & 0.9897 & 0.9622 & 0.9753 & 0.9680 & 0.9638 \\
Mover-1+idf$_{rand}$ & 0.9255 & \textbf{0.9945} & \textbf{0.9358} & 0.9901 & 0.9623 & 0.9756 & 0.9678 & \textbf{0.9645} \\
Mover-1+idf$_{rand}$ & 0.9254 & 0.9945 & 0.9318 & 0.9895 & 0.9623 & 0.9752 & 0.9678 & 0.9638 \\ \hline
\multicolumn{1}{c}{range(ori+rand)} & 0.0011 & 0.0005 & 0.0226 & 0.0062 & 0.0014 & 0.0019 & 0.0009 & 0.0038 \\
\multicolumn{1}{c}{CV(ori+rand)} & 0.04\% & 0.02\% & 0.95\% & 0.26\% & 0.06\% & 0.08\% & 0.04\% & 0.21\% \\
\multicolumn{1}{c}{AD(dis-ori)} & -0.0013 & -0.0036 & 0.0068 & 0.0064 & 0.0003 & -0.0059 & -0.0096 & -0.0010 \\
\multicolumn{1}{c}{RD(dis-ori)} & -0.14\% & -0.36\% & 0.74\% & 0.65\% & 0.03\% & -0.60\% & -0.99\% & -0.09\% \\ \hline
Mover-2+idf$_{ori}$ & 0.9242 & 0.9942 & 0.9137 & 0.9847 & \textbf{0.9631} & \textbf{0.9753} & 0.9661 & 0.9602 \\
Mover-2+idf$_{dis}$ & 0.9226 & 0.9903 & 0.9170 & 0.9914 & 0.9617 & 0.9684 & 0.9553 & 0.9581 \\
Mover-2+idf$_{rand}$ & \textbf{0.9287} & \textbf{0.9949} & 0.9586 & \textbf{0.9923} & 0.9598 & 0.9701 & 0.9683 & \textbf{0.9675} \\
Mover-2+idf$_{rand}$ & \textbf{0.9287} & \textbf{0.9949} & 0.9586 & \textbf{0.9923} & 0.9598 & 0.9701 & \textbf{0.9683} & \textbf{0.9675} \\
Mover-2+idf$_{rand}$ & 0.9216 & 0.9932 & 0.9353 & 0.9908 & 0.9613 & 0.9721 & 0.9617 & 0.9623 \\
Mover-2+idf$_{rand}$ & 0.9280 & 0.9940 & 0.9476 & 0.9912 & 0.9592 & 0.9691 & 0.9666 & 0.9651 \\ \hline
\multicolumn{1}{c}{range(ori+rand)} & 0.0071 & 0.0017 & 0.0449 & 0.0076 & 0.0039 & 0.0062 & 0.0065 & 0.0073 \\
\multicolumn{1}{c}{CV(ori+rand)} & 0.35\% & 0.07\% & 2.00\% & 0.32\% & 0.17\% & 0.26\% & 0.28\% & 0.49\% \\
\multicolumn{1}{c}{AD(dis-ori)} & -0.0016 & -0.0039 & 0.0034 & 0.0066 & -0.0014 & -0.0069 & -0.0108 & -0.0021 \\
\multicolumn{1}{c}{RD(dis-ori)} & -0.17\% & -0.39\% & 0.37\% & 0.67\% & -0.15\% & -0.71\% & -1.12\% & -0.21\% \\ \hline
BERT-F1+idf$_{ori}$ & 0.9272 & 0.9871 & \textbf{0.9305} & 0.9973 & 0.9695 & \textbf{0.9771} & 0.9633 & \textbf{0.9646} \\
BERT-F1+idf$_{dis}$ & \textbf{0.9276} & 0.9819 & 0.9007 & \textbf{0.9976} & \textbf{0.9704} & 0.9747 & 0.9545 & 0.9582 \\
BERT-F1+idf$_{rand}$ & 0.9272 & 0.9880 & 0.9247 & 0.9971 & 0.9663 & 0.9771 & 0.9637 & 0.9634 \\
BERT-F1+idf$_{rand}$ & 0.9272 & \textbf{0.9881} & 0.9242 & 0.9973 & 0.9668 & 0.9769 & 0.9639 & 0.9635 \\
BERT-F1+idf$_{rand}$ & 0.9271 & 0.9880 & 0.9314 & 0.9973 & 0.9664 & 0.9770 & \textbf{0.9638} & 0.9644 \\
BERT-F1+idf$_{rand}$ & 0.9273 & 0.9880 & 0.9263 & 0.9971 & 0.9667 & 0.9770 & 0.9637 & 0.9637 \\ \hline
\multicolumn{1}{c}{range(ori+rand)} & 0.0002 & \textbf{0.0010} & 0.0071 & 0.0002 & 0.0033 & 0.0002 & 0.0006 & 0.0012 \\
\multicolumn{1}{c}{CV(ori+rand)} & 0.01\% & 0.04\% & \textbf{0.36\%} & \textbf{0.01\%} & \textbf{0.14\%} & 0.01\% & 0.02\% & 0.08\% \\
\multicolumn{1}{c}{AD(dis-ori)} & 0.0004 & -0.0052 & -0.0298 & 0.0004 & 0.0008 & -0.0024 & -0.0088 & -0.0064 \\
\multicolumn{1}{c}{RD(dis-ori)} & 0.05\% & -0.52\% & -3.20\% & 0.04\% & 0.09\% & -0.24\% & -0.92\% & -0.67\% \\ \hline
\end{tabular}%
}
\caption{Segment-level Kendall's $\tau$ and system-level Pearson's $r$ on WMT19 for IDF-weighting tests. Bold values indicate the best performances.}
\label{tab:wmt19 idf}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccc|cccccc@{}}
\toprule
\multirow{3}{*}{metric} & \multicolumn{6}{c|}{TAC2008} & \multicolumn{6}{c}{TAC2009} \\
 & \multicolumn{3}{c}{\textbf{pyramid}} & \multicolumn{3}{c|}{\textbf{responsiveness}} & \multicolumn{3}{c}{\textbf{pyramid}} & \multicolumn{3}{c}{\textbf{responsivenes}} \\
 & r & rou & tau & r & rou & tau & r & rou & tau & r & rou & tau \\ \midrule
Mover-1+idf$_{ori}$ & \textbf{0.7581} & 0.6709 & 0.5167 & \textbf{0.7369} & 0.6071 & 0.5000 & \textbf{0.8296} & \textbf{0.6996} & 0.5448 & 0.7542 & 0.5908 & 0.4807 \\
Mover-1+idf$_{dis}$ & 0.7528 & 0.6667 & 0.5137 & 0.7337 & \textbf{0.6090} & \textbf{0.5015} & 0.8247 & 0.7007 & \textbf{0.5516} & 0.7554 & 0.5927 & \textbf{0.4809} \\
Mover-1+idf$_{rand}$ & 0.7581 & \textbf{0.6722} & 0.5187 & 0.7352 & 0.6035 & 0.4963 & 0.8291 & 0.6995 & 0.5496 & \textbf{0.7566} & \textbf{0.5931} & 0.4820 \\
Mover-1+idf$_{rand}$ & 0.7576 & 0.6718 & 0.5185 & 0.7344 & 0.6034 & 0.4964 & 0.8281 & 0.6990 & 0.5502 & 0.7540 & 0.5875 & 0.4772 \\
Mover-1+idf$_{rand}$ & 0.7561 & 0.6695 & 0.5136 & 0.7350 & 0.6034 & 0.4969 & 0.8296 & 0.6996 & 0.5502 & 0.7542 & 0.5908 & 0.4807 \\
Mover-1+idf$_{rand}$ & 0.7573 & 0.6712 & \textbf{0.5169} & 0.7349 & 0.6034 & 0.4965 & 0.8289 & 0.6994 & 0.5500 & 0.7549 & 0.5905 & 0.4800 \\ \midrule
\multicolumn{1}{c}{range(ori+rand)} & 0.0020 & 0.0027 & 0.0052 & 0.0025 & 0.0037 & 0.0037 & 0.0016 & 0.0006 & 0.0054 & 0.0026 & 0.0055 & 0.0048 \\
\multicolumn{1}{c}{CV(ori+rand)} & 0.11\% & 0.15\% & 0.40\% & 0.13\% & 0.27\% & 0.31\% & 0.08\% & 0.04\% & 0.43\% & 0.14\% & 0.33\% & 0.37\% \\
\multicolumn{1}{c}{AD(dis-ori)} & -0.0053 & -0.0042 & -0.0030 & -0.0031 & 0.0019 & 0.0015 & -0.0049 & 0.0010 & 0.0068 & 0.0012 & 0.0020 & 0.0002 \\
\multicolumn{1}{c}{RD(dis-ori)} & -0.70\% & -0.62\% & -0.58\% & -0.43\% & 0.32\% & 0.30\% & -0.60\% & 0.15\% & 1.25\% & 0.16\% & 0.33\% & 0.04\% \\ \midrule
Mover-2+idf$_{ori}$ & \textbf{0.7521} & \textbf{0.6623} & \textbf{0.5100} & \textbf{0.7338} & \textbf{0.6002} & \textbf{0.4939} & \textbf{0.8246} & 0.6934 & \textbf{0.5100} & 0.7530 & 0.5855 & 0.4754 \\
Mover-2+idf$_{dis}$ & 0.7428 & 0.6479 & 0.4968 & 0.7275 & 0.5925 & 0.4868 & 0.8160 & 0.6849 & 0.4968 & 0.7538 & 0.5846 & 0.4734 \\
Mover-2+idf$_{rand}$ & 0.7502 & 0.6594 & 0.5077 & 0.7304 & 0.5947 & 0.4895 & 0.8236 & 0.6909 & 0.5077 & \textbf{0.7552} & 0.5855 & 0.4753 \\
Mover-2+idf$_{rand}$ & 0.7496 & 0.6583 & 0.5066 & 0.7306 & 0.5972 & 0.4909 & 0.8223 & 0.6884 & 0.5066 & 0.7528 & 0.5811 & 0.4713 \\
Mover-2+idf$_{rand}$ & 0.7507 & 0.6608 & 0.5091 & 0.7311 & 0.5952 & 0.4893 & 0.8230 & \textbf{0.6935} & 0.5091 & 0.7537 & \textbf{0.5879} & \textbf{0.4773} \\
Mover-2+idf$_{rand}$ & 0.7502 & 0.6595 & 0.5078 & 0.7307 & 0.5957 & 0.4899 & 0.8229 & 0.6909 & 0.5078 & 0.7539 & 0.5849 & 0.4746 \\ \midrule
\multicolumn{1}{c}{range(ori+rand)} & 0.0025 & 0.0040 & 0.0035 & 0.0034 & 0.0055 & 0.0046 & 0.0024 & 0.0051 & 0.0035 & 0.0024 & 0.0068 & 0.0060 \\
\multicolumn{1}{c}{CV(ori+rand)} & 0.13\% & 0.23\% & 0.27\% & 0.19\% & 0.37\% & 0.39\% & 0.11\% & 0.31\% & 0.27\% & 0.13\% & 0.42\% & 0.46\% \\
\multicolumn{1}{c}{AD(dis-ori)} & -0.0093 & -0.0144 & -0.0133 & -0.0063 & -0.0078 & -0.0072 & -0.0087 & -0.0085 & -0.0133 & 0.0008 & -0.0010 & -0.0020 \\
\multicolumn{1}{c}{RD(dis-ori)} & -1.23\% & -2.17\% & -2.60\% & -0.86\% & -1.29\% & -1.45\% & -1.05\% & -1.23\% & -2.60\% & 0.11\% & -0.17\% & -0.43\% \\ \midrule
BERT-F1+idf$_{ori}$ & 0.7502 & 0.6498 & 0.4977 & 0.7249 & 0.5966 & 0.4905 & 0.8378 & 0.7208 & 0.5701 & 0.7488 & 0.6014 & 0.4891 \\
BERT-F1+idf$_{dis}$ & 0.7480 & 0.6410 & 0.4915 & 0.7272 & 0.5970 & 0.4902 & 0.8335 & 0.7162 & 0.5663 & \textbf{0.7532} & \textbf{0.6072} & 0.4941 \\
BERT-F1+idf$_{rand}$ & 0.7509 & 0.6498 & 0.4991 & \textbf{0.7283} & \textbf{0.6019} & 0.4946 & \textbf{0.8390} & 0.7245 & 0.5746 & 0.7484 & 0.6040 & 0.4906 \\
BERT-F1+idf$_{rand}$ & 0.7519 & 0.6540 & 0.5023 & 0.7243 & 0.5986 & 0.4921 & 0.8389 & 0.7233 & 0.5728 & 0.7484 & 0.6028 & 0.4898 \\
BERT-F1+idf$_{rand}$ & \textbf{0.7539} & \textbf{0.6561} & \textbf{0.5040} & 0.7254 & 0.5998 & 0.4930 & 0.8383 & \textbf{0.7252} & \textbf{0.5749} & 0.7514 & 0.6046 & \textbf{0.4916} \\
BERT-F1+idf$_{rand}$ & 0.7522 & 0.6533 & 0.5018 & 0.7260 & 0.6001 & \textbf{0.4932} & 0.8387 & 0.7243 & 0.5741 & 0.7494 & 0.6038 & 0.4907 \\ \midrule
\multicolumn{1}{c}{range(ori+rand)} & 0.0037 & 0.0063 & 0.0063 & 0.0040 & 0.0053 & 0.0041 & 0.0012 & 0.0045 & 0.0048 & 0.0031 & 0.0032 & 0.0024 \\
\multicolumn{1}{c}{CV(ori+rand)} & 0.19\% & 0.42\% & 0.51\% & 0.21\% & 0.32\% & 0.31\% & 0.06\% & 0.24\% & 0.34\% & 0.17\% & 0.21\% & 0.19\% \\
\multicolumn{1}{c}{AD(dis-ori)} & -0.0023 & -0.0089 & -0.0061 & 0.0023 & 0.0004 & -0.0003 & -0.0043 & -0.0046 & -0.0038 & 0.0044 & 0.0058 & 0.0050 \\
\multicolumn{1}{c}{RD(dis-ori)} & -0.30\% & -1.37\% & -1.23\% & 0.32\% & 0.07\% & -0.05\% & -0.52\% & -0.63\% & -0.67\% & 0.59\% & 0.97\% & 1.01\% \\ \bottomrule
\end{tabular}%
}
\caption{Correlations on with summary-level human judgements on TAC2008-2009 for IDF-weighting tests}
\label{tab:idf tac}
\end{table*}

==> structure/structure/1_introduction.tex <==
\section{Introduction}

%\todo{SE: we need to say that the NLP community has taken a lot of measures in the last years to sustain reproducibility and we'll see here whether they had any effect - I think the didn't. Maybe that goes to the conclusion}

%After the ``reproducibility crisis'' in science \citep{baker2016reproducibility} has been attested, a wide range of research on reproducibility has been conducted in various fields, including NLP. 
Reproducibility is a core aspect in machine learning (ML) and natural language processing (NLP). It requires that claims and results of previous work can independently be reproduced and is a prerequisite to trustworthiness. 
%of a scientific field. 
The last few years have seen vivid interest in the topic and many issues of non-reproducibility have been pointed out, leading to claims of a ``reproducibility crisis'' in science \citep{baker2016reproducibility}. 
\iffalse
\begin{figure}[hbtp]
    \centering
    \includegraphics[width=\columnwidth]{figure/metric_illustration.png}
    \caption{%Illustration of BERT-based evaluation metrics}
    BERT-based evaluation metrics can be thought of as consisting of three components: BERT, aggregation and comparison mechanisms, and preprocessing. In this work, our focus is on the last part.
    }
    \label{fig:ill_metric}
\end{figure}
\fi
%\todo{SE: @Yanran: make pluses less prominent, put a red box around preprocessing}
In the field of evaluation metrics for natural language generation (NLG), 
%According to 
the seminal work of \citet{post2018call} 
has demonstrated how different preprocessing schemes %of sentences 
can lead to substantially different results when using the dominant metric at the time, BLEU \citep{Papineni2002BleuAM}. 
Thus, when researchers employ such different preprocessing steps (a seemingly innocuous decision), 
this can directly lead to reproducibility failures of conclusions and/or metric performances. %, when researchers.

Even though BLEU and similar lexical-overlap metrics still appear to dominate the landscape of NLG (particular MT) evaluation \citep{marie-etal-2021-scientific}, it is obvious that %BLEU and similar 
metrics which measure surface level overlap are unsuitable for evaluation, especially for modern text generation systems with better paraphrasing capabilities \citep{mathur-etal-2020-tangled}. 
As a remedy, multiple higher-quality metrics based on BERT and its extensions have been proposed in the last few years \citep{zhang2019bertscore,zhao2019moverscore}. In this work, we %aim to 
investigate whether these more recent metrics have better reproducibility properties, thus filling a gap for the newer paradigm of metrics. We have good reason to suspect that reproducibility will be better: (i) 
as a response to the identified problems, recent years have seen %much awareness 
many efforts in the NLP and ML communities to improve reproducibility, e.g., by requiring authors to fill out specific check lists.\footnote{E.g., \url{https://aclrollingreview.org/responsibleNLPresearch/}.} 
  (ii) Designers of novel evaluation metrics should be particularly aware of reproducibility issues, as %evaluation metrics as 
 reproducibility is a core concept of proper evaluation of NLP models \citep{eval4nlp-2021-evaluation}. 
 
 Our results are disillusioning: out of four metrics we tested, three exhibit (severe) reproducibility issues. The problems relate to (i) heavy use of (undocumented) preprocessing, (ii) missing code, (iii) reporting lower results for competitors, %and higher results for own approaches, 
 and (iv) correlating with the wrong columns in the evaluation csv file. 
 Motivated by the findings on the role of preprocessing and following \citet{post2018call}, we then study its impact more closely in the second part of the paper (for those metrics making use of it), finding that it can indeed lead to substantial performance differences also for BERT-based metrics. %This can be dangerous, as different preprocessing schemes can be the reason for artificially inflating own approaches or downplaying competitors.  
 
 %\todo{SE: wider context: cracked foundations, but negativity on the rise} 

\iffalse
different preprocessing schemes and parameter settings can lead to widely changing scores of automatic evaluation metrics and consequently make the metric scores uncomparable across different papers. 
This is critical for the development of NLG, because many researchers select to assess the system quality using automatic evaluation metrics instead of human assessment, for the simple reason that the latter is costly. If the metric scores are unreproducible, those reported ``state-of-the-art'' results may cast doubt. 
Thus, it is essential to understand how reproducible the metric scores are, i.e., the range of the variation of the metric scores independent of the evaluated texts. Only with a clear acquaintance with this point, we can determine whether the increase or decrease of the metric score truly represents a performance gain or drop of an NLG system, or is just caused by non-reproducibility. 
However, there has been scarce research on this topic; in fact, to my best knowledge, \citet{post2018call} is the only related study, but with BLEU \citep{Papineni2002BleuAM}, an automatic evaluation metric proposed two decades ago. In recent years, novel evaluation metrics achieve a much higher correlation with human than BLEU, such as BERTScore \citep{zhang2019bertscore} and MoverScore \citep{zhao2019moverscore}, benefiting from the use of BERT \citep{devlin2018bert} or its variants. Hence, the motivation of this work is to inspect whether those BERT-based evaluation metrics also suffer from the problem of generating inconsistent and uncomparable scores across users and how large the consequent variation of the metric scores can be. This thesis is split into two parts:
\begin{itemize}
    \item \textbf{Reproduction}: In the first part, we conduct reproduction experiments for selected papers to investigate the determinant factors of reproducibility for BERT-based evaluation metrics (Section \ref{chapter:bert}).
    \item \textbf{Sensitivity Analysis}: As the second part, also the primary part of this thesis, we quantify the sensitivity of selected BERT-based evaluation metrics to the factors discussed in last part. In addition, I also analyze whether the considered evaluation metrics can consistently benefit from a certain configuration regarding those factors, trying to obtain a ``cleaner'' evaluation metric by dropping some user-supported settings (Section \ref{se:sensitivity}).

    %\item \textbf{Comparison between reproducibility of machine and human evaluation}: In the last part, I compare the reproducibility of BERT-based evaluation metrics with that of human evaluation, based on the results from the participation in a shared task that aims at replication of human judgements, in order to reveal which is a more reliable and reproducible way to assess the quality of an NLG system as well as the common causes of non-reproducibility in the evaluation procedures (Chapter \ref{chapter:comparison}). 
\end{itemize}
\fi

%\todo[inline]{SE: reasons to suspect that things have become better: (i) new reproducibility guidelines, (ii) people dealing with eval metrics should be doubly careful}

==> structure/structure/2_related.tex <==
\section{Related Work}
Relevant prior work to this work includes BERT-based evaluation metrics (Section \ref{sec:rela1}) and reproducibility in NLP (Section \ref{sec:rela2}).


\subsection{BERT-based Evaluation Metrics}
\label{sec:rela1}
In recent years, %after BERT \citep{devlin2018bert} was invented, 
many strong automatic evaluation metrics based on BERT \citep{devlin2018bert} or its variants have been proposed. It has been shown that those BERT-based evaluation metrics %are able to 
correlate much better with human judgements than traditional evaluation metrics such as BLEU \citep{Papineni2002BleuAM}. 
%On the one hand, it can be categorized into two types according to whether they are trained on human judgments: \emph{supervised} and \emph{unsupervised}. 
Popular supervised BERT-based evaluation metrics include BLEURT \citep{sellam-etal-2020-bleurt} and COMET \citep{rei2020comet}, which are trained on segment-level human judgements such as DA scores in WMT datasets. %Such training procedure is not needed for 
Unsupervised BERT-based evaluation metrics such as BERTScore \citep{zhang2019bertscore}, MoverScore \citep{zhao2019moverscore}, BaryScore \citep{colombo2021automatic} and XMoverScore \citep{zhao2020limitations} do not use training signals, thus potentially may generalize better to unseen language pairs \citep{Belouadi2022USCOREAE}. 
%On the other hand, they can be also divided into \emph{reference-based} and \emph{reference-free} evaluation metrics, based on whether their scoring procedure requires human generated references. 
MoverScore, BaryScore, and BERTScore are \emph{reference-based} evaluation metrics. 
%which computes \gls{WMD} between reference and hypothesis sentences. %BERTScore is another popular reference-based evaluation metric, which relies on contextual embeddings and greedy alignment. BLEURT also falls into this category. 
In contrast, \emph{reference-free} evaluation metrics directly compare system outputs to source texts. %There are more reference-free evaluation metrics for \gls{MT} than for other \gls{NLG} tasks, 
For MT, popular such metrics are Yisi-2 \citep{lo-2019-yisi}, XMoverScore, and SentSim \citep{song-etal-2021-sentsim}. %which compares texts in source and translation languages. 
%For other tasks, 
%however, some reference-free evaluation metrics have been also proposed, such as SUPERT \citep{gao2020supert}, which is designed for text summarization evaluation.

%In this work, we mainly focus on MoverScore, which is unsupervised and reference-based. In addition, I also consider its relevant evaluation metrics: (1) BERTScore, which is also an unsupervised reference-based evaluation metric; and (2) XMoverScore, which is the reference-free version of MoverScore for \gls{MT}.
%BERT-based evaluation metrics refer to the automated evaluation metrics that assess the performance of an NLG system by using BERT representations \citep{devlin2018bert} for word (workpiece) embeddings and measuring the semantic similarity between the embeddings of the system outputs and those of the reference/source texts. Such contextual word embeddings like BERT representations can give the same word different vectors depending on its context. Mathur et al. introduce both supervised and unsupervised evaluation metrics for MT relying on BERT representations. \citet{zhang2019bertscore} proposed BERTScore, which leverages greedy alignment and contextual mbeddings like BERT, while MoverScore \citep{zhao2019moverscore} instead computes Word Mover Distance \citep{kusner2015word} to measure the (dis)similarity. XMoverScore \citep{zhao2020limitations} is the reference-free version of MoverScore for MT, which directly compares the translations to the source texts. \citet{gao2020supert} and \citet{wu2020unsupervised} design unsupervised evaluation metrics for the text summarization, also making use of BERT embeddings. 




\subsection{Reproducibility in NLP}
\label{sec:rela2}
%\subsubsection{What is reproducibility in \gls{NLP}?}
%Until now, there has been no consensus definition of the terminology involved in this field, such as the definition of replication and reproduction. According to \citet{Cohen2018ThreeDO} and \citet{Belz2021ASR}, this kind of lack makes the findings of reproduction studies uncomparable across different papers and consequently slow down the pace of the development in this field. 

\citet{Cohen2018ThreeDO} define \textbf{replicability} as the ability to repeat the process of experiments and \textbf{reproducibility} as the ability to obtain the same results. %Besides, 
%According to the \emph{goal} of the reproduction attempts, \citet{Cohen2018ThreeDO} 
They further categorize reproducibility along 3 dimensions: (1) reproducibility of a \emph{conclusion}, (2) reproducibility of a \emph{finding}, and (3) reproducibility of a \emph{value}. 
%According to ACM (Association for Computing Machinery)\footnote{\url{https://www.acm.org/publications/policies/artifact-review-and-badging-current}}: 1) repeatability means the same results can be achieved by the same team with the same experimental setup; 2) reproducibility means the same results can be achieved by different team but with the same experimental setup; 3) replicability means the same results can be achieved by different teams with different experimental setup.
%\citet{rougier2017sustainable} relate the definition of reproduction and replication to the used \emph{software}: the results have been (1) \textbf{reproduced} if they are obtained with the original data and software and (2) \textbf{replicated} if they are obtained with new software based on the computational methodologies or models described in the original paper. 
%Similar, \citet{ml2017checklist} \todo{SE: missing citation YC: added. Do you think the following description is a bit spare? I prefer deleting this. SE: what means spare? I think it is too much; we should merge and reduce the definition of those 4 papers. YC: yes, that's what I mean.} and \citet{schloss2018identifying} define the relevant terms based on the use of \emph{code and data}:
%(1) the results are \textbf{reproducible} if the same results can be obtained using the same code and data; 
%(2) the results is \textbf{replicable} if comparable results can be obtained using the same code but different data; 
%(3) the results are \textbf{robust} if comparable results can be obtained using different code but the same data;
%(4) the results are \textbf{generalizable} if comparable results can be obtained using different code and data.
In a more recent study, \citet{belz-etal-2021-systematic} categorize reproduction studies according to the \emph{condition of the reproduction experiment}: (1) \emph{reproduction under the same condition}, i.e., re-using as close as possible resources and mimicking the authors' experimental procedure as closely as possible; (2) \emph{reproduction under varied conditions}, aiming to test whether the proposed methods can obtain similar results with some changes in the settings; (3) \emph{multi-test and multi-lab studies}, i.e., reproducing multiple papers using uniform methods and multiple teams attempting to reproduce the same paper, respectively. 

%
In the first part of this work, %I conduct the first 
our reproductions follow %
the first type of reproduction experiment described by 
\citet{belz-etal-2021-systematic}, %which is 
i.e., we adhere to the original experimental setup and re-use the resources provided by the authors whenever possible, aiming at exact reproduction.
%to obtain the results reported in the original papers. %This is also the third dimension of reproducibility defined by \citet{Cohen2018ThreeDO}, i.e., reconstructing identical values.
The second part %of this work 
falls into the second category of reproduction study described by \citet{belz-etal-2021-systematic}, i.e., to change some settings on purpose to see if comparable results can be obtained. 
%With a clear statement of the definition adopted, the findings in this work may be more helpful for future work.


%Despite the confusing terminology, the 
%Previous reproduction attempts %still 
%help reveal the causes of non-reproducibility and suggest ways to facilitate it. %\todo{SE: what does this mean?} %whether successful or failed. 
According to \citet{Fokkens2013OffspringFR} and \citet{wieling-etal-2018-squib}, the main challenge is the unavailability of the source code and data. 
%\todo{SE: until here}
\citet{Dakota2017TowardsRI} study reproducibility for text mining. They show that 80\% of the failed reproduction attempts were due to the lack of information about the datasets. %As a result, they proposed a checklist of the information about how the collection procedure of the datasets should be documented. 
To investigate the current situation about the availability of source data, \citet{Mieskes2017AQS} conducted quantitative analysis on the publications from five conferences. 
They show that though 40\% of the papers reported having collected or changed existing data, only 65.2\% of them provided the links to download the data; 18\% of them were invalid. 
Similarly, \citet{wieling-etal-2018-squib} assessed the availability of both source code and data of the papers
%. They considered the full papers 
from two ACL conferences (2011 and 2016). %The code and data were obtained from the links on papers or with the help of the authors. Then, they selected five publications from each year to reproduce. 
When comparing 2016 to 2011, the availability of both data and code increased, suggesting a growing trend of sharing resources for reproduction. However, even using the same code and data, they could only recreate the identical values for one paper. This implies that a successful replication is far beyond using the same code and data. %\todo{SE: what about 1-2 recent papers, i.e., 2020+?}
More recently, \citet{belz-etal-2021-systematic} analyzed 34 reproduction studies under the same condition (re-using the original resources when possible) for NLP papers. They found that only a small portion (14.03\%) of values could be exactly reproduced and the majority (59.2\%) of the reproduced values lead to worse results. Moreover, 1/4 deviations are over 5\%.

\iffalse
\citet{huber-coltekin-2020-reproduction} repeated the experiment\todo{SE: the experiment from Wieling? We need to rewrite this paper and maybe even drop it. They reproduce only one system?} in a study of automatic essay scoring with different experimental setups (e.g., implementation (code), datasets, and languages). The replication attempts demonstrate that the 
varying conditions can cause discrepancies in results and the authors argue that such reproduction %is more worthwhile 
may be more valuable
than pursuing identical values. 
\fi
%Similar observation was made by \citet{Fokkens2013OffspringFR}. They wanted to reproduce two studies, one of which is their previous study. Surprisingly, they were not even able to reproduce their own experiment results using the same software and data. They concluded that a tiny difference in some aspects such as preprocessing steps, software versions, and experimental setup can disturb the results and therefore lead to different conclusions. Besides, the details of those aspects are often omitted in the papers. 

%Inspired by \citet{Reimers2017OptimalHF}, who investigated the effect of hyperparameter settings of deep neurual networks, \citet{Crane2018QuestionableAI} studied the reproducibility for question answering with deep neural models. They demonstrated that many neglected factors such as random seed, multithreading, framework versions (e.g., Pytorch 0.2.0 vs. Pytorch 0.1.8), and even hardware can impact the training results. Moreover, the gap between the results from different settings is often larger than the improvement reported in the majority of the papers. 

%The causes for non-reproducibility mentioned above also exist in our concerned field - automatic evaluation metrics. 
In NLG, 
\citet{post2018call} attests to the non-comparability of BLEU \citep{Papineni2002BleuAM} scores across different papers. He argues that there are four causes. \textbf{First}, BLEU is a parameterized approach. Its parameters include (1) the number of references, (2) the calculation of the length penalty for multiple reference settings, (3) the n-gram length, and (4) the smoothing applied to the 0-count n-gram. %Since it is a corpus-level metric, the fourth parameter is rarely used. And in practice, the n-gram parameter is usually set to 4. Thus, the parameters regarding multiple references have the largest impact among those parameters. 
He shows that on WMT17 \citep{wmt17}, the BLEU score for English-Finnish increases by roughly 3\% absolute Pearson correlation from using one to two references. The \textbf{second} issue, which is regarded as the most critical, %factor for non-comparability, 
is the use of different preprocessing schemes. Among these, 
%preprocessing techniques applied to BLEU, 
tokenization of the references plays a key role.
The \textbf{third} problem is that preprocessing details are hard to come by and often omitted in papers. %They argue that if these preprocessing details are well documented, comparable scores can also be reproduced. 
The \textbf{fourth} problem is different versions of datasets, in his case a particular problem with the en-de language pair in WMT14. %They gave an example that the evaluated data for English-German language pair in WMT14 dataset used to be problematic. After the problematic pieces of data were removed, the number of sentences was reduced by 10\%, which often could not be noticed by researchers. 
%
%To solve these problems, they proposed a python evaluation script that allows only metric-internal tokenization, automatically downloads multiple datasets from the web, and logs the settings.

%In this work, we conduct a similar study to \citet{post2018call}, switching objectives from BLEU to novel BERT-based evaluation metrics.


==> structure/structure/3_datasets.tex <==
\section{Datasets \& Metrics}
%This section briefly presents the datasets used in this work. 
In our reproduction experiments (Section \ref{sec:reproduction}), following \citet{zhang2019bertscore}, \citet{zhao2019moverscore} and \citet{colombo2021automatic}, we use WMT15-18 \citep{wmt15,wmt16,wmt17,wmt18} for MT evaluation. Besides,
we follow \citet{zhao2019moverscore} to use 
%WMT17  \citep{wmt17} for machine translation evaluation,
TAC2008\footnote{\url{https://tac.nist.gov/2008/}} and TAC2009\footnote{\url{https://tac.nist.gov/2009/}} %from Text Analytics Conference\footnote{\url{https://tac.nist.gov/}} 
for text summarization evaluation, MSCOCO \citep{guo-etal-2018-meteor} for image captioning evaluation, and BAGEL \citep{wen2015semantically} and SFHOTEL \citep{mairesse2010phrase} for data-to-text generation (D2T) evaluation. For the reference-free metric SentSim, we will mainly report results on the MLQE-PE dataset \citep{fomicheva2020mlqe}. %\todo{SE: add a note}
% Besides, following \citet{zhang2019bertscore} and \citet{colombo2021automatic}, we use WMT15-16 and WMT18 for MT as well.
In further experiments (Section \ref{sec:sensitivity}), we consider
%WMT18 \citep{wmt18} and 
WMT19 \citep{wmt19} for MT as well. %introduce the 
The datasets for each NLG task are described in detail in the appendix (Section \ref{sec:dataset_description}). %following sections.

==> structure/structure/4_metrics.tex <==
%\section{BERT-Based Evaluation Metrics}
%In this section, we introduce the BERT-based evaluation metrics %involved 
%examined in this work. 
%The main experimental subject in this work is MoverScore \citep{zhao2019moverscore}, for which we conduct reproduction experiment and also a more comprehensive sensitivity investigation. In addition, for a wider perspective on reproducibility for BERT-based evaluation metrics, 
For our reproduction attempts, we consider MoverScore, 
%We consider 
BERTScore, %\citep{zhang2019bertscore} 
BaryScore, and SentSim. %\todo{SE: BaryScore needs definition and SentSim results need to be included} %\citep{colombo2021automatic} in some experiments as well, since BERTScore is arguably the most popular reference-based evaluation metric, %as MoverScore, whereas 
%XMoverScore is the reference-free version of MoverScore 
%and BaryScore [...].

%\subsection
\paragraph{MoverScore} 
%MoverScore \citep{zhao2019moverscore} 
%is a reference-based evaluation metric based on Word Mover Distance \citep{} and BERT representations.
\iffalse
Its scoring procedure can be split into the following steps:
\begin{itemize}[topsep=2pt,itemsep=-1pt,leftmargin=*]
%\begin{itemize}[]
    \item Obtain contextual embeddings of reference and hypothesis sentences with the BERT base uncased model finetuned on MNLI dataset.
    \item Aggregate the last 5 layers from BERT using concatenated power means \citep{rueckle-etal-2018-pmeans}.\todo{SE: order?? YC: what do you mean? SE: in which order does pmeans come in MoverScore? 2nd step? YC: yes, I think it is. Do you think the introduction to MoverScore is too much? I wrote this in thesis because I need to introduce noisy alignment removal.} %\citep{rehurek_lrec}.
    \item Extract n-gram sequences for reference and hypothesis sentences based on BERT representations. The n-gram embeddings ($x^{n}$ and $y^{n}$) are computed as the weighted sum over its word embeddings using IDF-weighting.
    \item Calculate \emph{transportation cost matrix} C, which contains Euclidean distance between each element in $x^{n}$ to each element in $y^{n}$.
    \item Calculate \emph{transportation flow matrix} F, which is a weight matrix containing weights for each n-gram embedding, denoting the amount of flow traveling from each element in $x^{n}$ to each element in $y^{n}$.
    
    \item WMD between $x^{n}$ and $y^{n}$ is then calculated as the formula given below: 
        \begin{align*}
            \text{WMD}(x^{n},y^{n}):=\min<C,F> 
        \end{align*}
    where $<C,F>$ is the sum of the element-wise product of C and F.
    
\end{itemize}
\fi
%Thus, 
%MoverScore 
measures semantic similarity between reference and hypothesis by aligning semantically similar words and computing the amount of traveling flow between these words using the Word Mover Distance \citep{kusner2015word}. 
%\citet{zhao2019moverscore} evaluated MoverScore on four \gls{NLG} tasks: \gls{MT}, text summarization, \gls{IC}, and \gls{d2t} generation and showed that MoverScore can achieve a high correlation with human judgments on \gls{MT}, text summarization, and \gls{IC}. 


%\paragraph{XMoverScore} 
%\todo{YC: we should delete the texts about XMoverScore (also the experiments for layer selection and noisy alignment removal), right? SE: Yes, probably}
%XMoverScore \citep{zhao2020limitations} is the reference-free version of MoverScore for \gls{MT}, which directly compares the hypotheses to the source texts. XMoverScore leverages contextual embeddings with \gls{M-BERT}. It has been shown that \gls{M-BERT} is inefficient for cross-lingual tasks \citep{pires2019multilingual,Cao2020Multilingual,zhao2020limitations}. To address this issue, \citet{zhao2020limitations} proposed two re-mapping methods: \gls{CLP} and \gls{UMD}, which can improve the cross-lingual alignments in multilingual embedding space. Besides, they use a GPT language model \citep{radford2018improving} of the target language to penalize the translationese of the system translations to reflect their fluency level. 

\paragraph{BERTScore}
%BERTScore \citep{zhang2019bertscore} is also a reference-based evaluation metric. It leverages contextual embeddings such as BERT, 
calculates the cosine similarity for each token in the reference sentence with each token in the hypothesis sentence, and uses greedy alignment to obtain %\todo{SE: obtain??} 
the similarity scores between sentences. It has three variants: Recall, Precision, and F1. 
%\citet{zhang2019bertscore} evaluated BERTScore on MT and IC tasks. They recommended using F1 for MT because it consistently performs well across different settings; for IC, they claim that BERTScore-Recall outperforms the other two variants.

\paragraph{BaryScore}
%BaryScore 
%is another reference-based evaluation metric, which\todo{SE: missing} 
computes the Wasserstein distance (i.e., Earth Mover Distance \citep{rubner2000earth}) between the barycentric distribution \citep{agueh2011barycenters} of the contexual representations of reference and hypothesis to measure the dissimilarity between them.

\paragraph{SentSim} is a reference-free evaluation metrics. It combines sentence- (based on \citet{reimers-gurevych-2020-making}) and word-level models (extending a.o.\ BERTScore to the multilingual case) to score a pair of source text and hypothesis. 

==> structure/structure/5_reproduction.tex <==
\section{Reproduction Attempts}
\label{sec:reproduction}
%This section presents the experiment setup (Section \ref{set:reproduction})  and the corresponding results (Section \ref{re:reproduction}) for reproduction experiment. After that, an investigation of the factors that may affect the reproducibility of BERT-based evaluation metrics is conducted (Section \ref{sec:factors}).
%The reproduction experiment can be divided into two parts. In the first, 
%We first attempt 
Our main focus will be 
to reproduce the results on \textbf{MT} %\todo{SE: Our focus is MT and other tasks are not thoroughly evaluated across papers, right? YC: no, actually the three metrics were also evaluated on IC using MSCOCO.} 
reported in \citet{zhang2019bertscore}, \citet{zhao2019moverscore},  \citet{colombo2021automatic} and \citet{song-etal-2021-sentsim}. %In the second, 
%Then, we aim to reproduce all results reported in \citet{zhao2019moverscore}. 
%\paragraph{Experimental Setup}
%\label{set:reproduction}
\subsection{Reproduction on MT}
%In this part, we attempt to reproduce the results on MT reported in \citet{zhang2019bertscore}, \citet{zhao2019moverscore}, and \citet{colombo2021automatic}. 
%All three 
MoverScore, BaryScore and BERTScore %evaluation metrics 
were originally evaluated on MT but with different WMT datasets \citep{wmt15,wmt16,wmt17,wmt18}. 
%BERTScore was the first of them to be proposed; 
\citet{zhang2019bertscore} used WMT18 \citep{wmt18} as the main evaluation dataset. 
%for it. Soon after, 
\citet{zhao2019moverscore} %proposed MoverScore and 
reported the results on WMT17 \citep{wmt17} for both MoverScore and BERTScore-F1. \citet{colombo2021automatic} compared their metric BaryScore with MoverScore and BERTScore-F1 on WMT15 \citep{wmt15} and WMT16 \citep{wmt16}. %All authors of the subsequent proposed approaches claim that their metrics are superior to those proposed previously. %according to their experiments.
MoverScore claims to outperform BERTScore (which was published earlier on Arxiv), and BaryScore claims to outperform the earlier two. 

%As the three studies confirm the contribution of the use of the finetuned BERT model on NLI dataset \citep{wang-etal-2018-glue},\todo{SE: all three papers acknowledge this? Maybe we should rewrite to: "we evaluate all three models using the same BERT model (bert-base-uncased); two of the metrics [BERT+NLI]". Or we simply drop this sentence here} to examine the reliability of the claims regarding the improvement from the mechanisms (e.g., Word Mover Distance),
%To examine the reliability of these claims, 
%in addition to reproduce the results reported in the original papers, 
We evaluate the three metrics with the same BERT model (BERT-base-uncased) 
%\todo{SE: so they have different BERT models and in addition you evaluate on BERT-based-uncased?} 
on all MT datasets mentioned above, using the reproduction resources provided by the authors of each metric. 
We also evaluate MoverScore and BaryScore on a BERT model finetuned on NLI (as in the original papers). 
The code and data for reproduction were released on their respective githubs.\footnote{BERTScore (WMT18): \url{https://github.com/Tiiiger/bert_score/tree/master/reproduce}; MoverScore (WMT17): \url{https://github.com/AIPHES/emnlp19-moverscore/tree/master/examples}; BaryScore (WMT15-16): \url{https://github.com/PierreColombo/nlg_eval_via_simi_measures/tree/main/raw_score}.} 
%We re-use them to reproduce the results and compare the three evaluation metrics. 
In our reproduction experiments, we use the metrics with the configurations
%the version of each metric 
found in their evaluation scripts or papers. 
Although \citet{zhao2019moverscore} also reported the results for BERTScore-F1, they did not provide information about the used parameter settings. 
Similarly, \citet{colombo2021automatic} evaluated the other two metrics on WMT15-16, but except for the model choice, all other settings are unclear. Moreover, except for \citet{zhang2019bertscore}, who explicitly state which results were obtained using IDF-weighting, the authors of the other two approaches did not mention this in their papers. %\todo{SE: Would we not get multiple results if we use multiple githubs?} 
%Based on those facts mentioned above, we have to make some assumptions about the metric configurations. 
%\todo{SE: until here}
For the unclear metric configurations, we keep them 
%as in their own evaluation scripts
default. The configurations used here are given below:%in Appendix [...].

\begin{itemize}[topsep=2pt,itemsep=-1pt,leftmargin=*]
    \item \textbf{BERTScore}
    We report the reproduced results for BERTScore-F1 that uses 
    %with 
    BERT-base-uncased, with the default layer 9 of the BERT representation for this model, and IDF-weighting.
    
    \item \textbf{MoverScore}
     We report the reproduced results for unigram MoverScore (MoverScore-1) using BERT-base-uncased or its finetuned version on MNLI, the last five layers from BERT aggregated by power means \citep{rueckle-etal-2018-pmeans}, IDF-weighting, punctuation removal and subwords removal (only keep the first subword in each word).
    
    %We use the released version of MoverScore, which makes use of 1) BERT based uncased model finetuned on MNLI dataset and 2) the embeddings of the last five layers aggregated by power means. \citet{zhao2019moverscore} used IDF-weighting, punctuation removal, and the first subword of each word for both tasks. 
    \item \textbf{BaryScore}
    We report the reproduced results for BaryScore\footnote{BaryScore outputs scores relying on Wasserstein distance and those relying on Sinkhorn distance \citep{cuturi2013sinkhorn} together. We report the results for Wasserstein distance, which are denoted as BaryScore-W or Bary-W.} that makes use of BERT-base-uncased or its finetuned version on MNLI, the last five layers aggregated using Wasserstein Barycenter, and IDF-weighting.
    
\end{itemize}
The metrics with finetuned model are marked with $^{+}$ in the following.


\begin{table*}[!htb]
\centering
%\resizebox{\textwidth}{!}
{\small %
\begin{tabular}{@{}c|lcccccccc@{}}
\toprule
                            & metric       & cs-en & de-en & et-en & fi-en          & ru-en & tr-en & zh-en & avg   \\ \midrule
\multirow{3}{*}{Reproduced} 
& BaryScore-W  & 0.360 & 0.525 & 0.379 & 0.280          & 0.322 & 0.254 & \textbf{0.252} & 0.339 \\
& MoverScore-1 & 0.362 & 0.529 & 0.391 & \textbf{0.297} & 0.338 & 0.288 & 0.244 & 0.350 \\

& BERTScore-F1 & {\color[HTML]{009901} \textbf{0.376}} & {\color[HTML]{009901} \textbf{0.538}} & {\color[HTML]{009901} \textbf{0.393}} & {\color[HTML]{009901} 0.295} & {\color[HTML]{009901} \textbf{0.341}} & {\color[HTML]{009901} \textbf{0.290}} & {\color[HTML]{009901} 0.244} & {\color[HTML]{009901} \textbf{0.354}} \\ \midrule
Reported                    & BERTScore-F1 & 0.375 & 0.535 & 0.393 & 0.294          & 0.339 & 0.289 & 0.243 & 0.353 \\ \bottomrule
\end{tabular}%
}
\caption{Reproduction: Segment-level Kendall's $\tau$ on WMT18 to-English language pairs using the evaluation script provided by \citet{zhang2019bertscore}. Reported values are taken from \citet{zhang2019bertscore}. Values in green denote the reproduced results are better than the reported. Bold values refer to the best reproduced results with BERT-base-uncased model.}
\label{tab: reproduction wmt18}

\centering
%\resizebox{\textwidth}{!}{%
{\small 
\begin{tabular}{@{}c|lllllllll@{}}
\toprule
 &
  metric &
  cs-en &
  de-en &
  fi-en &
  lv-en &
  ru-en &
  tr-en &
  zh-en &
  avg \\ \midrule
\multirow{4}{*}{Reproduced} &
  BaryScore-W &
  0.651 &
  0.651 &
  0.816 &
  0.693 &
  0.695 &
  \textbf{0.746} &
  0.718 &
  0.710 \\
 &
  MoverScore-1 &
  \textbf{0.660} &
  \textbf{0.690} &
  0.806 &
  0.685 &
  \textbf{0.736} &
  0.732 &
  \textbf{0.720} &
  \textbf{0.718} \\
 &
  BERTScore-F1 &
  {\color[HTML]{FE0000} 0.655} &
  {\color[HTML]{FE0000} 0.682} &
  {\color[HTML]{009901} \textbf{0.823}*} &
  {\color[HTML]{009901} \textbf{0.713}} &
  {\color[HTML]{FE0000} 0.725} &
  {\color[HTML]{009901} 0.718} &
  {\color[HTML]{009901} 0.712} &
  {\color[HTML]{FE0000} 0.718} \\
 &
  MoverScore-1$^{+}$ &
  0.670* &
  0.708* &
  {\color[HTML]{FE0000} 0.821} &
  {\color[HTML]{FE0000}0.717*} &
  0.738* &
  0.762* &
  0.744* &
  0.737* \\ \midrule
\multirow{2}{*}{Reported} & MoverScore-1$^{+}$ & 0.670       & 0.708       & 0.835 & 0.746 & 0.738       & 0.762       & 0.744       & 0.743 \\
                          & BERTScore-F1  & 0.670 &  0.686 & 0.820 & 0.710 & 0.729 &  0.714 &  0.704 &  0.719 \\ \bottomrule
\end{tabular}%
}
\caption{Reproduction: Segment-level Pearson's $r$ on WMT17 to-English language pairs using evaluation script provided by \citet{zhao2019moverscore}. Reported results are cited from \citet{zhao2019moverscore}. $^{+}$ refers to using the finetuned BERT-based-uncased model on MNLI. Values in green/red denote the reproduced results are better/worse than the reported. Bold values refer to the best results with BERT-base-uncased model. Values with * denote the best reproduced/reported results.}
\label{tab: reproduction wmt17}


\end{table*}




% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}clllllllllllll@{}}
%\hline
\toprule
\multicolumn{1}{l|}{} &
  \multicolumn{6}{c|}{WMT15} &
  \multicolumn{7}{c}{WMT16} \\
\multicolumn{1}{l|}{} &
  metric &
  \multicolumn{1}{c}{cs-en} &
  \multicolumn{1}{c}{de-en} &
  \multicolumn{1}{c}{fi-en} &
  \multicolumn{1}{c}{ru-en} &
  \multicolumn{1}{c|}{avg} &
  \multicolumn{1}{c}{cs-en} &
  \multicolumn{1}{c}{de-en} &
  \multicolumn{1}{c}{ru-en} &
  \multicolumn{1}{c}{fi-en} &
  \multicolumn{1}{c}{ro-en} &
  \multicolumn{1}{c}{tr-en} &
  \multicolumn{1}{c}{avg} \\ \midrule
\multicolumn{1}{c|}{} &
  BERT-F &
  {\color[HTML]{009901} \textbf{0.750}} &
  {\color[HTML]{009901} 0.733} &
  {\color[HTML]{009901} 0.752} &
  {\color[HTML]{009901} \textbf{0.745}} &
  \multicolumn{1}{l|}{{\color[HTML]{009901} 0.745}} &
  {\color[HTML]{009901} \textbf{0.747}} &
  {\color[HTML]{FE0000} 0.640} &
  {\color[HTML]{009901} 0.672} &
  {\color[HTML]{009901} 0.661} &
  {\color[HTML]{009901} \textbf{0.723}} &
  {\color[HTML]{FE0000} 0.688} &
  {\color[HTML]{009901} 0.689} \\
  \multicolumn{1}{c|}{} 
 &
  Mover-1 &
  {\color[HTML]{009901} 0.734} &
  {\color[HTML]{009901} 0.731} &
  {\color[HTML]{009901} 0.743} &
  {\color[HTML]{009901} 0.731} &
  \multicolumn{1}{l|}{{\color[HTML]{009901} 0.735}} &
  {\color[HTML]{009901} 0.740} &
  {\color[HTML]{009901} 0.633} &
  {\color[HTML]{009901} \textbf{0.676}} &
  {\color[HTML]{009901} 0.655} &
  {\color[HTML]{009901} 0.714} &
  {\color[HTML]{009901} 0.693} &
  {\color[HTML]{009901} 0.685} \\
  \multicolumn{1}{c|}{} 
 &
  Bary-W &
  {\color[HTML]{009901} 0.751} &
  {\color[HTML]{FE0000} \textbf{0.731}} &
  {\color[HTML]{009901} \textbf{0.769}} &
  {\color[HTML]{FE0000} 0.740} &
  \multicolumn{1}{l|}{{\color[HTML]{009901} \textbf{0.748}}} &
  {\color[HTML]{FE0000} 0.735} &
  {\color[HTML]{009901} \textbf{0.672}} &
  {\color[HTML]{FE0000} 0.659} &
  {\color[HTML]{009901} \textbf{0.673}} &
  {\color[HTML]{FE0000} 0.715} &
  {\color[HTML]{009901} \textbf{0.709}} &
  {\color[HTML]{009901} \textbf{0.694}} \\
  \multicolumn{1}{c|}{} 
 &
  Mover-1$^{+}$ &
  {\color[HTML]{009901} 0.745} &
  {\color[HTML]{009901} 0.755*} &
  {\color[HTML]{009901} 0.774} &
  {\color[HTML]{009901} 0.765*} &
  \multicolumn{1}{l|}{{\color[HTML]{009901} 0.760}} &
  {\color[HTML]{009901} 0.765*} &
  {\color[HTML]{009901} 0.676} &
  {\color[HTML]{009901} 0.696*} &
  {\color[HTML]{009901} 0.707*} &
  {\color[HTML]{009901} 0.742*} &
  {\color[HTML]{009901} 0.736} &
  {\color[HTML]{009901} 0.720*} \\
\multicolumn{1}{c|}{\multirow{-5}{*}{Reproduced}} &
  Bary-W$^{+}$ &
  {\color[HTML]{FE0000} 0.753*} &
  {\color[HTML]{FE0000} 0.755} &
  {\color[HTML]{FE0000} 0.787*} &
  {\color[HTML]{FE0000} 0.763} &
  \multicolumn{1}{l|}{{\color[HTML]{FE0000} 0.764*}} &
  {\color[HTML]{FE0000} 0.758} &
  {\color[HTML]{009901} 0.700*} &
  {\color[HTML]{FE0000} 0.677} &
  {\color[HTML]{009901} 0.706} &
  {\color[HTML]{FE0000} 0.732} &
  {\color[HTML]{009901} 0.744*} &
  {\color[HTML]{FE0000} 0.720} \\ \midrule
  \multicolumn{1}{c|}{} 
 &
  BERT-F &
  \textbf{0.743} &
  0.722 &
  0.747 &
  \textbf{0.740} &
  \multicolumn{1}{l|}{0.738} &
  0.741 &
  \textbf{0.653} &
  0.651 &
  0.654 &
  0.702 &
  \textbf{0.707} &
  0.685 \\
  \multicolumn{1}{c|}{} 
 &
  Mover &
  0.688 &
  0.718 &
  0.700 &
  0.686 &
   \multicolumn{1}{l|}{0.698} &
  0.674 &
  0.609 &
  0.644 &
  0.631 &
  0.642 &
  0.661 &
  0.644 \\
  \multicolumn{1}{c|}{}
 &
  Bary &
  0.742 &
  \textbf{0.741} &
  \textbf{0.766} &
  0.737 &
   \multicolumn{1}{l|}{\textbf{0.747}} &
  \textbf{0.742} &
  0.646 &
  \textbf{0.675} &
  \textbf{0.671} &
  \textbf{0.725} &
  0.693 &
  \textbf{0.692} \\
  \multicolumn{1}{c|}{}
 &
  Mover$^{+}$ &
  0.710 &
  0.711 &
  0.722 &
  0.673 &
  \multicolumn{1}{l|}{0.704} &
  0.707 &
  0.624 &
  0.640 &
  0.645 &
  0.664 &
  0.663 &
  0.657 \\
\multicolumn{1}{c|}{\multirow{-5}{*}{Reported}} &
  Bary$^{+}$ &
  0.759* &
  0.758* &
  0.799* &
  0.776* &
  \multicolumn{1}{l|}{0.773*} &
  0.766* &
  0.685* &
  0.694* &
  0.702* &
  0.743* &
  0.738* &
  0.721* \\ \bottomrule
\end{tabular}%
}
\caption{Reproduction: Segment-level Pearson's r on WMT15-16 using evaluation script provided by \citet{colombo2021automatic}. Reported values are cited from \citet{colombo2021automatic}. $^{+}$ represents using the fine-tuned BERT-base-uncased model on MNLI. Values in green/red denote the reproduced results are better/worse than the reported. Bold values refer to the best results with BERT-base-uncased model. Values with * denote the best reproduced/reported results.}
\label{tab: reproduction wmt1516}
\end{table*}


\paragraph{Results}
As Table \ref{tab: reproduction wmt18} %\todo{YC: I'm considering using color signals in the reproduction tables. E.g., green denotes the reproduced results are better than the reported and red denotes they are worse. SE: ok}
shows, we do not obtain identical results for BERTScore-F1 with \citet{zhang2019bertscore} on \textbf{WMT18} to-English language pairs. %However, %, all reproduced values are higher than or equal to the reported, with an average deviation 0.001.
%\todo{SE: @Yaran, please check the spacing carefully as well as capitalization at the beginning of sentences} 
The maximal deviation between the reported and reproduced results can be seen on the evaluated data for 
%are on 
de-en -- around 0.003 absolute Pearson's $r$. %\todo{SE: let's discuss this: absolute Pearson} 
Most of the deviations are about 0.001. 
This might be because of tiny differences in rounding strategies, framework versions, etc.
Further, among the three evaluation metrics, BERTScore-F1 performs best, whereas BaryScore is worst. %\se{making BaryScore the worst-performing metric, contrary to the claims in the original paper}. %This observation contrasts with \citet{zhao2019moverscore} and \citet{colombo2021automatic}.

%Except that, all difference are smaller than 0.001 Pearson's $r$. 

Table \ref{tab: reproduction wmt17} displays the reproduction results on \textbf{WMT17} to-English language pairs, leveraging the resources from \citet{zhao2019moverscore}. As for MoverScore-1$^{+}$, 5 out of 7 values can be perfectly reproduced (excluding the average value). The unreproducible results on fi-en and lv-en are 0.012 and 0.031 lower than the reported, %\todo{SE: 1.2 and 3.1 points lower?} 
respectively. \se{On personal communication, the authors told us that they changed the preprocessing for these settings, which is impossible to identify from the released paper or code}. %\todo{SE: impossible to identify is true, right?}
%Next, despite %we 
We obtain comparable average value for BERTScore-F1 with \citet{zhao2019moverscore} (0.718 vs.\ 0.719), %we cannot reproduce %of 
%the results of any single language pair. 
but the results on individual language pairs differ. %\todo{SE: code from BERTSCore github?} 
%\todo{SE: from the resources on the MoverScore repro? YC: yes} %According to the reproduced results, 
%Nevertheless, 
Except for fi-en, MoverScore-1$^{+}$ correlates better with humans than BERTScore-F1, which is in line with the observation from \citet{zhao2019moverscore}. When applying the same BERT model, BaryScore performs slightly worse than the other two metrics, %MoverSocre-1 and BERTScore-F1 alternate as the best measure among the three metrics on different language pairs 
except for tr-en. %where BaryScore outperforms both of them. %\todo{SE: need to stress that BaryScore did not evaluate originally on these datasets. YC: I presented which metric was evaluated on which datasets in the setup of this part. We need stress it here?}

Table \ref{tab: reproduction wmt1516} shows the results of the reproduction attempts on \textbf{WMT15-16} based on the code and data provided by \citet{colombo2021automatic}. \citet{colombo2021automatic} reported Pearson, Spearman and Kendall correlation with human ratings; %because of the page limit, 
we relegate the reproduction results for Kendall and Spearman correlation, which are similar to those for Pearson correlation, to Section \ref{sec:repro_wmt15}. %in appendix.
%\todo{SE: can you say a sentence: are the same as what you report here? Are they entirely different?} 
We are not able to reproduce identical values for any evaluation metric, even for %the proposed approach -- 
BaryScore. However, the reproduced results for BaryScore and BaryScore$^{+}$ are comparable with the reported: around 0.001 Pearson off the reported average values in 3 out of 4 cases.
%differing by on average smaller than 0.001 Pearson's $r$. %\todo{YC: I'm not sure how to express the correlation in percent?} from those reported. 
For BERTScore-F1, the reproduced average values are around 0.005 Pearson better than the reported, while for MoverScore/MoverScore$^{+}$, they are 0.056/0.063 Pearson better. %than the reported in average.
\citet{colombo2021automatic} observed that BaryScore$^{+}$ performs best on all language pairs in WMT15-16, which is inconsistent with our observation:
%but in our reproduction attempts, 
MoverScore-1$^{+}$ outperforms BaryScore$^{+}$ on half the language pairs in these two datasets. 
%When applying 
With BERT-base-uncased, 
%\todo{SE: the above results refer to a different BERT model?} 
BaryScore performs best among the three evaluation metrics on these two datasets, however --- it achieves the highest correlation on 6 out of 10 language pairs.
%\todo{SE: Could you please give average values in the table?} %\todo{SE: sorry, I don't understand. BERT-based-uncased wasn't used above? What did the authors originally report? Btw. Average values in Table 3 would be nice YC: the metrics with + use fintuned model. They report BaryScore and MoverScore using both original and fintuned BERT-base-uncased. And I compare their performance when all using the same model. I wrote this in the setup for this part.}

%\todo{SE: do I understand correctly that on WMT15-16 when you reproduce MoverScore you use the code that the BaryScore people use?}

%Summary: \todo{YC: not finished yet}
%In summary, %it is hard to 
\paragraph{Summary}
We can rarely reconstruct identical values but %it is possible to 
obtained comparable results for the three discussed metrics, even when some of the metric configurations are missing. %as long as the authors provide the code and data. 
However, we can overall not reproduce the \emph{conclusions} for three main reasons: (i) authors report lower scores for competitor metrics; %(which makes their own approaches look better); 
(ii) authors selectively evaluate on specific datasets (maybe omitting those for which their metrics do not perform well?); (iii) unlike the authors of BERTScore, the authors of BaryScore and MoverScore do not provide a unique hash, %\todo{SE: what's that? YC: a string contains the parameter settings of BERTScore. Here I originally mean BERTScore has this function to easily document its parameter settings, but the authors of MoverScore and BaryScore did not report it when reporting BERTScore.} 
making reproduction of the original values more difficult; (iv) undocumented preprocessing involved. 

\iffalse
In contrast, the reproduced results for %other 
compared metrics can vastly differ from the reported ones, which %should be 
is 
responsible for our non-reproducibility of the conclusions.
%\todo{SE: authors could copy and paste previous results? But I think the BaryScore authors evaluated on totally new datasets, right? YC: yes.} 
%Despite that 
Further,
%we can not find a legitimate motivation of that the authors of the new metrics use distinct dataset 
on the datasets the authors used, most observations can be reproduced, whereas on other datasets, the observations are often against the authors' claims. 
This can cast doubt on their motivation of the dataset selection. 
While BERTScore %enables producing 
provides a unique hash to overcome the difficulty in reproducibility,
%\todo{SE: what kind of hash is this?} 
both \citet{zhao2019moverscore} and \citet{colombo2021automatic} did not %report 
\se{provide} it.
\fi

%there is no reason for that the authors choose another dataset to evaluate their new metric, when they intend to compare it with others. 
Following the three reproduction attempts, we cannot conclude that the newer approaches are better than the prior ones (BertScore), %in scoring algorithm 
as \citet{zhao2019moverscore} and \citet{colombo2021automatic} claim. 
\se{We also point out that the three metrics perform very similar when using the same underlying BERT model; using a BERT model fine-tuned on NLI seems to have a bigger impact. This casts some doubt on whether the more complicated word alignments (as used in BaryScore and MoverScore) really have a critical effect.}
%\todo{YC: BaryScore also performs worse than MoverScore on WMT17-18. So `prior ones' should also include MoverScore?}
%We can even conclude that the most recent metric (BaryScore) performs worse than the earlier two when taking multiple datasets into account.\todo{YC: I guess it's better to drop this sentences? since BaryScore with pure bert model beats MoverScore on 2 out of 4 datasets?}

%\todo{SE: need to integrate a brief sentence on SentSim here...}
\paragraph{SentSim} \todo{SE: @JB: please a short paragraph here}

\subsection{Reproduction for other tasks} 

\se{In Section \ref{sec:reproduction_other}, we reproduce results for other tasks, especially summarization, image captioning and data-to-text generation, with a focus on MoverScore. We find that we can only reproduce the reported results for summarization,
%cannot reproduce the reported results, 
and our results are on average 0.1 Pearson's $r$ (-12.8\%) down %\todo{SE: absolute pearson for you is percentage points? YC: no. I mean the relative performance change from the reported. Plus ``-'' better? SE: wait. From 20\% to 22\%, there are 2pp different but 10\%. You mean 10\%?} 
for IC and 0.06 Spearman's $\rho$ (-27.8\%) down for D2T generation. A reason is that the authors of MoverScore did not release their evaluation script and we can only speculate as to their employed preprocessing steps. As long as these are not reported in the original papers or released code, claim %can be made 
regarding performance of the metrics are hard to verify.\footnote{We cannot rule out the possibility that %there were 
we made 
mistakes in our reproduction attempts (e.g., incorrect evaluation scripts or use of datasets), but the unavailability of the resources makes the detection of potential errors difficult.}} %\todo{SE: @Yanran, what do you think about this summary? YC: nice!}





==> structure/structure/6_factors.tex <==
\section{Sensitivity Analysis} %Factors Affecting Metric Scores}
\label{sec:sensitivity}
%Based on the reproduction results discussed above, BERT-based evaluation metrics suffer from the same problem as  BLEU of generating inconsistent scores when different preprocessing schemes or parameter settings are applied. 
%Hence, in this section, we discuss 
%the factors 
%the preprocessing and parameters of the reproduced metrics that affects their reproducibility. 

In the previous section, we have seen that preprocessing may play a vital role for obtaining state-of-the-art results (at least for some of the metrics). Similar to the case of BLEU \cite{post2018call}, we now examine this aspect in more detail. 

\iffalse
First, according to their evaluation scripts, 
we determine %which 
the preprocessing steps %were 
taken to achieve the results 
for BERTScore, MoverScore and BaryScore. 
%in \citet{zhang2019bertscore}, \citet{zhao2019moverscore}, and \citet{colombo2021automatic}.
%MoverScore and BERTScore 
%the papers, we inspected the evaluation scripts provided in their Github repositories\footnote{BERTScore: \url{https://github.com/Tiiiger/bert_score/tree/master/reproduce}\\MoverScore: \url{https://github.com/AIPHES/emnlp19-moverscore/tree/master/examples}}. \citet{zhao2019moverscore} released the evaluation scripts for WMT17 \citep{wmt17} (MT) and TAC2008/2009\footnote{\url{https://tac.nist.gov/}} (text summarization). \citet{zhang2019bertscore} also released that for WMT17. %The preprocessing steps are listed below:
\fi

According to the papers and evaluation scripts, 
%For 
\textbf{MoverScore} uses the following main preprocessing steps (besides those handled by BERT, given in Section \ref{sec:prep}) %, the following preprocessing steps were taken:
%\begin{itemize}
%    \item \textbf{MoverScore}
    %\begin{enumerate}
        %\item[M5.] 
        (i) \emph{Subwords Removal}: discard BERT representations of all subwords except the first.
        %\item[M6.] 
        (ii) \emph{Punctuation Removal}: discard BERT representations of punctuations.
        %\item[M7.] 
        (iii) \emph{Stopwords Removal}: discard BERT representations of stopwords (only for summarization).\footnote{In Section \ref{sec:subwords}, we describe subword removal and stopword and punctuation removal used in MoverScore.}
    %\end{enumerate}
%    \item \textbf{BERTScore}
The preprocessing steps for \textbf{BERTScore} and \textbf{BaryScore} are only related to lowercasing and tokenization, both of which are handled by BERT. %\todo{YC: BaryScore uses AutoTokenizer from transformers, which doesn't have the parameter related to lowercasing. I'll check it later if it lowercases the texts automatically.}
%    \begin{enumerate}
%        \item[B1.] \emph{Lowercasing} when using uncased BERT (handled by BERT)
%        \item[B2.] \emph{Tokenization} (handled by BERT)
%    \end{enumerate}
%\end{itemize}

We observe that 
%(i) preprocessing schemes for similar datasets can differ substantially because %of the 
%for the different metrics. %authors. 
%\citet{zhao2019moverscore} did 
(i) MoverScore uses much more preprocessing than %\citet{zhang2019bertscore} and \citet{colombo2021automatic} 
BERTScore and BaryScore 
on WMT datasets; 
%\item 
(ii) %The same 
authors 
may take different preprocessing steps for different tasks, e.g.,  
\citet{zhao2019moverscore} %took all steps but stopwords removal for MT (steps 1-6), while for summarization, they 
remove stopwords for summarization but not for MT. %but did not preprocess the input texts (steps 3-7).
    %\item 
    %(iii) BERT-based evaluation metrics may omit all preprocessing steps except those automatically performed by BERT. E.g., \citet{zhang2019bertscore} did not do any additional preprocessing for BERTScore.
    %\item 
%    (iii) Some common preprocessing techniques, including stopwords removal and punctuation removal, are still used in MoverScore (steps 6-7), but the authors choose to perform the preprocessing on BERT representations rather than the input texts.
    %\item 
%    (v) Using BERT may lead to additional preprocessing steps like subwords removal (step 5 for MoverScore). 
    %This may be motivated by speed concerns instead of performance improvement.
%\end{itemize}


%\todo{YC: maybe the introduction of the preprocessing techniques also can be dropped? (the following 3-4 paragraphs)}
\iffalse
The first two steps (M1+M2)
\emph{splitting+dedokenization} are reverse steps. With these,
redundant whitespace characters can be removed. E.g., after \emph{split+detokenize}, the sentence \emph{``I love\ \ \ \ dogs .\ ''} is converted to \emph{``I love dogs.''}. Except that, \citet{zhao2019moverscore} did not apply further preprocessing techniques to the input texts. Intuitively, extra preprocessing may reduce the context information, resulting in a biased representation, because BERT assigns each word the representation based on its context. 
\fi
%This thesis focuses 
%\todo{SE: Not sure what the logic is. Do we want to say: Steps M1-4 are minor, now let's focus on the important ones? YC: how about saying we only test different parameter settings? (stopwords and punctuation removal are controlled by parameters.) I'm not sure if we should list the steps in so detail.}

%We focus 
%on the preprocessing steps performed on BERT representations which are controlled by the parameters of MoverScore (and BERTScore), i.e., steps M5-7.\todo{SE: BaryScore?}
%In Section \ref{sec:sensitivity}, we will mainly focus on the preprocessing steps of subword removal, stopword selection and punctuation removal, not those handled by BERT. 

%The following paragraphs describe these preprocessing techniques.



%\subsection{Parameters}
%\label{section:parameters}
\paragraph{IDF-weighting}
Besides preprocessing (in a proper sense), all three considered evaluation metrics use \textbf{parameters}. 
%All the three evaluation metrics are parameterized approaches.
%Parameterization makes evaluation 
This makes them 
%metrics 
more flexible, %allowing %people 
%to adjust them depending on specific needs. However, 
%it 
but also complicates reproduction: the difference in one parameter setting can lead to reproduction failure. %In this thesis, 
We study the impact of the parameters related to %\textbf{preprocessing} as well as 
\textbf{IDF-weighting}% and \textbf{layer selection \& aggregation}
. %\footnote{In addition, MoverScore enables the selection of the embedding granularity with the parameter N-gram, leading to several variants; BaryScore and BERTScore have parameters regarding model choice and layer selection.
%%BERTScore has a parameter determining which language model to use. 
%We do not consider them in this work.} %since the details of these two parameters are well documented in their papers.} 
%The importance of preprocessing is already discussed in last section. Below are the reasons for the remaining two options:
%MoverScore have parameters associated with stopwords list, punctuation removal and subwords removal (M5-7). 
%Further, 
%\begin{enumerate}
     %\item 
    %Both 
%    \todo{YC: the introduction of IDF-weighting should also be reduced if we remove the description of the preprocessing techniques.}
%    \citet{zhang2019bertscore}, \citet{zhao2019moverscore} and \citet{colombo2021automatic} utilize \textbf{IDF-weighting} to reduce the importance of common words. 
IDF-weighting measures how critical a word is to a corpus; thus, it is corpus-dependent. The choice of corpus %selection 
may lead to deviations of metric scores. 
    %As BERT-based evaluation metrics rely on word embeddings, it is easy to incorporate word importance weighting to them. \citet{zhang2019bertscore} have shown that BERTScore benefit substantially from IDF-weighting on IC.
    %\item 
    
    %BERT generates representations of different sizes depending on its model size. E.g., embeddings with BERT base models have 12 layers, and that with BERT large models have 24 layers. It is important to \textbf{select a good layer or aggregation strategy} for BERT-based approaches \citep{peters-etal-2018-deep, reimers2019alternative}. Both \citet{zhang2019bertscore} and \citet{zhao2019moverscore} conducted layer-wise experiments for their evaluation metrics. \citet{zhao2019moverscore} also compared two aggregation algorithms: power means \citep{rücklé2018concatenated} and routing \citep{zhao2018investigating, zhao2019towards}. The released version of MoverScore leverages power means to aggregate the last 5 layers.\todo{SE: if we drop this, then maybe we merge ``parameters and preprocessing'' YC: i think so.}
    
%\end{enumerate}




%\subsection{Conclusion}
%\label{section: faclast}



%To conclude, 
%based on the discussions in Sections \ref{section:preprocessing} and %Section 
%\ref{section:parameters}, 
%we summarize the factors considered in this work in Table \ref{tab:fac}.
MoverScore is the main experiment object in the remainder. %of these sections. 
Compared to %BERTScore, 
the other metrics, %MoverScore has more parameters; 
its authors 
took more preprocessing steps to achieve the results in the paper, suggesting that it is more likely to obtain uncomparable scores across different users when using MoverScore.

==> structure/structure/6_factors_unused.tex <==
%that may affect the scores of BERT-based evaluation metrics from two perspectives as \citet{post2018call}:   
%\begin{inparaenum}[(i)]
%\item 
%(i) preprocessing %(Section \ref{section:preprocessing}) 
%and
%(ii) parameters %(Section \ref{section:parameters}), 
%\end{inparaenum}
%using MoverScore and BERTScore as examples. %Section \ref{section: faclast} summarizes the factors for which we conducted experiments further in this thesis.
%\todo{YC: I guess maybe we can only discuss the parameters in this section and only mention MoverScore uses extra preprocessing step M1-M2 in one sentence?}
 
%\subsection{Preprocessing}
%\label{section:preprocessing}


==> structure/structure/7_sensitivity_1.tex <==
We will also investigate the sensitivity of %BERT-based evaluation metrics to the factors discussed in Section \ref{sec:factors}. 
%MoverScore and 
BERTScore to the factors discussed above; %in Section \ref{sec:factors}; 
we omit BaryScore and SentSim from further consideration. %\todo{SE: SentSim is not the same as BERTScore...} as it may have similar behavior as BERTScore. %\todo{SE: SentSim} 
%The experimental setup is presented in Section \ref{set:sensitivity}, followed by the corresponding results (Section \ref{re:sensitivity}). 
%In addition, based on the experiment results, we conduct further experiments, aiming at improving the reproducibility for MoverScore (Section \ref{cleaner}).
Importantly, we move beyond English-only evaluation, as reported in the original MoverScore paper. \emph{This will estimate how much uncertainty there is from preprocessing when a user applies MoverScore to a non-English language pair, which requires new IDF corpora, new stopword lists and may have higher morphological complexity (which is related to choice of subwords).}
%We will focus on the preprocessing steps of subword removal, stopword selection and punctuation removal, not those handled by BERT. 

We use two statistics to quantify the sensitivity of the evaluation metrics. When there are only \textbf{two compared values} $a,b$, we compute 
%Absolute Different (AD) and 
Relative Difference (\texttt{RD}) to reflect the %absolute and 
relative performance variation regarding a certain parameter. %factor.\todo{SE: which factor, b?} 
%\paragraph{Relative Difference (RD)}
%\emph{Relative Difference} is the ratio of absolute difference to the reference value. 
%Since this work concerns different dimensions such as different evaluation metrics, NLG tasks, datasets, and factors, to ensure the representation of the deviations are comparable across them, it is necessary to use scaled and dimensionless statistics like RD. In this work, RD is expressed as percentage, as the formula given below:
%\begin{align*}
%\texttt{RD}(a,b)=\frac{a-b}{b}*100\% 
%\end{align*}
%where $b$ is the reference value.
When there are \textbf{more than two compared values}, we compute 
%range to directly show the maximum deviation of the values, and
Coefficient of Variation (\texttt{CV}) to reflect the extent of variability of the metric performance: 
%\paragraph{Range}
%\emph{Range} refers to the difference between the largest and smallest values of a set of data: %calculated by subtracting the sample maximum and minimum, as shown below:
%$$Range(x) = x_{max}-x_{min}$$ where $x$ is the set of data.\todo{SE: why isn't it relative?}
%\paragraph{Coefficient of Variation (CV)} 
%\emph{Coefficient of Variation} is defined as the ratio of the standard deviation to the mean. It is also a dimensionless and scaled statistics, measuring dispersion of a set of data. We report the population (or sample) \texttt{CV}:
%In this work, two kinds of CV are considered. First, if the tested cases are only a sample from all possible situations, we calculate 
%sample CV. Secondly, if the tested cases already contain all possible scenarios, we calculate population CV. The difference between them is whether sample or population standard deviation is taken into account. 
%Similar to RD, they are expressed as percentage in this work. Their formulas are given below:
%\begin{itemize}
    %\item \textbf{Population CV}
    \begin{align*}
        \texttt{RD}(a,b)=\frac{a-b}{b}*100\% 
,\quad\texttt{CV}(x) &= \frac{\sigma}{\mu}*100\% 
        \quad 
        %\intertext{where}\quad 
        %\sigma &= \sqrt{\frac{\sum {({x_{i}-\mu)}^2}  }{N} } 
    \end{align*}
    
%    \item \textbf{Sample CV}
%    
%    \begin{align*}
%        CV(x) &= \frac{s}{\overline{x}}*100\% \\
%        \intertext{where}
%        s &= \sqrt{\frac{\sum {({x_{i}-\overline{x} )}^2}  }{N-1} } 
%    \end{align*}
    
     
%\end{itemize}
where $\sigma$ is the standard devation and $\mu$ is the mean and $b$ is the reference value. 
%According to the characteristics of those statistics, 
Larger absolute values of the statistics indicate higher sensitivity of the evaluation metrics. 
%Based on the parameter of the tested factors, we use AD and RD to represent the variation regarding IDF-weighting disabling and punctuation removal, range and sample CV to quantify the sensitivity regarding changing stopwords settings and IDF-weighting, %(since we could only test some stopword lists and IDF-weighting corpora), 
%and range and %population
%CV to reflect the impact of subword selection.



%The statistics used to quantify the sensitivity are described in Section \ref{statistics}. Based on the results of reproduction experiments (details see Section \ref{re:reproduction}), 
We only consider MT and summarization evaluation in this part. 
%in order to avoid the bias from the potential incorrect evaluation scripts and ensure %my 
%results are comparable with \citet{zhao2019moverscore}. 
%As mentioned in previous sections, we mainly focus on MoverScore in this work. %, so most experiments are about it and based on monolingual evaluation which it is originally designed for. 
%Further, 
%\citet{zhao2019moverscore} only evaluated MoverScore on English data,
%As MoverScore is originally designed to evaluate NLG system outputs in English, 
%so we first investigate the sensitivity to the factors in English evaluation. 
%To begin, we inspect how sensitive the evaluation metrics are to different settings regarding stopwords in Section \ref{stopwords set}. Then we disable IDF-weighting to check whether it positively impacts the evaluation metrics or not. Given that IDF-weighting is corpus-dependent, we also inspect the sensitivity of the evaluation metrics to various IDF-weighting corpora (Section \ref{idf set}). Subsequently, since MoverScore uses a single parameter to enable discarding all subwords except the first and punctuation removal, we test their impacts together (Section \ref{sub set}). Then, we extend the former experiments to other language environment (Section \ref{compare set}), to see if the evaluation metrics behave consistently to those factors in the evaluation of different languages. 
In each experiment, we only adjust the settings of the tested factors and keep the others default   
%The default configuration of the evaluation metrics involved in these experiments are given %below:
%in the appendix 
(given in Section \ref{sec:default}). In addition to English \se{(``to-English'')}, we consider MT evaluation for other 6 languages \se{(``from-English'')}, \se{for which we use multilingual BERT}: Chinese (zh), Turkish (tr), Finnish (fi), Czech (cs), German (de), and Russian (ru). 
%We choose those languages because at least two of the tested WMT datasets contain %the 
%evaluation data for them (WMT17-19).\footnote{WMT19 does not contain evaluation data for Turkish and Czech.} 
%We report the results for MoverScore-1 and BERTScore-F1 on WMT17-19 in Section. 
%\subsection{Statistics}
%\label{statistics}


%\paragraph{Absolute Difference (AD)}
%\emph{Absolute Difference} measures the distance between two real numbers on the real line by simple subtraction. It demonstrates the variation between two numbers most intuitively. Its formula is given below: 
%$$AD(a,b)=a-b$$









\subsection{Stopwords Removal}
%\paragraph{Experimental Setup}
\label{stopwords set}
In this experiment, we consider 4 stopword settings including disabling stopwords removal and applying 3 different stopword lists for the examined languages. %According to \citet{zhao2019moverscore}, unigram and bigram MoverScore alternates as the best measure on different tasks; thus, we consider these two variants in this test. 
We obtain the stopword lists 
%for other languages 
from the resources listed in %the appendix (see 
Section \ref{sec:otherlangs}. 
%In addition, we also test the sensitivity of BERTScore-F1 to stopwords as a comparison, despite that it does originally not support this technique. 
%We denote the evaluation metrics with different stopword settings as \emph{metric name + size of stopword list}. E.g., \emph{Mover-1+326} represents unigram MoverScore applying the stopword list from SpaCy. 
%We calculate CV and range of the correlations over the 4 stopword settings for each language pair in WMT datasets.
We inspect the sensitivity of MoverScore-1, MoverScore-2 (MoverScore using bigrams) and BERTScore-F1 to stopword settings, despite that BERTScore does originally not %support this technique. 
employ stopwords. 

%The \texttt{CV} regarding stopwords is denoted as \texttt{CV$_{\text{STOP}}$}. %\todo{YC: or CV(stop) is better? and later CV(idf) and CV(sub)?} 
For English MT, we calculate \texttt{CV} of the correlations \se{with humans} over the 4 stopword settings for each language pair in the datasets, then average \texttt{CV}s over the language pairs in each dataset to obtain the average \texttt{CV} per dataset. For summarization, we calculate \texttt{CV} of the correlations over the 4 stopword settings for each criterion on each dataset. 
%We relegate the results for MoverScore-2 and BERTScore-F1 and those on system-level MT and summarization to Appendix \ref{sec:stop}.
%, as the metrics are less sensitive on them. The correlation for each setting is also included in the appendices. 
%Here, we only present the %average 
%overall 
%CVs for MoverScore-1 in segment-level MT evaluation.\todo{SE: In results, we can summarize others in 1-2 sentences} 
%in Section \ref{re:stopwords}.

\paragraph{Results}
\label{re:stopwords}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}


%This section describes the results of stopwords tests in English evaluation, following the experimental setup described in Section \ref{stopwords set}. 
%We denote the \texttt{CV} regarding stopwords as \texttt{CV$_{\text{STOP}}$}.\todo{YC: or CV(stop) is better? and later CV(idf) and CV(sub)?}
%For MT, we calculate \texttt{CV} of the correlations \se{with humans} over the 4 stopword settings for each language pair in the datasets, then we average the \texttt{CV}s over the language pairs in each dataset to obtain the average \texttt{CV} per dataset; in the end we average the \texttt{CV}s for the three datasets to get the average \texttt{CV} for each evaluation metric. For summarization, we calculate \texttt{CV} of the correlations over the 4 stopword settings for each criterion on each dataset. \todo{YC: I'm not sure if the former sentences should be put in last paragraph?}
%We relegate the results for system-level MT and summarization to Appendix \ref{sec:stop}, as the metrics are less sensitive on them. The correlation for each setting is also included in the appendices. 
%The performance of each evaluation metric with each setting on each dataset and the corresponding statistics can be found in Appendix \ref{appendix: stopwords tables}. 
%Here, we only present the average 
%overall 
%CVs for segment-level MT evaluation. 
%for MT and the CVs for 
%for segment-level MT evaluation. The results for summarization and 
%summarization, which can reflect the variations of metric performances independent of the differences in absolute correlations. 

%Table \ref{tab:cv stopwords} 
On segment-level MT, as Figure \ref{fig:stopwords} (top) shows, %those average \texttt{CV}s. 
the sensitivity changes with varying datasets and languages. 
%For English,  %evaluation, 
%MoverScore-1 behaves more consistently to stopwords on multiple datasets than for other languages; %environment; 
%its \texttt{CV}$_{\text{STOP}}$ deviate from each other least. The reason might be that the \texttt{CV}$_{\text{STOP}}$ for English is averaged over the language pairs in each dataset and consequently the impact of outliers can be reduced. In contrast, each dataset contains only one set of data for every other language. 
Most of the \texttt{CV}$_{\text{STOP}}$ are in range of 2-4\%. This leads to %0.06 to 0.11
6-11\%
absolute variation of the metric performance when the average correlation is, for example, 0.7 (95\% confidence interval). %This could be the cause of the non-reproducibility of MoverScore in other papers. E.g., our reproduced MoverScore on WMT15-16 is 0.06 absolute Pearson better than \citet{colombo2021automatic} reported (the correlations on WMT15-16 are around 0.7). 
%While this may already make a difference between 
%While stopwords can thus already have considerable impact, 
%\todo{SE: 6-11\% is a lot!!}
For some datasets and languages this is even more pronounced: for example, for Russian on WMT17, the \texttt{CV}$_{\text{STOP}}$ is above 10\%. 

\yc{%We relegate other results 
%for MoverScore-2 and BERTScore-F1 and those on system-level MT and summarization 
%to Section \ref{sec:stop} in appendix.
Among the examined metrics, 
MoverScore-2 behaves slightly more sensitively than MoverScore-1, whereas BERTScore-F1 is much more sensitive than MoverScore-1 on Chinese and English. %evaluation. 
Compared to other tasks, 
stopwords removal has the largest (but negative) impact in segment-level MT evaluation (cf.\ Section \ref{sec:stop_best}).
%compared with its impact on other tasks.
%Comparing the evaluation tasks, the metrics are most sensitive in segment-level MT evaluation, but the impact of stopwords removal are almost always negative here (details see Section \ref{sec:stop}).)
}

%for segment-level MT evaluation. 
%It can be observed that all average CVs per dataset at system-level are within 0.5\%, even including BERTScore-F1, whose average CV is up to 7.72\% at segment-level, suggesting that these evaluation metrics are much less sensitive to stopwords at system-level than at segment-level. The reason could be that system-level scores are average values, and consequently, some positive and negative deviations compensate for each other within one system. Next, when 
%When comparing BERTScore to MoverScore, BERTScore-F1 are roughly up to 4 times as sensitive as the two variants of MoverScore based on their \texttt{CV}s. On the other hand, MoverScore-2 is more sensitive than MoverScore-1; its average \texttt{CV}s per dataset are larger than MoverScore-1 except on WMT17, resulting in a +0.17 percent points absolute difference in average \texttt{CV}s over the three datasets. The reason might be that the changes in stopwords can lead to various combinations of n-grams.\todo{SE: don't understand } 
%As a result, the impact is more considerable on multiple grams than unigram.

%Figure \ref{fig:sum cv sw} shows the CVs on TAC2008-2009 datasets. Among the three types of correlations, Kendall's $\tau$ varies the most, whereas Pearson's $r$ varies the least under the same evaluation condition. In the evaluation of pyramid, these evaluation metrics are slightly more sensitive than in the evaluation of responsiveness. Next, when comparing the three evaluation metrics, similar observation to MT evaluation can be made that 1) BERTScore-F1 is most sensitive among the three evaluation metrics and 2) MoverScore-2 is more sensitive compared with MoverScore-1. 

%Besides, MoverScore is less sensitive to stopwords in summarization evaluations than in segment-level MT evaluations, since 1) the CVs for MoverScore-1 on summarization are within 0.5\%, while the minimal average CV for segment-level MT evaluation is 1.42\% (WMT19); and 2) all average CVs per WMT dataset for MoverScore-2 are about 2\% in segment-level MT evaluations whereas the maximum CV is about 1.5\% on summarization. In contrast, BERTScore-F1 does not show this characteristic unless only Pearson correlation is considered. 

%When looking at the individual correlation for each stopword setting, it can be observed that the stopword list provided by \citet{zhao2019moverscore} (153 words) and the NLTK stopword list (179 words) have the same effect. Figure \ref{fig:example stopwords} illustrates some examples of the variations of metric performance with the changes of stopwords settings. The first two line charts show the correlations of MoverScore-1 on WMT17; the third one demonstrates the correlations of both unigram and bigram MoverScore on TAC2008 dataset. It shows that the correlations are identical when using the two stopword lists in all evaluation tasks. By checking the difference in these two stopword lists, we found that the MoverScore stopword list excludes contractions from NLTK stopword list, such as \emph{wouldn't} and \emph{haven't}, which are split into smaller wordpieces by BERT's tokenizer due to the feature of subword-level tokenizers. Hence, stopwords in the form of contractions cannot influence the metric scores.

%Next, to inspect whether the evaluation metrics benefit from stopwords removal, we take a look at the best stopword settings for each evaluation task. Figure \ref{fig:sw distribution} illustrates the distribution of the best stopword settings. The rings from the inside to the outside represent MoverScore-1, MoverScore-2, and BERTScore-F1. As mentioned above, the NLTK stopword list impacts the evaluation metrics equally with the MoverScore stopword list, so there are only three settings left. we regard each language pair in WMT datasets as a test case for MT, resulting in 21 test cases (3 datasets times 7 language pairs). For summarization tasks, we regard each type of correlation as a test case for each criterion, resulting in 6 test cases (3 correlations times 2 datasets). For segment-level MT evaluation (Figure \ref{fig:sw distribution}(a)), there is only one case that the best result is achieved by removing stopwords, which takes place on MoverScore-1.
%In contrast, the best stopword lists for system-level MT evaluation can be any of the settings for all evaluation metrics (Figure \ref{fig:sw distribution}(b)). However, in about 50\% of the test cases, MoverScore still performs best when disabling stopwords removal. In pyramid evaluation (Figure \ref{fig:sw distribution}(c)), MoverScore-1 achieves the best results using the original stopword list for all test cases, whereas disabling stopwords removal is still the best choice for MoverScore-2 and BERTScore-F1. In the evaluation of responsiveness ((Figure \ref{fig:sw distribution}(d))), two cases (33.3\%) can be seen that MoverScore-1 applying the original stopword list performs best; this happens only once on MoverScore-2 (16.7\%). BERTScore-F1 never benefit from stopwords removal on all evaluation tasks. 

%The difference between the impacts of stopwords removal on MoverScore in segment-level MT and summary-level summarization evaluations may be due to the fact that summary evaluation requires greater attention to the content words. However, the CVs for MoverScore in summarization evaluations are small, suggesting the performance gain from stopwords removal is tiny. In contrast, MoverScore behaves more sensitive to stopwords in segment-level MT evaluations, but stopwords removal has negative impact here, suggesting the performance drop from stopwords removal is larger than the performance gain from stopwords removal. Hence, for the purpose of improving reproducibility, MoverScore should drop the parameter regarding stopwords removal.
%The inconsistency between the sensitivity of MoverScore and BERTScore may result from the difference in their scoring algorithms. In conclusion, it seems stopwords removal is not needed for considered BERT-based evaluation metrics; the reason could be that BERT already correctly gives those non-content words enough low attention.

\subsection{IDF-weighting}
%\paragraph{Experimental Setup}
\label{idf set}
%\todo{SE: original IDF for languages }
In this test, we first disable IDF-weighting for the evaluation metrics (idf$_{\text{dis}}$), and compare the metric performance to that when applying original IDF-weighting\footnote{The original IDF weights for MoverScore are extracted from the reference and hypothesis corpus. And those for BERTScore are computed using the reference corpus.
} (idf$_{\text{ori}}$) by calculating the \texttt{RD} between them. We denote this statistic as \texttt{RD}(dis,ori); negative values indicate idf$_{\text{ori}}$ works better and vice versa.
%With this, we can clearly know whether IDF-weighting positively impacts these evaluation metrics and how large the deviation can be resulting from this factor. 
Next, to inspect the sensitivity to varying IDF-weighting corpora, 
we apply IDF-weighting from four randomly generated corpora to the evaluation metrics additionally (idf$_{\text{rand}}$): %\todo{SE: what is idf-random? I see this is the definition, right? YC: yes} 
each corpus consists of 2k English segments randomly selected from the concatenated corpus of all tested datasets. %, namely WMT17-19 and TAC2008-2009. 
%We consider the internal corpora %first 
%because in practice, users %often 
%may select %to use 
%a certain part of the evaluated datasets as the IDF-weighting corpus. %although the selection of texts used to compute IDF-weighting fully depends on them. 
The corresponding variability of the metric performance is quantified by the \texttt{CV} of the correlations with humans over the 5 IDF-weighting corpus selections (idf$_{\text{ori}}$ + 4 idf$_{\text{rand}}$), marked with \texttt{CV}$_{\text{IDF}}$. %We use the same method to calculate 
%The \texttt{CV}$_{\text{IDF}}$ 
%%per dataset 
%for English %and for each evaluation metric 
%is calculated as in stopwords test.
We examine the sensitivity regarding IDF-weighting of MoverScore-1, MoverScore-2, and BERTScore-F1. 
Subsequently, we test the IDF-weighting from %large-domain and 
large-scale corpora (idf$_{\text{large}}$). These corpora are obtained from Hugging Face Datasets.\footnote{\url{https://huggingface.co/datasets}} They are listed in Section \ref{sec:idf_corpora}.%\todo{SE: why does this not go in CV from above?}

%Similar to stopwords, %the results for MoverScore-2 and BERTScore-F1 as well as the results on system-level MT and summarization are given in Appendix [...]. 
%we only discuss the results for MoverScore-1 on segment-level MT here and relegate other results to Appendix [...].
%we put the correlation for each setting, the corresponding statistics, and the results for system-level MT and summarization in Appendix \ref{sec:idf} and only present the scaled statistics on segment-level MT evaluation here.
%, namely RD and CV. 


%We report the results on WMT17-19 and TAC2008-2009 for MoverScore-1, MoverScore-2 and BERTScore-F1 in Section \ref{re:internal} (internal IDF-weighting). Based on the former results (details see Section \ref{re:internal} (internal IDF-weighting)), 
%Subsequently, we test the IDF-weighting from %large-domain and 
%large-scale corpora. %further, expecting it can provide more comprehensive and precise information about word importance. 
%The results are presented in Section \ref{re:external} (external IDF-weighting).
%We obtain these corpora from Hugging Face Datasets.\footnote{\url{https://huggingface.co/datasets}} They are listed in the appendix (Section \ref{sec:idf_corpora}).
%\todo{YC: the external idf part is related to improving the reproducibility of MoverScore, so maybe it also can be dropped?}

%\todo{SE: we see here averages over all to-X languages where X is en, fi, zh, etc.?}
\begin{figure*}[!htb]
    
\scalebox{0.9}{
\begin{minipage}[t]{0.55\textwidth}
\flushleft
%\centering
\includegraphics[height=0.47\textheight]{figure/MoverScore-1_cvs_seg.png}
\caption{From top to bottom: \texttt{CV}$_{\text{STOP}}$, \texttt{CV}$_{\text{IDF}}$, \texttt{CV}$_{\text{SUB}}$. WMT17-19, segment-level evaluation, MoverScore-1.}
\label{fig:stopwords}
\end{minipage}%
%
\hspace{0.5cm}
\begin{minipage}[t]{0.38\textwidth}
%\flushright
\centering
\includegraphics[height=0.47\textheight]{figure/MoverSocre-1_rds_seg.png}
\centering
\caption{\texttt{RD}(dis,ori), \texttt{RD}(dis,pr). WMT17-19, segment-level evaluation, MoverScore-1.}
\label{fig:mover1_rd_seg}
\end{minipage}%
}

%\caption{fdddd}
\end{figure*}






\iffalse

\centering
    \subfigure[From top to bottom: \texttt{CV}$_{\text{STOP}}$, \texttt{CV}$_{\text{IDF}}$, \texttt{CV}$_{\text{SUB}}$.]{\includegraphics[width=0.2\textwidth]{figure/MoverScore-1_seg.png}}\hspace{0.1cm}
    
    \subfigure[\texttt{RD}(dis,ori)]{\includegraphics[width=0.2\textwidth]{figure/MoverScore-1_seg_idf_rd.png}}
    
    \subfigure[\texttt{RD}(dis,pr)]{\includegraphics[width=0.2\textwidth]{figure/MoverScore-1_seg_pr_rd.png}}
    
    \caption{%Sensitivity to stopwords: 
    %Coefficients of variation of the correlations of MoverScore-1 applying different stopword settings with segment-level human judgements in WMT17-19 (\texttt{CV}$_{\text{STOP}}$).
    WMT17-19, segment-level evaluation, MoverScore-1.
    }
    
\begin{figure*}[!htb]
    \centering
    \includegraphics[scale=0.4]{figure/stopwords.png}\vspace{0.1cm}
    \includegraphics[%width=\textwidth
    scale=0.4]{figure/idf-corpus.png}\vspace{0.1cm}
    \includegraphics[%width=\textwidth
    scale=0.4]{figure/subwords.png}
    \caption{%Sensitivity to stopwords: 
    %Coefficients of variation of the correlations of MoverScore-1 applying different stopword settings with segment-level human judgements in WMT17-19 (\texttt{CV}$_{\text{STOP}}$).
    From top to bottom: \texttt{CV}$_{\text{STOP}}$, \texttt{CV}$_{\text{IDF}}$, \texttt{CV}$_{\text{SUB}}$. WMT17-19, segment-level evaluation, MoverScore-1.
    }
    \label{fig:stopwords}
\end{figure*}

\begin{figure*}[]
    \centering
    \includegraphics[width=\textwidth]{figure/idf-corpus.png}
    \caption{Sensitivity to IDF-weighting corpus: Coefficients of variation of the correlations of MoverScore-1 using IDF-weighting from varying corpora with segment-level human judgements in WMT17-19 (\texttt{CV}$_{\text{IDF}}$).}
    \label{fig:idf corpus}
\end{figure*}
\begin{figure*}[]
    \centering
    \includegraphics[width=\textwidth]{figure/subwords.png}
    \caption{Sensitivity to subword selection: Coefficients of variation of the correlations of MoverScore-1 applying different subword selection strategies with segment-level human judgements in WMT17-19 (\texttt{CV}$_{\text{SUB}}$).}
    \label{fig:subwords}
\end{figure*}
\fi

\paragraph{Results}\label{re:idf}
%Figure %\ref{fig:idf_dis} (appendix) 
%\ref{fig:stopwords} (middle)
%displays the results for segment-level MT.
%We first give \texttt{RD}(dis,ori) for segment-level MT %to-English language pairs 
%in Figure \ref{fig:mover1_rd_seg}(a). %Only on one language pair 
As seen in Figure \ref{fig:mover1_rd_seg}(a), 
\texttt{RD}(dis,ori) is positive on only one to-English language pair (WMT19 kk-en), %while on three 
but on three from-English language pairs (WMT17 en-de, en-zh, and en-tr). Overall, IDF-weighting is thus beneficial. 
%it has negative impact in the evaluation of German, Chinese and Turkish on WMT17.
%indicating a positive impact of IDF-weighting on MoverScore-1. %The maximal performance drop for to-English language pairs can be seen on WMT19 de-en, with over 35\%, whose reversed language pair obtain the 
The maximal performance drops %for both directions can be seen 
are on WMT19 de-en (over 35\%) and %its reversed language pair 
de-en 
(over 10\%), respectively.
%Figure \ref{fig:idf_dis}(b) shows \texttt{RD}(dis,ori) for other tested languages. 
%On WMT18-19,
%In the evaluation of other languages, 
%MoverScore-1 benefits from IDF-weighting for all languages, whereas on WMT17, IDF-weighting has negative impact in the evaluation of German, Chinese and Turkish. The maximum deviation appears on WMT19 en-de, which is just the reserved language pair where MoverScore drops most in English evaluation when disabling IDF-weighting. 
Most \texttt{RD}(dis,ori) have absolute values smaller than 5\%. This means, suppose the correlation is 0.7, the performance can fall by around 0.035 because of disabling IDF-weighting. 


%, which is much larger than the deviations on the other evaluation data. %the relative performance change on MT when disabling IDF-weighting with \texttt{RD(dis,ori)}\todo{SE: dis-ori means? disabling minus original? If you mean it in the sense of `minus' here, then you need to rewrite all variants of `idf-ori' etc. (e.g., idf$_{\text{ori}}$) Yc: rewrote.} in Figure \ref{fig:idf dis}. Negative percentage values indicate positive impacts of IDF-weighting and vice versa. Firstly, all average \texttt{RD(dis,ori)} are negative, implying a positive impact of IDF-weighting on segment-level MT evaluation tasks. 
%Further, the differences in RDs between evaluation levels suggest that these evaluation metrics benefit from IDF-weighting more at segment-level, since 1) all average RDs at system-level are within -1\%,\todo{SE: minus 1 percent?} whose absolute values are much smaller than those of the RDs at segment-level; and 2) less positive RDs$_{\text{IDF}}$\todo{SE: as above, notation is unclear to me} can be seen in segment-level evaluations (e.g., IDF-weighting impacts MoverScore negatively only once). 
%Next, among these three evaluation metrics, at segment-level, on the one hand, BERTScore-F1 is least sensitive, which %is on the contrary to 
%contrasts with 
%the observations in the stopwords tests;
%(Section \ref{re:stopwords}); 
%on the other hand, similar to the observation in the stopwords tests, bigram MoverScore is more sensitive than unigram MoverScore. 
%It is noteworthy that the maximal performance drop (WMT19 de-en)
%of MoverScore 
%is much larger than the drops on the other language pairs.\todo{SE: which other drops do you compare to? YC: I compare the maximal drop of MoverScore (de-en) to all other drops of MoverScore.}  %but this does not take place on BERTScore-F1. 
%By checking the correlations for this language pair, %namely de-en in WMT19 
%(details see Table \ref{tab:wmt19 idf} in Appendix \ref{sec:idf}), it can be seen that when using IDF-weighting, MoverScore outperforms BERTScore-F1 substantially on this evaluated data (0.22 vs. 0.15 Kendall's $\tau$), but their performances differ only slightly when disabling IDF-weighting (smaller than 0.01 Kendall's $\tau$). %On the contrary, the performances of all evaluation metrics fall most on WMT18 tr-en at system-level. 

%which is already capable of disturbing the ranking of the compared evaluation metrics and therefore leading to non-reproducibility of the conclusions. 



%Figure \ref{fig:rd idf sum} shows the RDs$_{\text{IDF}}$ on TAC2008-2009. Those values fluctuate around 0, implying that IDF-weighting does not lead to consistent improvement in summarization evaluations. However, for MoverScore, IDF-weighting still has a positive impact in most cases, and the performance drop is often larger than the enhancement due to IDF-weighting disabling, especially for bigram MoverScore. Regarding BERTScore-F1, the cases that IDF-weighting impacts it positively/negatively are fairly distributed. Among these three evaluation metrics, MoverScore-1 is least sensitive with all deviations smaller than 1\% except on TAC2009 responsiveness; bigram MoverScore is again more sensitive than unigram MoverScore; BERTScore-F1 has the in-between variations. Further, different correlations can behave the other way around, i.e., one correlation may increase while another falls under the same evaluation condition. E.g., the Pearson correlation of MoverScore-2 rises when disabling IDF-weighting in responsiveness evaluation on TAC2009, whereas the other two correlations descend.


%\begin{table}[h]
%\centering
%\resizebox{\columnwidth}{!}{%
%\begin{tabular}{@{}lcccc@{}}
%\toprule
%metric  & WMT17-$r$ & WMT18-$\tau$ & WMT19-$\tau$ & AVG    \\ \midrule
%Mover-1 & 0.13\%  & 0.67\%    & 2.56\%    & 1.12\% \\
%Mover-2 & 0.78\%  & 1.19\%    & 3.84\%    & 1.94\% \\
%BERT-F1 & 0.20\%  & 0.32\%    & 0.41\%    & 0.31\%   \\ \bottomrule
%\end{tabular}%
%}
%\caption{Sensitivity to IDF-weighting corpus: Average coefficients of variation of the %correlations with segment-level human judgements on WMT17-19 to-English language %pairs.}
%\label{tab: idf corpus}
%\end{table}


Next, \texttt{CV}$_{\text{IDF}}$ for segment-level MT is presented in Figure \ref{fig:stopwords} (middle). %\ref{fig:idf corpus}. %displays \texttt{CV}$_{\text{IDF}}$. %\todo{SE: meaning? YC: added in last paragraph.} 
%For all languages in WMT19, MoverScore-1 behaves most sensitively on WMT19 among the three datasets. 
In English evaluation, the maximal variation is also caused by the result for de-en in WMT19, where idf$_{\text{ori}}$ yields considerably better result than idf$_{\text{rand}}$ (0.22 vs. 0.17 Kendall's $\tau$). 
%The maximal \texttt{CV$_{\text{IDF}}$} among all tested languages and datasets can be observed again on the reserve language pair where maximal \texttt{CV$_{\text{IDF}}$} for English exists. 
While en-de has \texttt{CV} values above 4.5\%, 
most \texttt{CV}$_{\text{IDF}}$ are smaller than 1\%. %When correlation is 0.7, varying IDF-weighting corpus can result in 0.028 absolute variation (95\% confidence interval), which also can be responsible for the non-reproducibility of MoverScore.

\yc{
BERTScore-F1 is less sensitive to IDF-weighting than both MoverScore variants. Among the evaluation tasks, the metrics are again most sensitive on segment-level MT, where for English, 
%For MoverScore, 
idf$_{\text{ori}}$ works best for MoverScore (even idf$_{\text{large}}$ cannot %provide more applicable IDF weights for it),
improve its performance), 
while %for BERTScore-F1,
idf$_{\text{rand}}$ and idf$_{\text{ori}}$ are almost equally effective for BERTScore-F1 (cf. Section \ref{sec:idf}).} 
%On the contrary, the effectiveness of IDF-weighting for other languages are less stable.}
%All CVs are smaller than 1\% except those in segment-level MT evaluations, suggesting that the selection of IDF-weighting corpora impacts the metric performance slightly. 
%The maximum variation of MoverScore can be seen on WMT19, which is also caused by the results for de-en; MoverScore with idf$_{\text{ori}}$ outperforms it with idf$_{\text{rand}}$ substantially here (0.22 vs. 0.17 Kendall's $\tau$ for MoverScore-1; 0.22 vs. 0.15 for MoverScore-2).\todo{SE: same numbers as above?} %Similar to stopwords, it can be observed that Kendall is most sensitive among the three correlations, whereas Pearson is least sensitive. 
%When comparing the three evaluation metrics at segment-level, BERTScore-F1 is the least sensitive one, and bigram MoverScore is more sensitive than unigram MoverScore, which is in line with the previous observations (IDF-weighting disabling tests). This may be %due to that 
%because 
%BERTScore originally only uses the references to compute IDF-weighting, whereas MoverScore computes IDF-weighting for references and hypotheses separately. %thus, the actual variations of IDF-weighting of BERTScore is smaller than those of MoverScore. 


%To investigate whether idf$_{\text{rand}}$ also positively impacts the evaluation metrics, we calculate RDs(random-dis), which denote the relative performance change from disabling IDF-weighting to applying idf$_{\text{rand}}$. 
%In this test, only segment-level MT evaluation is concerned since those evaluation metrics behave most sensitively to IDF-weighting in this evaluation. There are 84 test cases because 4 idf$_{\text{rand}}$ are applied to each language pair. The middle column of Figure \ref{fig:idf rd wmt seg} shows these values. The average RDs(random-dis) for all evaluation metrics are positive, suggesting a positive impact of idf$_{\text{rand}}$. Subsequently, we calculate RDs(random-ori), representing the performance change from using idf$_{\text{ori}}$ to idf$_{\text{rand}}$. The right column of Figure \ref{fig:idf rd wmt seg} shows these values. It can be seen that BERTScore-F1 performs even a little better with idf$_{\text{rand}}$, shown with a positive average RD(random-ori) +0.05\%. However, those values fluctuate around 0; therefore, we would only say that idf$_{\text{rand}}$ and idf$_{\text{ori}}$ are equally effective to BERTScore-F1. As for MoverScore, in the majority of the cases, idf$_{\text{ori}}$ still works better. Further, the extrema in the figures for MoverScore can be seen at the same position (red box), which denotes the results for de-en in WMT19. The cause is, as mentioned before, idf$_{\text{ori}}$ leads to a substantial performance enhancement to MoverScore on this evaluation data.



%We can conclude that IDF-weighting positively impacts BERT-based evaluation metrics in English evaluations, regardless of where it originates. However, original IDF-weighting still works best for MoverScore. Based on the results, we test IDF-weighting from large-domain and large-scale corpora, expecting it can provide more comprehensive information about the word importance, since original IDF-weighting is computed using only 1000-3000 documents. 


%\paragraph{External IDF-weighting}
%\label{re:external}


%Table \ref{tab:external en} presents the results for external IDF-weighting test in English evaluation. First, the size of those corpora is much larger than the original corpora  but MoverScore still performs better with original IDF-weighting. Secondly, the results for Wikipedia shows that the metric performance does not enhance with the increasing size of corpora. Thirdly, although those corpora contain articles in many domains, they do not provide more applicable IDF-weighting neither. In conclusion, no IDF-weighting from large-domain and large-scale works as well as the original IDF-weighting in English evaluation.


\subsection{Subwords \& Punctuation}
%\paragraph{Experimental Setup}
%\label{sub set}

In this experiment, we evaluate the sensitivity % of MoverScore-1%\todo{SE: why MoverScore-1? This looks a bit random; sometimes MoverScore, sometimes M-1, sometimes M-1 and M-2} 
to different subword selection and punctuation removal (PR). We measure the performance change from using to disabling PR by calculating the \texttt{RD} between them, which we denote as %We denote this statistic as 
\texttt{RD}(dis,pr); negative values indicate MoverScore with PR performs better and vice versa. In addition to the original two selections of subwords (keeping the first subword and keeping all subwords), 
%There are originally two selections of subwords: keeping the first subword and keeping all subwords. In addition, 
we also %implement another technique, i.e., to 
average the embeddings of the subwords in a word to get the word-level BERT representations. %This leads to 6 configurations together with PR: 1) first, 2) all, 3) ave-all, 4) first+PR, 5) all+PR, and 6) ave-all+PR. 
To quantify the sensitivity to subword selection, we calculate \texttt{CV} of the correlations with humans over the 3 subword selections, denoted as \texttt{CV}$_{\text{SUB}}$. We inspect the corresponding sensitivity of MoverScore-1.
%The \texttt{CV}$_{\text{SUB}}$ for English is derived using the same method as in stopwords test.\todo{SE: ??? for other languages?? drop this sentence?}
%In addition, we calculate the \texttt{CV} of the correlations over the whole 6 configuations (\texttt{CV}$_{\text{PR+SUB}}$), as MoverScore uses one single parameter to control both of the aspects.
%We report the results on WMT17-19 and TAC2008-2009 for MoverScore-1.% in Section \ref{re:sub}. 
%We also relegate the results on system-level MT and summarization to Appendix [...] and only present the results on segment-level MT here.


%\begin{figure}[h]
%    \centering
%    
%    \includegraphics[width=\columnwidth]{figure/seg punc en.png}
%    \caption{Sensitivity to punctuation removal: Relative differences [...]}
%    \label{fig:punc en}
%\end{figure}



\paragraph{Results}%\todo{YC: not modified yet.}
\label{re:sub}
%This sections presents the experiment results for subword selection and punctuation removal in English evaluation, following the experiment setup described in Section \ref{sub set}. 
%To begin, %we present the results for segment-level MT.
%We show \texttt{RD}(dis,pr) for segment-level MT % for to-English language pairs 
%the relative performance change from removing to keeping punctuations in MT evaluations 
%In Figure \ref{fig:mover1_rd_seg}(b), %in the appendix. %with \texttt{RD}(dis,pr).\todo{SE: notation? } Positive values indicate positive impacts of PR. %Firstly, it can be also observed that the evaluation metrics are more sensitive at segment-level than system-level. Secondly, 
%Despite the average \texttt{RD}(dis,pr) %at both evaluation levels 
%being negative, the values fluctuate around 0, so the effectiveness of PR in MT evaluations cannot be confirmed. Most \textt{RD}(dis,pr) have absolute values smaller than 1\%, indicating a smaller impact of PR compared with IDF-weighting.  
%PR negatively impacts MoverScore-1 in 5 of 21 test cases in English evaluation. %indicating a positive impact of PR on MoverScore in English evaluation. 
%In contrast, on about half of the from-English language pairs, PR negatively impacts MoverScore-1.%, shown in Figure \ref{fig:pr_dis}(b).
%As the authors of MoverScore only reported the results on English data, they may thus select 
%only consider 
%an optimal preprocessing strategy only for that case. %chasing for a higher reported performance. 
Figure \ref{fig:mover1_rd_seg}(b) shows that 
most \texttt{RD}(dis,pr) have absolute values smaller than 1\%, while both values for en-tr are over 3\%.
%Next, RDs(keep) on TAC2008-2009 are visualized in Figure \ref{fig:punc rd wmt}(b). It also shows that the contribution of PR is unstable. MoverScore-1 performs even better when keeping punctuations on responsiveness. However, the deviations are within 0.6\%, implying a low sensitivity of MoverScore to punctuations in summarization evaluations. The three correlations behave again inconsistently on TAC2009 pyramid, where the Pearson correlation drops a bit while the other two rise when keeping punctuations. Similar observation has been made in IDF-weighting disabling tests discussed in Section \ref{re:idf}. 
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
%\begin{table}[h]
%\centering
%\resizebox{\columnwidth}{!}{%
%\begin{tabular}{@{}lcccc@{}}
%\toprule
%   & WMT17-$r$ & WMT18-$\tau$ & WMT19-$\tau$ & AVG    \\ \midrule
%CV$_{\text{SUB}}$    & 1.94\%  & 1.48\%    & 1.38\%    & 1.60\% \\
%CV$_{\text{PR+SUB}}$ & 1.58\%  & 1.36\%    & 1.18\%    & 1.37\% \\ \bottomrule
%\end{tabular}%
%}
%\caption{Sensitivity to subword selection and punctuation removal: Average coefficients of variation of the correlations of MoverScore-1 with segment-level human judgements on WMT17-19 to-English language pairs.}
%\label{tab: cv ss pr}
%\end{table}
Further, the
%the variation of metric performance regarding subword selection on WMT17-19 
\texttt{CV}$_{\text{SUB}}$ for segment-level MT is presented
in Figure \ref{fig:stopwords} (bottom). %\ref{fig:subwords}. 
%\ref{tab: cv ss pr}. %Again MoverScore is more sensitive at segment-level than at system-level. 
%The metric performance again varies most at segment-level on WMT19 de-en. % and at system-level on WMT18 tr-en
%; the largest deviations from changing IDF-weighting also take place on this evaluation data.
%these two language pairs. %This may suggest that the evaluation data itself is also a determinant of reproducibility for evaluation metrics. 
%The average \texttt{CV}$_{\text{SUB}}$ for segment-level evaluation (1.6\%) indicates a similar level of sensitivity of MoverScore to subwords, stopwords and IDF-weighting (the average \texttt{CV$_{\text{STOP}}$} 
%for stopwords and IDF-weighting 
%and \texttt{CV$_{\text{IDF}}$} are 1.87\% and 1.12\%, respectively).
The average \texttt{CV}$_{\text{SUB}}$ over all datasets for most languages are smaller than 2\%, whereas 
highly inflectional languages such as Turkish and Russian are considerably more sensitive, with average values over 4\%. 


\yc{%The remaining results are given in Section \ref{sec:sub} in the appendix. 
Similar as %to the observation in 
for stopwords and IDF weighting, %experiments, 
MoverScore-1 behaves most sensitively on segment-level MT, where the default configuration of PR and subwords, which uses the first subword and removes punctuations, works %more 
%consistently 
best for English. However, for other languages, only in 2 out of 16 cases is it best to select the default configuration (cf. Section \ref{sec:sub_best}). As the authors of MoverScore only reported the results on English data, they may thus select 
%only consider 
an optimal preprocessing strategy only for that case.
%not only leveraging the first subword yield better results, no matter averaging or not, with or without PR. 
%yields the best results for English. 
}

%\todo{SE: which subword setting is best? which stopword setting is best? which idf weighting is best? Maybe just give a brief sentence}
%Next, the CVs on TAC2008-2009 are shown in \ref{fig:sub rd wmt}(b). Except the Kendall correlation on TAC2008 pyramid, all CVs are within 1\%, implying the insensitivity of MoverScore to subword selection in summarization evalautions. And the three correlations in descending order of sensitivity are again Kendall, Spearman, and Pearson. 

%To investigate which configuration of subword selection and punctuation removal in combination is optimal, we show the number of times that each configuration works best in Figure \ref{fig:sub punc best}. we mark the default setting \emph{first+PR} with $*$. On the most sensitive task, namely segment-level MT evaluation, MoverScore-1 achieves the best performance applying the original setting in 12 out of 21 cases. In system-level MT evaluations, using all subwords and punctuation removal is the best choice (9/21). As for summarization, there is no explicit clue about which is the best configuration. Considering that MoverScore-1 is most sensitive in segment-level MT evaluations, keeping the original setting is the best choice for now. 



%\subsection{Comparison among Evaluated Languages}%\todo{YC: I'm not sure if we should write an independent part for other languages or we could merge them into the former sections?}
%\paragraph{Experimental Setup}
%\label{compare set}
%In this test, we compare the sensitivity of the evaluation metrics across different language environment by extending the former experiments to 
%the monolingual evaluation for other 6 languages: Chinese (zh), Turkish (tr), Finnish (fi), Czech (cs), German (de), and Russian (ru).

%We choose those languages because at least two WMT datasets contain %the 
%evaluation data for them. %in the question language. 
%making a comparison across datasets possible and thus preventing drawing conclusions from results generated by chance. 
%We obtain the stopword lists for other languages from the resources listed in the appendix (see Section \ref{sec:otherlangs}).  


%We report the results for MoverScore-1 and BERTScore-F1 on WMT17-19 in Section \ref{re:compare}.
%\todo{SE: It would generally be better to give results for each setting right away, to decrease cognitive load for the reader}

%\paragraph{Results}
%\label{re:compare}
%This section compares the sensitivities of MoverScore-1 and BERTScore-F1 in MT evaluation across different languages, following the experiment setup described in Section \ref{compare set}. The main purpose of this section is to answer the following two questions: 1) \emph{Is the sensitivity of BERT-based evaluation metrics similar across different evaluation languages?}; and 2) \emph{Do positive/negative factors still positively/negatively affect BERT-based evaluation metrics for other languages?}.

%\textbf{Q1: Is the sensitivity of BERT-based evaluation metrics similar across different evaluation languages?}

%To examine how large impact the factors have in the evaluation of other languages, 
%We calculate the average statistics over WMT17-19 for all tested languages. Figure \ref{fig:all} demonstrates the results. The evaluation metrics behave more sensitive at segment-level than at system-level for all languages, which is consistent with English evaluation. Almost all values for system-level evaluation are within 1\%. The exception is Turkish, whose \texttt{CV}-subwords of MoverScore-1 and \texttt{RD}-idf of BERTScore-F1 have absolute values over 1\%. The performance of BERTScore-F1 even drops more at system-level than at segment-level when disabling IDF-weighting (-2.58\% vs.\ -1.21\%). Furthermore, it is interesting that at system-level, MoverScore-1 behaves most sensitively in Turkish evaluation to all factors except punctuation removal. %Overall, at system-level, those factors have only tiny impacts on BERT-based evaluation metrics, so 
%We discuss the similarity and dissimilarity of sensitivity across different languages in segment-level evaluation further in the following paragraphs. 



%\textbf{MoverScore-1}: Russian is most sensitive to \textbf{stopwords}; its \texttt{CV}-stopwords is 3.62 percent points higher than that of English. Chinese and Turkish are slightly less sensitive than English with a absolute deviation of \texttt{CV}s-stopwords within 0.3 percent points. German and Turkish are more sensitive to \textbf{IDF-weighting} than English, and only the \texttt{CV}s-idf of these three languages are over 1 percent points. However, the deviations of \texttt{CV}s-idf of all languages to the \texttt{CV}-idf of English are within 1 percent point, so there is no considerable difference in the sensitivity to IDF-weighting across different languages. Next, except for Turkish, all other RDs-idf are negative, indicating a positive impact of IDF-weighting to some extent, but it should be noted that the contribution of IDF-weighting can not be confirmed only by an average \texttt{RD}, since negative and positive \texttt{RD}s can compensate for each other in multiple datasets. Hence, we also show the \texttt{RD}-idf for each dataset later, to investigate whether MoverScore truely benefits from IDF-weighting in the evaluation of other languages.  As for \textbf{subwords}, German and Chinese show a lower sensitivity than English. The \texttt{CV}-subwords of Chinese is even smaller than 1\%. The reason might be that Chinese is a character-based language,  and after the tokenization by multilingual BERT, there are rarely wordpieces with ``\#\#''. %As a result, the selection of subwords won’t affect MoverScore in Chinese evaluation too much. 
%The \texttt{CV}s-subwords of Russian and Turkish are about 2.5 percent points higher than that of English, suggesting MoverScore is more sensitive to subwords in the evaluation of these two languages. Except these, all deviations of \texttt{CV}s-subwords of other languages to that of English are whithin 1 percent point. Further, all \texttt{RD}s-punctuation are within 1\% except for Chinese, suggesting a low sensitivity of MoverScore to \textbf{punctuation removal}. %There is no explanation for the fact that Chinese is according to my test more sensitive to punctuation removal than other languages, since Chinese punctuation uses a completely different set of punctuation marks from other languages, and in my tests, only the default set punctuations in Python are removed, which does not contain any Chinese punctuation. 
%The reason could be that some of the system translations contains western punctuations by mistake. Similar to IDF-weighting disabling tests, it can not be simply determined with an average \texttt{RD} whether punctuation removal has a positive impact, so we also discuss this later\todo{SE: later?} in more details. 



%\textbf{BERTScore-F1}: For \textbf{stopwords}, only the deviation of \texttt{CV}-stopwords of Chinese to that of English is within 1 percent point, suggesting the sensitivity of BERTScore-F1 to stopwords is similar in the evaluation of these two languages. Chinese and English are also most sensitive compared with other languages, whereas Finnish is least sensitive. Regarding \textbf{IDF-weighting}, BERTScore-F1 is insensitive for all languages except for Turkish; its \texttt{CV} is close to 2\% whereas the others are within 0.31\%. Further, the effectiveness of IDF-weighting seems unstable across different languages. Similar to MoverScore-1, we show the \texttt{RD}s-idf on each dataset later. 


%\paragraph{Between MoverScore and BERTScore} Although the behavior of each language to each factor are different across these two evaluation metrics, there %is still something in common: 
%are still common findings: 

%\begin{itemize}


    %\item Both evaluation metrics have the same ranking of the magnitudes of the effects of IDF-weighting and stopwords for each language. They are more sensitive to stopwords than to IDF-weighting with the only exception that MoverScore behaves more sensitively to IDF-weighting in the evaluation of Turkish.
    %On MoverScore, subword selection has the second largest impact. The exceptions is German, which behaves least sensitive to subwords.
    
    
    %\item Interestingly, %as the matter of fact, 
    %English and Chinese have almost synchronized behavior to stopwords; although the results on both languages show big difference between the two evaluation metrics regarding stopwords, the \texttt{CV}-stopwords of these two languages remain closest. Further, for some languages, such as German, Czech, and Finnish, the difference is less pronounced (absolute deviation of \texttt{CV}s within one percent point).
    
    
    %\item Both evaluation metrics behave most sensitively to IDF-weighting in the evaluation of Turkish compared with other languages.
    
%\end{itemize}


%\subsubsubsection{Q2: Do positive/negative factors still positively/negatively affect BERT-based evaluation metrics for other languages?}

%\paragraph{Stopwords Removal}

%Table \ref{tab:sw distribution} displays the best stopword setting for each language in segment-level MT evaluations. Except Finnish and Turkish, disabling stopwords removal is always the best choice for all other languages. For Finnish, only on one dataset, MoverScore-1 performs better using stopwords removal, whereas, for Turkish, both evaluation metrics achieve the best performance applying the same stopword lists. The reason might be that both Turkish and Finnish belong to agglutinative languages, and those languages tend to have a high rate of affixes or morphemes per word, which means there may exist more noise in word embeddings. In summary, \emph{for most languages, BERT-based evaluation metrics do not benefit from stopwords removal, which is consistent with English evaluation}.






%\paragraph{IDF-weighting}

%Figure \ref{fig:idf rd all languages} shows the relative performance change from using the original to disabling IDF-weighting for each language on each dataset. \textbf{MoverScore-1} performs worse when disabling IDF-weighting on WMT18 and WMT19 for all languages. However, on WMT17, IDF-weighting has negative impact in the evaluation of German, Chinese and Turkish. The maximum deviation appears on WMT19 en-de, which is just the reserved language pair where MoverScore-1 drops most when disabling IDF-weighting in English evaluation. 

%For \textbf{BERTScore-F1}, no language behaves consistently on all datasets. 

%Besides, it can be observed that the performance drop is never out of the range of RD for English, whereas there are two values for each evaluation metric that is larger than the maximum performance improvement for English (MoverScore: WMT17 en-zh and en-tr; BERTScore: WMT17 en-de and WMT18 en-tr). Thus, those facts suggest that \emph{the effectiveness of IDF-weighting seems less stable in the evaluation of other languages compared with English}.

%\paragraph{Punctuation Removal \& Subwords Selection}


%First, we show the relative change from removing to keeping punctuations for each language on each dataset in Figure \ref{fig:punc sub all}. Despite of Turkish, fluctuation of RDs for all other languages is within the range of RDs for English. Furthermore, no language behaves consistently on all datasets except Czech; both negative and positive extrema can be observed even on one single language, namely Turkish. This kind of inconsistency has been previously observed on English. All of the facts mentioned suggest \emph{the similar effects of punctuation removal across different evaluation languages}. Next, we also examine the best configuration of subword selection and punctuation removal in combination for each language, as shown in Table \ref{tab:ditro}. \emph{In contrast to English, MoverScore-1 is more likely to get better results when not only using the first subword, no matter with or without punctuation removal}. Further, \emph{no configuration always performs best for a certain language on all datasets, which is in line with English evaluation}. In addition, it is noteworthy that \emph{MoverScore-1 never achieves the best results applying \emph{ave-all+PR} for all languages, including English}. 


%\subsection{Experimental Setup}
%\label{set:sensitivity}












%\subsubsection{Stopwords Removal in English}


%\subsubsection{IDF-weighting in English Evaluation}
 

%\subsubsection{Subword Selection \& Punctuation Removal in English Evaluation}



%\subsubsection{Comparison among Evaluated Languages}


%\subsubsection{Noisy Alignment Removal}
%\label{noisy set}
%In this experiment, we inspect the effect of \gls{NAR} on \gls{WMD}-based evaluation metric, i.e., MoverScore and XMoverScore, and also its effect in combination with n-gram. In the first step, we evaluate MoverScore-1 and XMoverScore-1 applying noisy alignment removal with dropout\_rate from 0.1 to 0.5 on WMT17 to-English language pairs, allowing for a comparison of the effects of NAR between monolingual and cross-lingual evaluations. Subsequently,  we evaluate MoverScore-1 on all language pairs in WMT18-19 to study the effects of NAR in the evaluation of different languages. Lastly, we study the effect of embedding granularity on the noisy removal version of MoverScore and XMoverScore. we present the results in Section \ref{re:noisy}.


%\subsubsection{Layer Selection \& Aggregation}
%\label{layer set}
%In this experiment, we conduct layer-wise evaluation for XMoverScore and then compare the results to \citet{zhao2019moverscore}. we show the variation of metric performance regarding different layer selection and compare the metric performances obtaining from the best single layer and power means to see if power means also works well in cross-lingual evaluation. For XMoverScore, we test the variants with and without language model on the target side. we do not consider the variant with re-mapping, since the authors only released the mapping matrices for layer 8 and 12. we report the results for MoverScore-1 and XMoverScore-1 in Section \ref{re:layer}.



%\subsection{Experiment Results}
%\label{re:sensitivity}

%\subsubsection{Stopwords Removal in English Evaluation}



%\subsubsection{IDF-weighting in English Evaluation}




%\subsubsection{Subword Selection \& Punctuation Removal in English Evaluation}


%\subsubsection{Comparison among Evaluated Languages}







%\subsubsection{Noisy Alignment Removal}
%\label{re:noisy}
%This section describes the evaluation results of noisy alignment removal (NAR). First, we show whether the WMD-based evaluation metrics benefit from NAR in both monolingual and cross-lingual evaluations in Table \ref{tab:noisy}, evaluated on WMT17 to-English pairs. First, \emph{noisy alignment removal does not lead to consistent improvement}. In fact, when only the average correlations are considered, only XMover-1+CLP benefits from NAR. In cross-lingual evaluations, the metric performances on ru-en can be consistently improved by NAR; in contrast, that on lv-en and zh-en never enhance with NAR. In monolingual evaluations, NAR is beneficial to MoverScore on fi-en and lv-en, no matter with or wihout IDF-weighting. Secondly, \emph{IDF-weighting still has positive impact when applying noisy alignment removal}. For all dropout rates, IDF-weighting impacts MoverScore positively. As described above, the performance enhancement with NAR can be seen on different language pairs in monolingual and cross-lingual evaluations. It may be caused by the difference in BERT and multilingual BERT. 






%Hence, we also consider monolingual setup for other languages, with multilingual BERT. Figure \ref{fig:noisy 18 19} demonstrates the results on WMT18 and WMT19. As the figure shows, NAR leads to consistent performance improvement for all languages except Chinese and English. It is interesting that Chinese and English are distant languages but they behave similarly with NAR; In contrast, similar languages to English, like German, do not behave consistently with English. To my best knowledge, the only thing that English and Chinese have in common is they are high-resource languages in NLP. So we assume the difference in the effectiveness of NAR between these two languages and others is due to that multilingual BERT does not handle those languages well and consequently the non-optimal representations leading to more noisy alignments in WMD. To verify this, we evaluate NAR with language-specific BERT. Table \ref{tab: noisy language specific} shows the results for German and Turkish. It can be seen that NAR still has positive impact after applying language-specific models, just the improvement for Turkish falls a little. As a result, the previous assumpation can not be confirmed and the reason of the ineffectiveness of NAR on Chinese and English is unclear so far. 


%Next, we study the effect of n-gram on noisy alignment removal. we test the n-gram from 1 to 3 and dropout rate from 0.1 to 0.5. Table \ref{tab:noisy-ngram} shows the results on WMT17 for both cross-lingual and monolingual evaluations. In monolingual evaluations, unigram MoverScore performs best for all dropout rates, suggesting \emph{a negative impact of n-gram in monolingual evaluations}. As for cross-lingual evaluations, the metric performance enhances with increasing n-gram before applying the LM on the target side for all dropout rates. However, it is interesting that an opposite result emerges after applying the LM: unigram XMoverScore performs best except for dropout rate 0.1, where bigram works slightly better than unigram. This suggests that n-gram works like a syntax model here; it plays a similar role to LM. However, the improvement from n-gram is tiny compared with LM.




%\subsubsection{Layer Selection \& Aggregation}
%\label{re:layer}
%This section presents the experiment results of Section \ref{layer set}. Table \ref{tab:mover layer}, \ref{tab:xmover layer} and \ref{tab:xmover LM layer} show the layer-wise experiment results for MoverScore-1, XMoverScore-1 and XMoverScore-1+LM, respectively.  
%First, the variations of metric performances with the changes of layer selection are much larger in cross-lingual evaluations; The CVs for MoverScore are within 1\% except on cs-en, whereas the CVs for XMoverScore range from 5.34\% to 24.69\%. After applying LM on the target side, the CV for XMoverScore decreases from 11.68\% to 3.65\% on average. Secondly, the RDs of the metric performances between using the best layer and power means show that the positive impact of power means decreases in cross-lingual evaluations; the RD in monolingual evaluation is -0.08\% on average while that in cross-lingual evaluations range from -18.57\% to 0.51\% and is -4.16\% in average. Similar to layer selection, the value drops after applying LM on the target side. The difference between monolingual and cross-lingual evaluations may due to the use of multilingual BERT. The results of previous experiments show that multilingual BERT or different evaluated languages can lead to changing effects of some factors, so the effects of layer selection and aggregation should be also studied in monolingual evaluations of other languages further. we leave this in future work.

==> structure/structure/7_sensitivity_old.tex <==
\section{Sensitivity Analysis}
\label{sec:sensitivity}
In this section, we investigate the sensitivity of BERT-based evaluation metrics to the factors discussed in Section \ref{sec:factors}. The experimental setup is presented in Section \ref{set:sensitivity}, followed by the corresponding results (Section \ref{re:sensitivity}). 
%In addition, based on the experiment results, we conduct further experiments, aiming at improving the reproducibility for MoverScore (Section \ref{cleaner}).


\subsection{Experimental Setup}
\label{set:sensitivity}

The statistics used to quantify the sensitivity are described in Section \ref{statistics}. Based on the results of reproduction experiments (details see Section \ref{re:reproduction}), we only consider MT and summarization evaluation in this part, in order to avoid the bias from the potential incorrect evaluation scripts and ensure %my 
results are comparable with \citet{zhao2019moverscore}. As mentioned in previous sections, we mainly focus on MoverScore in this work. %, so most experiments are about it and based on monolingual evaluation which it is originally designed for. 
%Further, 
\citet{zhao2019moverscore} only evaluated MoverScore on English data,
%As MoverScore is originally designed to evaluate NLG system outputs in English, 
so we first investigate the sensitivity to the factors in English evaluation. To begin, we inspect how sensitive the evaluation metrics are to different settings regarding stopwords in Section \ref{stopwords set}. Then we disable IDF-weighting to check whether it positively impacts the evaluation metrics or not. Given that IDF-weighting is corpus-dependent, we also inspect the sensitivity of the evaluation metrics to various IDF-weighting corpora (Section \ref{idf set}). Subsequently, since MoverScore uses a single parameter to enable discarding all subwords except the first and punctuation removal, we test their impacts together (Section \ref{sub set}). Then, we extend the former experiments to other language environment (Section \ref{compare set}), to see if the evaluation metrics behave consistently to those factors in the evaluation of different languages. In each experiment, we only adjust the settings of the tested factors and keep the others default. The default configuration of the evaluation metrics involved in these experiments are given %below:
in the appendix (Section \ref{sec:default}). 




\subsubsection{Statistics}
\label{statistics}
We use 4 statistics to quantify the sensitivity of the evaluation metrics. When there are only \textbf{two compared values}, we compute Absolute Different (AD)\todo{SE: definition is missing} and Relative Difference (RD) to reflect the absolute and relative performance variation regarding a certain factor.

%\paragraph{Absolute Difference (AD)}
%\emph{Absolute Difference} measures the distance between two real numbers on the real line by simple subtraction. It demonstrates the variation between two numbers most intuitively. Its formula is given below: 
%$$AD(a,b)=a-b$$

\paragraph{Relative Difference (RD)}
\emph{Relative Difference} is the ratio of absolute difference to the reference value. 
%Since this work concerns different dimensions such as different evaluation metrics, NLG tasks, datasets, and factors, to ensure the representation of the deviations are comparable across them, it is necessary to use scaled and dimensionless statistics like RD. In this work, RD is expressed as percentage, as the formula given below:
$$RD(a,b)=\frac{a-b}{b}*100\%$$ where $b$ is the reference value.



When there are \textbf{more than two compared values}, we compute range to directly show the maximum deviation of the values, and Coefficient of Variation (CV) to reflect the extent of variability. 

\paragraph{Range}
\emph{Range} refers to the difference between the largest and smallest values of a set of data: %calculated by subtracting the sample maximum and minimum, as shown below:
 

$$Range(x) = x_{max}-x_{min}$$ where $x$ is the set of data.

\paragraph{Coefficient of Variation (CV)} 
\emph{Coefficient of Variation} is defined as the ratio of the standard deviation to the mean. It is also a dimensionless and scaled statistics, measuring dispersion of a set of data. We report the population CV (or the sample CV)
%In this work, two kinds of CV are considered. First, if the tested cases are only a sample from all possible situations, we calculate 
%sample CV. Secondly, if the tested cases already contain all possible scenarios, we calculate population CV. The difference between them is whether sample or population standard deviation is taken into account. 
%Similar to RD, they are expressed as percentage in this work. Their formulas are given below:
%\begin{itemize}
    %\item \textbf{Population CV}
    
    \begin{align*}
        CV(x) &= \frac{\sigma}{\mu}*100\% 
        \quad 
        %\intertext{where}\quad 
        %\sigma &= \sqrt{\frac{\sum {({x_{i}-\mu)}^2}  }{N} } 
    \end{align*}
    
%    \item \textbf{Sample CV}
%    
%    \begin{align*}
%        CV(x) &= \frac{s}{\overline{x}}*100\% \\
%        \intertext{where}
%        s &= \sqrt{\frac{\sum {({x_{i}-\overline{x} )}^2}  }{N-1} } 
%    \end{align*}
    
     
%\end{itemize}
where $\sigma$ is the standard devation and $\mu$ is the mean. 

%According to the characteristics of those statistics, 
Larger absolute values of the statistics indicate higher sensitivity of the evaluation metrics. Based on the parameter of the tested factors, we use AD and RD to represent the variation regarding IDF-weighting disabling and punctuation removal, range and sample CV to quantify the sensitivity regarding changing stopwords settings and IDF-weighting, %(since we could only test some stopword lists and IDF-weighting corpora), 
and range and %population
CV to reflect the impact of subword selection.





\subsubsection{Stopwords Removal in English}
\label{stopwords set}


In this experiment, we consider 4 stopword settings including disabling stopwords removal and applying 3 different stopword lists. The first stopword list is obtained from the Github repository of MoverScore, which contains 153 words. Since users may first choose the existing stopword lists from popular libraries, we consider the stopword lists from NLTK \citep{bird2009natural} and SpaCy \citep{spacy2}, which consist of 179 and 326 words, respectively. %According to \citet{zhao2019moverscore}, unigram and bigram MoverScore alternates as the best measure on different tasks; thus, we consider these two variants in this test. 
In addition, we also test the sensitivity of BERTScore-F1 to stopwords as a comparison, despite it does initially not supporting this technique. we denote the evaluation metrics with different stopword settings as \emph{metric name + size of stopword list}. E.g., \emph{Mover-1+326} represents unigram MoverScore applying the stopword list from SpaCy. 
%We calculate CV and range of the correlations over the 4 stopword settings for each language pair in WMT datasets.
We report the results for MoverScore-1, MoverScore-2 and BERTScore-F1 on WMT17-19 and TAC2008-2009 datasets in Section \ref{re:stopwords}.

\subsubsection{IDF-weighting in English Evaluation}
\label{idf set}
In this test, we first disable IDF-weighting (idf-dis) for the evaluation metrics, and compare the metric performance to that when applying original IDF-weighting(idf-ori).

%With this, we can clearly know whether IDF-weighting positively impacts these evaluation metrics and how large the deviation can be resulting from this factor. 
Next, we apply IDF-weighting from four corpora to the evaluation metrics (idf-random);\todo{SE: what is idf-random?} each corpus consists of 2k English segments randomly selected from all tested datasets, namely WMT17-19 and TAC2008-2009. We consider the internal corpora first because in practice, users %often 
may select to use a certain part of the evaluated datasets as the IDF-weighting corpus. %although the selection of texts used to compute IDF-weighting fully depends on them. 
%We report the results on WMT17-19 and TAC2008-2009 for MoverScore-1, MoverScore-2 and BERTScore-F1 in Section \ref{re:internal} (internal IDF-weighting). Based on the former results (details see Section \ref{re:internal} (internal IDF-weighting)), 
Subsequently, we test the IDF-weighting from %large-domain and 
large-scale corpora. %further, expecting it can provide more comprehensive and precise information about word importance. 
%The results are presented in Section \ref{re:external} (external IDF-weighting).
We obtain these corpora from Hugging Face Datasets.\footnote{\url{https://huggingface.co/datasets}} They are listed in the appendix (Section \ref{sec:idf_corpora}). 

\subsubsection{Subword Selection \& Punctuation Removal in English Evaluation}
\label{sub set}
In this experiment, we evaluate the sensitivity of MoverScore-1 to different subword selection and  PR (punctuation removal). There are originally two selections of subwords: keeping the first subword and keeping all subwords. In addition, we also implement another technique, i.e., to average the embeddings of the subwords in one word to get the word-level BERT representations. This leads to 6 configurations together with PR: 1) first, 2) all, 3) ave-all, 4) first+PR, 5) all+PR, and 6) ave-all+PR. We report the results on WMT17-19 and TAC2008-2009 for MoverScore-1 in Section \ref{re:sub}.


\subsubsection{Comparison among Evaluated Languages}
\label{compare set}
In this test, we compare the sensitivity of the evaluation metrics across different language environment by extending the former experiments to 
the monolingual evaluation for other 6 languages: Chinese (zh), Turkish (tr), Finnish (fi), Czech (cs), German (de), and Russian (ru).

We choose those languages because at least two WMT datasets contain the evaluation data in the question language, making a comparison across datasets possible and thus preventing drawing conclusions from results generated by chance. We obtain the stopword lists for other languages from the resources listed in the appendix (see Section \ref{sec:otherlangs}).  


We report the results for MoverScore-1 and BERTScore-F1 on WMT17-19 in Section \ref{re:compare}.
\todo{SE: It would generally be better to give results for each setting right away, to decrease cognitive load for the reader}

%\subsubsection{Noisy Alignment Removal}
%\label{noisy set}
%In this experiment, we inspect the effect of \gls{NAR} on \gls{WMD}-based evaluation metric, i.e., MoverScore and XMoverScore, and also its effect in combination with n-gram. In the first step, we evaluate MoverScore-1 and XMoverScore-1 applying noisy alignment removal with dropout\_rate from 0.1 to 0.5 on WMT17 to-English language pairs, allowing for a comparison of the effects of NAR between monolingual and cross-lingual evaluations. Subsequently,  we evaluate MoverScore-1 on all language pairs in WMT18-19 to study the effects of NAR in the evaluation of different languages. Lastly, we study the effect of embedding granularity on the noisy removal version of MoverScore and XMoverScore. we present the results in Section \ref{re:noisy}.


%\subsubsection{Layer Selection \& Aggregation}
%\label{layer set}
%In this experiment, we conduct layer-wise evaluation for XMoverScore and then compare the results to \citet{zhao2019moverscore}. we show the variation of metric performance regarding different layer selection and compare the metric performances obtaining from the best single layer and power means to see if power means also works well in cross-lingual evaluation. For XMoverScore, we test the variants with and without language model on the target side. we do not consider the variant with re-mapping, since the authors only released the mapping matrices for layer 8 and 12. we report the results for MoverScore-1 and XMoverScore-1 in Section \ref{re:layer}.



\subsection{Experiment Results}
\label{re:sensitivity}

\subsubsection{Stopwords Removal in English Evaluation}
\label{re:stopwords}
This section describes the results of stopwords tests in English evaluation, following the experimental setup described in Section \ref{stopwords set}. For MT, we calculate CV of the correlations \se{with humans} over the 4 stopword settings for each language pair in the datasets, then we average the CVs over the language pairs in each dataset to obtain the average CV per dataset; in the end, we average the CVs for the three datasets to get the average CV per evaluation metric. For summarization, we calculate CV of the correlations over the 4 stopword settings for each criterion on each dataset. The performance of each evaluation metric with each setting on each dataset and the corresponding statistics can be found in Appendix \ref{appendix: stopwords tables}. Here, we only present the average
%overall 
CVs for MT and the CVs for summarization, which can reflect the variations of metric performances independent of the differences in absolute correlations. 



 
Table \ref{tab:sw wmt all} displays the average CVs for MT. It can be observed that all average CVs per dataset at system-level are within 0.5\%, even including BERTScore-F1, whose average CV is up to 7.72\% at segment-level, suggesting that these evaluation metrics are much less sensitive to stopwords at system-level than at segment-level. The reason could be that system-level scores are average values, and consequently, some positive and negative deviations compensate for each other within one system. Next, when comparing BERTScore to MoverScore, BERTScore-F1 are roughly up to 4 times as sensitive as the two variants of MoverScore based on their CVs. On the other hand, MoverScore-2 is more sensitive than MoverScore-1; its average CVs per dataset are larger than MoverScore-1 except on WMT17, resulting in a +0.17 percent points absolute difference in average CVs over the three datasets. The reason might be that the changes in stopwords can lead to various combinations of n-gram. As a result, the impact is more considerable on multiple grams than unigram.





Figure \ref{fig:sum cv sw} shows the CVs on TAC2008-2009 datasets. Among the three types of correlations, Kendall's $\tau$ varies the most, whereas Pearson's $r$ varies the least under the same evaluation condition. In the evaluation of pyramid, these evaluation metrics are slightly more sensitive than in the evaluation of responsiveness. Next, when comparing the three evaluation metrics, similar observation to MT evaluation can be made that 1) BERTScore-F1 is most sensitive among the three evaluation metrics and 2) MoverScore-2 is more sensitive compared with MoverScore-1. 

Besides, MoverScore is less sensitive to stopwords in summarization evaluations than in segment-level MT evaluations, since 1) the CVs for MoverScore-1 on summarization are within 0.5\%, while the minimal average CV for segment-level MT evaluation is 1.42\% (WMT19); and 2) all average CVs per WMT dataset for MoverScore-2 are about 2\% in segment-level MT evaluations whereas the maximum CV is about 1.5\% on summarization. In contrast, BERTScore-F1 does not show this characteristic unless only Pearson correlation is considered. 





When looking at the individual correlation for each stopword setting, it can be observed that the stopword list provided by \citet{zhao2019moverscore} (153 words) and the NLTK stopword list (179 words) have the same effect. Figure \ref{fig:example stopwords} illustrates some examples of the variations of metric performance with the changes of stopwords settings. The first two line charts show the correlations of MoverScore-1 on WMT17; the third one demonstrates the correlations of both unigram and bigram MoverScore on TAC2008 dataset. It shows that the correlations are identical when using the two stopword lists in all evaluation tasks. By checking the difference in these two stopword lists, we found that the MoverScore stopword list excludes contractions from NLTK stopword list, such as \emph{wouldn't} and \emph{haven't}, which are split into smaller wordpieces by BERT's tokenizer due to the feature of subword-level tokenizers. Hence, stopwords in the form of contractions cannot influence the metric scores.




Next, to inspect whether the evaluation metrics benefit from stopwords removal, we take a look at the best stopword settings for each evaluation task. Figure \ref{fig:sw distribution} illustrates the distribution of the best stopword settings. The rings from the inside to the outside represent MoverScore-1, MoverScore-2, and BERTScore-F1. As mentioned above, the NLTK stopword list impacts the evaluation metrics equally with the MoverScore stopword list, so there are only three settings left. we regard each language pair in WMT datasets as a test case for MT, resulting in 21 test cases (3 datasets times 7 language pairs). For summarization tasks, we regard each type of correlation as a test case for each criterion, resulting in 6 test cases (3 correlations times 2 datasets). For segment-level MT evaluation (Figure \ref{fig:sw distribution}(a)), there is only one case that the best result is achieved by removing stopwords, which takes place on MoverScore-1.
In contrast, the best stopword lists for system-level MT evaluation can be any of the settings for all evaluation metrics (Figure \ref{fig:sw distribution}(b)). However, in about 50\% of the test cases, MoverScore still performs best when disabling stopwords removal. In pyramid evaluation (Figure \ref{fig:sw distribution}(c)), MoverScore-1 achieves the best results using the original stopword list for all test cases, whereas disabling stopwords removal is still the best choice for MoverScore-2 and BERTScore-F1. In the evaluation of responsiveness ((Figure \ref{fig:sw distribution}(d))), two cases (33.3\%) can be seen that MoverScore-1 applying the original stopword list performs best; this happens only once on MoverScore-2 (16.7\%). BERTScore-F1 never benefit from stopwords removal on all evaluation tasks. 

The difference between the impacts of stopwords removal on MoverScore in segment-level MT and summary-level summarization evaluations may be due to the fact that summary evaluation requires greater attention to the content words. However, the CVs for MoverScore in summarization evaluations are small, suggesting the performance gain from stopwords removal is tiny. In contrast, MoverScore behaves more sensitive to stopwords in segment-level MT evaluations, but stopwords removal has negative impact here, suggesting the performance drop from stopwords removal is larger than the performance gain from stopwords removal. Hence, for the purpose of improving reproducibility, MoverScore should drop the parameter regarding stopwords removal.
The inconsistency between the sensitivity of MoverScore and BERTScore may result from the difference in their scoring algorithms. In conclusion, it seems stopwords removal is not needed for considered BERT-based evaluation metrics; the reason could be that BERT already correctly gives those non-content words enough low attention.


\subsubsection{IDF-weighting in English Evaluation}
\label{re:idf}
This section presents the results of IDF-weighting tests in English evaluation, following the experimental setup in Section \ref{idf set}. Similar to stopwords, we put the whole results and the corresponding statistics in Appendix \ref{appendix: idf tables} and only present the scaled statistics here, namely RD and CV. we use the same methods to get the average CVs per dataset and per evaluation metric as in stopwords tests.

\paragraph{Internal IDF-weighting}

\label{re:internal}


To begin, we show the relative performance change on MT when disabling IDF-weighting with RDs(dis-ori) in Figure \ref{fig:rd dis ori wmt}. Negative percentage values indicate positive impacts of IDF-weighting and vice versa. Firstly, all average RDs(dis-ori) are negative, implying a positive impact of IDF-weighting on MT evaluation tasks. Further, the differences in RDs between evaluation levels suggest that these evaluation metrics benefit from IDF-weighting more at segment-level, since 1) all average RDs at system-level are within -1\%, whose absolute values are much smaller than those of the RDs at segment-level;

and 2) less positive RDs(dis-ori) can be seen in segment-level evaluations (e.g., IDF-weighting impacts MoverScore negatively only once). Next, among these three evaluation metrics, at segment-level, on the one hand, BERTScore-F1 is least sensitive, which is on the contrary to the observation in the stopwords tests (Section \ref{re:stopwords}); on the other hand, similar to the observation in the stopwords tests, bigram MoverScore is more sensitive than unigram MoverScore. It is noteworthy that the maximal performance drop of MoverScore is much larger than the other drops, but this does not take place on BERTScore-F1. By checking the correlations for this language pair, namely de-en in WMT19 (details see Table \ref{tab:wmt19 idf} in \ref{appendix: idf tables}), it can be seen that when using IDF-weighting, MoverScore outperforms BERTScore-F1 substantially on this evaluated data (0.22 vs. 0.15 Kendall's $\tau$), but their performances differ only slightly when disabling IDF-weighting (smaller than 0.01 Kendall's $\tau$). Quite the contrary, the performances of all evaluation metrics fall most on WMT18 tr-en at system-level. 




Figure \ref{fig:rd idf sum} shows the RDs(dis-ori) on TAC2008-2009. Those values fluctuate around 0, implying that IDF-weighting does not lead to consistent improvement in summarization evaluations. However, for MoverScore, IDF-weighting still has a positive impact in most cases, and the performance drop is often larger than the enhancement due to IDF-weighting disabling, especially for bigram MoverScore. Regarding BERTScore-F1, the cases that IDF-weighting impacts it positively/negatively are fairly distributed. Among these three evaluation metrics, MoverScore-1 is least sensitive with all deviations smaller than 1\% except on TAC2009 responsiveness; bigram MoverScore is again more sensitive than unigram MoverScore; BERTScore-F1 has the in-between variations. Further, different correlations can behave the other way around, i.e., one correlation may increase while another falls under the same evaluation condition. E.g., the Pearson correlation of MoverScore-2 rises when disabling IDF-weighting in responsiveness evaluation on TAC2009, whereas the other two correlations descend.






Next, Table \ref{tab:wmt idf cv} and Table \ref{tab:tac idf cv} display CVs(ori+random) for MT and summarization evaluation tasks. All CVs are smaller than 1\% except those in segment-level MT evaluations, suggesting that the selection of IDF-weighting corpora impacts the metric performance slightly. The maximum variation of MoverScore can be seen on WMT19, which is also caused by the results for de-en; MoverScore with idf-ori outperforms it with idf-random substantially here (0.22 vs. 0.15 Kendall's $\tau$). Similar to stopwords, it can be observed that Kendall is most sensitive among the three correlations, whereas Pearson is least sensitive. When comparing the three evaluation metrics in segment-level MT evaluations, BERTScore-F1 is the least sensitive one, and bigram MoverScore is more sensitive than unigram MoverScore, which is in line with the previous observations (IDF-weighting disabling tests). It may be due to that BERTScore originally only uses the references to compute IDF-weighting, whereas MoverScore computes IDF-weighting for references and hypotheses separately; thus, the actual variations of IDF-weighting of BERTScore is smaller than those of MoverScore. 




To investigate whether idf-random also positively impacts the evaluation metrics, we calculate RDs(random-dis), which denote the relative performance change from disabling IDF-weighting to applying idf-random. 
In this test, only segment-level MT evaluation is concerned since those evaluation metrics behave most sensitively to IDF-weighting in this evaluation. There are 84 test cases because 4 idf-random are applied to each language pair. The middle column of Figure \ref{fig:idf rd wmt seg} shows these values. The average RDs(random-dis) for all evaluation metrics are positive, suggesting a positive impact of idf-random. Subsequently, we calculate RDs(random-ori), representing the performance change from using idf-ori to idf-random. The right column of Figure \ref{fig:idf rd wmt seg} shows these values. It can be seen that BERTScore-F1 performs even a little better with idf-random, shown with a positive average RD(random-ori) +0.05\%. However, those values fluctuate around 0; therefore, we would only say that idf-random and idf-ori are equally effective to BERTScore-F1. As for MoverScore, in the majority of the cases, idf-ori still works better. Further, the extrema in the figures for MoverScore can be seen at the same position (red box), which denotes the results for de-en in WMT19. The cause is, as mentioned before, idf-ori leads to a substantial performance enhancement to MoverScore on this evaluation data.



We can conclude that IDF-weighting positively impacts BERT-based evaluation metrics in English evaluations, regardless of where it originates. However, original IDF-weighting still works best for MoverScore. Based on the results, we test IDF-weighting from large-domain and large-scale corpora, expecting it can provide more comprehensive information about the word importance, since original IDF-weighting is computed using only 1000-3000 documents. 


\paragraph{External IDF-weighting}
\label{re:external}


Table \ref{tab:external en} presents the results for external IDF-weighting test in English evaluation. First, the size of those corpora is much larger than the original corpora  but MoverScore still performs better with original IDF-weighting. Secondly, the results for Wikipedia shows that the metric performance does not enhance with the increasing size of corpora. Thirdly, although those corpora contain articles in many domains, they do not provide more applicable IDF-weighting neither. In conclusion, no IDF-weighting from large-domain and large-scale works as well as the original IDF-weighting in English evaluation.



\subsubsection{Subword Selection \& Punctuation Removal in English Evaluation}
\label{re:sub}
This sections presents the experiment results for subword selection and punctuation removal in English evaluation, following the experiment setup described in Section \ref{sub set}. 







To begin, we show the relative performance change from removing to keeping punctuations in MT evaluations in Figure \ref{fig:punc rd wmt}(a) with RD(keep). Positive values indicate positive impacts of punctuation removal (PR). Firstly, it can be also observed that the evaluation metrics are more sensitive at segment-level than system-level. Secondly, despite the average RDs at both evaluation levels being negative, the values fluctuate around 0, so the effectiveness of PR in MT evaluations can not be confirmed. Next, RDs(keep) on TAC2008-2009 are visualized in Figure \ref{fig:punc rd wmt}(b). It also shows that the contribution of PR is unstable. MoverScore-1 performs even better when keeping punctuations on responsiveness. However, the deviations are within 0.6\%, implying a low sensitivity of MoverScore to punctuations in summarization evaluations. The three correlations behave again inconsistently on TAC2009 pyramid, where the Pearson correlation drops a bit while the other two rise when keeping punctuations. Similar observation has been made in IDF-weighting disabling tests discussed in Section \ref{re:idf}. 



Further, we show the variation of metric performance regarding subword selection on WMT17-19 in Figure \ref{fig:sub rd wmt}(a) with CV. Again MoverScore is more sensitive at segment-level than at system-level. The metric performance varies most at segment-level on WMT19 de-en and at system-level on WMT18 tr-en; the largest deviations from changing IDF-weighting also take place on these two language pairs. This may suggest that the evaluation data itself is also a determinant of reproducibility for evaluation metrics. The average CV for segment-level evaluation (1.6\%) indicates a similar level of sensitivity of MoverScore to subwords, stopwords and IDF-weighting (the average CVs for stopwords and IDF-weighting are 1.87\% and 1.12\%, respectively). Next, the CVs on TAC2008-2009 are shown in \ref{fig:sub rd wmt}(b). Except the Kendall correlation on TAC2008 pyramid, all CVs are within 1\%, implying the insensitivity of MoverScore to subword selection in summarization evalautions. And the three correlations in descending order of sensitivity are again Kendall, Spearman, and Pearson. 

 




To investigate which configuration of subword selection and punctuation removal in combination is optimal, we show the number of times that each configuration works best in Figure \ref{fig:sub punc best}. we mark the default setting \emph{first+PR} with $*$. On the most sensitive task, namely segment-level MT evaluation, MoverScore-1 achieves the best performance applying the original setting in 12 out of 21 cases. In system-level MT evaluations, using all subwords and punctuation removal is the best choice (9/21). As for summarization, there is no explicit clue about which is the best configuration. Considering that MoverScore-1 is most sensitive in segment-level MT evaluations, keeping the original setting is the best choice for now. 

\subsubsection{Comparison among Evaluated Languages}
\label{re:compare}

This section compares the sensitivities of MoverSocre-1 and BERTScore-F1 in MT evaluation across different languages, following the experiment setup described in Section \ref{compare set}. The main purpose of this section is to answer the following two questions: 1) \emph{Is the sensitivity of BERT-based evaluation metrics similar across different evaluation languages?}; and 2) \emph{Do positive/negative factors still positively/negatively affect BERT-based evaluation metrics for other languages?}.

\subsubsubsection{Q1: Is the sensitivity of BERT-based evaluation metrics similar across different evaluation languages?}
To examine how large impact the factors have in the evaluation of other languages, we calculate the average statistics over WMT17-19 for all tested languages. Figure \ref{fig:all} demonstrates the results. The evaluation metrics behave more sensitive at segment-level than at system-level for all languages, which is consistent with English evaluation. Almost all values for system-level evaluation are within 1\%. The exception is Turkish, whose CV-subwords of MoverScore-1 and RD-idf of BERTScore-F1 have absolute values over 1\%. The performance of BERTScore-F1 even drops more at system-level than at segment-level when disabling IDF-weighting (-2.58\% vs. -1.21\%). Furthermore, it is interesting that at system-level, MoverScore-1 behaves most sensitively in Turkish evaluation to all factors except punctuation removal. Overall, at system-level, those factors have only tiny impacts on BERT-based evaluation metrics, so 
We discuss the similarity and dissimilarity of sensitivity across different languages in segment-level evaluation further in the following paragraphs. 



\paragraph{MoverScore-1} Russian is most sensitive to \textbf{stopwords}; its CV-stopwords is 3.62 percent points higher than that of English. Chinese and Turkish are slightly less sensitive than English with a absolute deviation of CVs-stopwords within 0.3 percent points. German and Turkish are more sensitive to \textbf{IDF-weighting} than English, and only the CVs-idf of these three languages are over 1 percent points. However, the deviations of CVs-idf of all languages to the CV-idf of English are within 1 percent point, so there is no considerable difference in the sensitivity to IDF-weighting across different languages. Next, except Turkish, all other RDs-idf are negative, indicating a positive impact of IDF-weighting to some extent, but it should be noted that the contribution of IDF-weighting can not be confirmed only by an average RD, since negative and positive RDs can compensate for each other in multiple datasets. Hence, we also show the RD-idf for each dataset later, to investigate whether MoverScore truely benefits from IDF-weighting in the evaluation of other languages.  As for \textbf{subwords}, German and Chinese show a lower sensitivity than English. The CV-subwords of Chinese is even smaller than 1\%. The reason might be that Chinese is a character-based language,  and in fact, after the tokenization by multilingual BERT, there are rarely wordpieces with ``\#\#''. As a result, the selection of subwords won’t affect MoverScore in Chinese evaluation too much. The CVs-subwords of Russian and Turkish are about 2.5 percent points higher than that of English, suggesting MoverScore is more sensitive to subwords in the evaluation of these two languages. Except them, all deviations of CVs-subwords of other languages to that of English are whithin 1 percent point. Further, all RDs-punctuation are within 1\% except for Chinese, suggesting a low sensitivity of MoverScore to \textbf{punctuation removal}. There is no explanation for the fact that Chinese is according to my test more sensitive to punctuation removal than other languages, since Chinese punctuation uses a completely different set of punctuation marks from other languages, and in my tests, only the default set punctuations in Python are removed, which does not contain any Chinese punctuation. The reason could be that some of the system translations contains western punctuations by mistake. Similar to IDF-weighting disabling tests, it can not be simply determined with an average RD whether punctuation removal has a positive impact, so we also discuss this later in more details. 



\paragraph{BERTScore-F1} For \textbf{stopwords}, only the deviation of CV-stopwords of Chinese to that of English is within 1 percent point, suggesting the sensitivity of BERTScore-F1 to stopwords is similar in the evaluation of these two languages. Chinese and English are also most sensitive compare with other languages, whereas Finnish is least sensitive. Regarding \textbf{IDF-weighting}, BERTScore-F1 is insensitive for all languages except for Turkish; its CV is close to 2\% whereas the others are within 0.31\%. Further, the effectiveness of IDF-weighting seems unstable across different languages. Similar to MoverScore-1, we show the RDs-idf on each dataset later. 


\paragraph{Between MoverScore and BERTScore} Although the behaviours of each language to each factor are different across these two evaluation metrics, there is still something in common: 

\begin{itemize}


    \item Both evaluation metrics have the same ranking of the magnitudes of the effects of IDF-weighting and stopwords for each language. They are more sensitive to stopwords than to IDF-weighting with the only exception that MoverScore behaves more sensitively to IDF-weighting in the evaluation of Turkish.
    On MoverScore, subword selection has the second largest impact. The exceptions is German, which behaves least sensitive to subwords.
    
    
    \item Interestingly, as the matter of fact, English and Chinese have almost synchronized behaviour to stopwords; although the results on both languages show big difference between the two evaluation metrics regarding stopwords, the CV-stopwords of these two languages remain closest. Further, for some languages, such as German, Czech, and Finnish, the difference is less pronounced (absolute deviation of CVs within one percent point).
    
    
    \item Both evaluation metrics behave most sensitively to IDF-weighting in the evaluation of Turkish compared with other languages.
    
\end{itemize}


\subsubsubsection{Q2: Do positive/negative factors still positively/negatively affect BERT-based evaluation metrics for other languages?}

\paragraph{Stopwords Removal}

Table \ref{tab:sw distribution} displays the best stopword setting for each language in segment-level MT evaluations. Except Finnish and Turkish, disabling stopwords removal is always the best choice for all other languages. For Finnish, only on one dataset, MoverScore-1 performs better using stopwords removal, whereas, for Turkish, both evaluation metrics achieve the best performance applying the same stopword lists. The reason might be that both Turkish and Finnish belong to agglutinative languages, and those languages tend to have a high rate of affixes or morphemes per word, which means there may exist more noise in word embeddings. In summary, \emph{for most languages, BERT-based evaluation metrics do not benefit from stopwords removal, which is consistent with English evaluation}.






\paragraph{IDF-weighting}

Figure \ref{fig:idf rd all languages} shows the relative performance change from using the original to disabling IDF-weighting for each language on each dataset. \textbf{MoverScore-1} performs worse when disabling IDF-weighting on WMT18 and WMT19 for all languages. However, on WMT17, IDF-weighting has negative impact in the evaluation of German, Chinese and Turkish. The maximum deviation appears on WMT19 en-de, which is just the reserved language pair where MoverScore-1 drops most when disabling IDF-weighting in English evaluation. 

For \textbf{BERTScore-F1}, no language behaves consistently on all datasets. 

Besides, it can be observed that the performance drop is never out of the range of RD for English, whereas there are two values for each evaluation metric that is larger than the maximum performance improvement for English (MoverScore: WMT17 en-zh and en-tr; BERTScore: WMT17 en-de and WMT18 en-tr). Thus, those facts suggest that \emph{the effectiveness of IDF-weighting seems less stable in the evaluation of other languages compared with English}.





\paragraph{Punctuation Removal \& Subwords Selection}


First, we show the relative change from removing to keeping punctuations for each language on each dataset in Figure \ref{fig:punc sub all}. Despite of Turkish, fluctuation of RDs for all other languages is within the range of RDs for English. Furthermore, no language behaves consistently on all datasets except Czech; both negative and positive extrema can be observed even on one single language, namely Turkish. This kind of inconsistency has been previously observed on English. All of the facts mentioned suggest \emph{the similar effects of punctuation removal across different evaluation languages}. Next, we also examine the best configuration of subword selection and punctuation removal in combination for each language, as shown in Table \ref{tab:ditro}. \emph{In contrast to English, MoverScore-1 is more likely to get better results when not only using the first subword, no matter with or without punctuation removal}. Further, \emph{no configuration always performs best for a certain language on all datasets, which is in line with English evaluation}. In addition, it is noteworthy that \emph{MoverScore-1 never achieves the best results applying \emph{ave-all+PR} for all languages, including English}. 




%\subsubsection{Noisy Alignment Removal}
%\label{re:noisy}
%This section describes the evaluation results of noisy alignment removal (NAR). First, we show whether the WMD-based evaluation metrics benefit from NAR in both monolingual and cross-lingual evaluations in Table \ref{tab:noisy}, evaluated on WMT17 to-English pairs. First, \emph{noisy alignment removal does not lead to consistent improvement}. In fact, when only the average correlations are considered, only XMover-1+CLP benefits from NAR. In cross-lingual evaluations, the metric performances on ru-en can be consistently improved by NAR; in contrast, that on lv-en and zh-en never enhance with NAR. In monolingual evaluations, NAR is beneficial to MoverScore on fi-en and lv-en, no matter with or wihout IDF-weighting. Secondly, \emph{IDF-weighting still has positive impact when applying noisy alignment removal}. For all dropout rates, IDF-weighting impacts MoverScore positively. As described above, the performance enhancement with NAR can be seen on different language pairs in monolingual and cross-lingual evaluations. It may be caused by the difference in BERT and multilingual BERT. 






Hence, we also consider monolingual setup for other languages, with multilingual BERT. Figure \ref{fig:noisy 18 19} demonstrates the results on WMT18 and WMT19. As the figure shows, NAR leads to consistent performance improvement for all languages except Chinese and English. It is interesting that Chinese and English are distant languages but they behave similarly with NAR; In contrast, similar languages to English, like German, do not behave consistently with English. To my best knowledge, the only thing that English and Chinese have in common is they are high-resource languages in NLP. So we assume the difference in the effectiveness of NAR between these two languages and others is due to that multilingual BERT does not handle those languages well and consequently the non-optimal representations leading to more noisy alignments in WMD. To verify this, we evaluate NAR with language-specific BERT. Table \ref{tab: noisy language specific} shows the results for German and Turkish. It can be seen that NAR still has positive impact after applying language-specific models, just the improvement for Turkish falls a little. As a result, the previous assumpation can not be confirmed and the reason of the ineffectiveness of NAR on Chinese and English is unclear so far. 
















%Next, we study the effect of n-gram on noisy alignment removal. we test the n-gram from 1 to 3 and dropout rate from 0.1 to 0.5. Table \ref{tab:noisy-ngram} shows the results on WMT17 for both cross-lingual and monolingual evaluations. In monolingual evaluations, unigram MoverScore performs best for all dropout rates, suggesting \emph{a negative impact of n-gram in monolingual evaluations}. As for cross-lingual evaluations, the metric performance enhances with increasing n-gram before applying the LM on the target side for all dropout rates. However, it is interesting that an opposite result emerges after applying the LM: unigram XMoverScore performs best except for dropout rate 0.1, where bigram works slightly better than unigram. This suggests that n-gram works like a syntax model here; it plays a similar role to LM. However, the improvement from n-gram is tiny compared with LM.




%\subsubsection{Layer Selection \& Aggregation}
%\label{re:layer}
%This section presents the experiment results of Section \ref{layer set}. Table \ref{tab:mover layer}, \ref{tab:xmover layer} and \ref{tab:xmover LM layer} show the layer-wise experiment results for MoverScore-1, XMoverScore-1 and XMoverScore-1+LM, respectively.  
%First, the variations of metric performances with the changes of layer selection are much larger in cross-lingual evaluations; The CVs for MoverScore are within 1\% except on cs-en, whereas the CVs for XMoverScore range from 5.34\% to 24.69\%. After applying LM on the target side, the CV for XMoverScore decreases from 11.68\% to 3.65\% on average. Secondly, the RDs of the metric performances between using the best layer and power means show that the positive impact of power means decreases in cross-lingual evaluations; the RD in monolingual evaluation is -0.08\% on average while that in cross-lingual evaluations range from -18.57\% to 0.51\% and is -4.16\% in average. Similar to layer selection, the value drops after applying LM on the target side. The difference between monolingual and cross-lingual evaluations may due to the use of multilingual BERT. The results of previous experiments show that multilingual BERT or different evaluated languages can lead to changing effects of some factors, so the effects of layer selection and aggregation should be also studied in monolingual evaluations of other languages further. we leave this in future work.

==> structure/structure/8_discussion.tex <==
\subsection{Discussion}
\label{sec:conclusion}
%In this section, I 
We summarize the findings from the previous experiments along 4 dimensions.

%\begin{itemize}
%    \item 
\textbf{Evaluation Tasks}: 
    Among the considered NLG tasks, %in this work, namely segment-level and system-level MT and summary-level text summarization, 
    BERT-based evaluation metrics are more likely to generate inconsistent scores in segment-level MT evaluation. Their sensitivity %to %those factors 
    is less pronounced in system-level MT and summarization. %except the sensitivity of BERTScore-F1 to stopwords in summarization evaluation.
    In the latter two cases, average scores are considered, over the translations within one system or over the multiple references. %and consequently 
    Thus, some of the variation in metric scores %can compensate for each other, 
    will cancel out, leading to a less fluctuating metric performance from varying preprocessing schemes.
%    \item 
%\textbf{Correlations}: 
%    The three correlations in descending order regarding sensitivity are Kendall, Spearman, and Pearson, suggesting that it is more likely to obtain uncomparable scores across different papers if Kendall correlation is reported in those papers.
%    \item 
    \textbf{Evaluation metrics}:
    Among the two variants of MoverScore, %the scores generated 
    MoverScore-2 are more %likely to be affected by different settings of those factors. 
    sensitive to parameter settings. 
    BERTScore-F1 behaves less sensitively to IDF-weighting than MoverScore while it behaves much more sensitively to stopwords in the evaluation of Chinese and English compared with MoverScore-1. %XMoverScore is much more sensitive to different layer selection compared with its reference-based version MoverScore.
%   \item 
\textbf{Languages}: Overall, the considered evaluation metrics %behave differently in the evaluation of different languages. 
have different sensitivities %to preprocessing 
in different languages. 
%However, there is still something in common, such as the ranking of the magnitude of the effects of those factors, and the difference in sensitivity between evaluation levels. 
Furthermore, %it can be observed that the language pair involving 
highly inflectional languages such as Turkish and Russian as well as German often become ``outliers'' or obtain extrema in our experiments. %Chinese and English often stick together, such as in the experiments for stopwords removal and noisy alignment removal, although they are distance languages. These may due to the evaluation data or the languages themselves. 
%\item 
\textbf{Importance of factors}:
    Stopwords removal has the largest but mostly negative impact. %on those evaluation metrics. %among the tested factors. 
    IDF-weighting positively impacts  %\todo{YC: why IDF belongs to preprocessing?}%those 
    evaluation metrics in English evaluation but its contribution is much less stable in the evaluation of other languages. %\todo{SE: say something better about subword selection: which one is the best across languages?} 
    MoverScore benefits from subwords and punctuation removal in segment-level MT evaluation for English, but on other tasks or for other languages, no configuration of PR and subword selection consistently performs best.
    %It seems subword selection and punctuation removal just randomly impact the evaluation metrics on different tasks and there is no explicit clue about which is the best configuration of their combinations in different language environment. %Noisy alignment removal positively impacts MoverScore for all tested languages except Chinese and English. Layer selection has much larger impact on reference-free than on reference-based evaluation metrics. The effectiveness of power means also drops in cross-lingual evaluations. 

%\end{itemize}





==> structure/structure/9_conclusion.tex <==
\section{Conclusion}
We investigated reproducibility for BERT-based evaluation metrics, finding several problematic aspects, including using heavy undocumented preprocessing, reporting lower scores for competitors, selective evaluation on %`non-standard' 
datasets, and copying correlation scores from wrong indices. %Some of the 
%In the end, we can only speculate as to the reasons of the identified issues, e.g., %(i.e., reporting bad scores for competitors, omitting to evaluate on reference datasets from other papers, preprocessing) could be as
%whether they are forms of scientific misconduct \citep{carafoli2015scientific} or 
%whether they are genuine omissions and misunderstandings. % Our selection of metrics was not a random sample, however, and informed by popularity of techniques (BERTScore, MoverScore) as well as recency (BaryScore, SentSim), so it is unclear how well our results will gene
%Of course, the problem may also lie in the reviewing process, which may select inadequate reviewers 
 Our findings cast some doubts on previously reported results and findings, i.e., whether more the complex alignment schemes are really more effective than the greedy alignment of BERTScore. \se{In terms of preprocessing, we found that it can have a large effect depending (a.o.) on the languages and tasks involved. To better compare the effect of aggregation schemes on top of BERT, we recommend to minimize its role in the future, and employ uniform preprocessing across metrics.} 
 On the positive side, as authors are nowadays much more willing to publish their resources, it is considerably easier to spot such problems, which may also be one reason why critique papers such as ours have become more popular in the last few years \citep{Beese2022DetectingSI}. %\todo{SE: do our results generalize? is the peer review process adequate?}. 
 In a wider context, our paper contributes to addressing the ``cracked foundations'' of evaluation for text generation \citep{gehrmann2022repairing} and to better understanding their limitations \citep{Leiter2022TowardsEE}. %\todo{SE: maybe add a hint to future work: reproduce more metrics} 
 
 In the future, we would like to reproduce more recent BERT-based metrics (e.g., with other aggregation mechanisms \citep{chen-etal-2020-improving-text,Rony2022RoMeAR},  normalization schemes \citep{zhao-etal-2021-inducing} or different design choices \citep{yuan2021bartscore}) to obtain a broader assessment of reproducibility issues in this context. We would also like to quantify, at a larger scale, the bias in research induced from overestimating one's own model vis-\`a-vis competitor models. 

\iffalse
In this work, motivated by \citet{post2018call}, I studied reproducibility for BERT-based evaluation metrics, in order to examine whether they suffer from the same problem with BLEU of generating inconsistent and uncomparable scores across users. To do so, I first conducted a reproduction experiment for MoverScore and compared its evaluation script to BERTScore. I found that the authors of MoverScore applied much more preprocessing steps to achieve the results reported in the paper. All the reproduction attempts with my own evaluation scripts and datasets downloaded by myself failed, suggesting the importance of sharing code and data, which has been regarded as the main cause of non-reproducibility by many researchers. Then, I quantified the variation of metric performance regarding those factors, finding that the preprocessing technique, stopwords removal, has the largest impact among the tested factors. For a broader perspective, I compared the sensitivity across different evaluated languages in MT evaluations. This comparison shows that the impact of some factors can change with the changing evaluation languages. I confirmed the contribution of IDF-weighting in English evaluation and noisy alignment removal in the evaluation of all tested languages except Chinese and English.
In contrast, stopwords removal has a negative impact except in Turkish evaluation. Further, based on the results of a human evaluation replication, I found that the reproducibility of these two types of evaluation is about the same if there is insufficient reproduction resource obtained from the authors. Of course, this point can not be verified with such few observation samples, but it also helps reveal how inconsistent the metric scores can be with changing experimental setup. In this work, although I quantified the variation of metric performance regarding some factors and pointed out the inconsistency of their impacts across different evaluation languages, I did not get deeper insights into the causes, which should be studied in future work.
\fi 

==> structure/table.tex <==
\begin{table}[h]
\centering
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\multicolumn{1}{c}{} & cs-en & de-en & fi-en          & lv-en          & ru-en & tr-en & zh-en & average \\ \midrule
original             & 0.670 & 0.708 & \textbf{0.835} & \textbf{0.746} & 0.738 & 0.762 & 0.744 & 0.743   \\
reproduced           & 0.670 & 0.708 & \textbf{0.821} & \textbf{0.717} & 0.738 & 0.762 & 0.744 & 0.737   \\ \bottomrule
\end{tabular}%
}
\caption{\emph{Reproduction}: Original and reproduced segment-level Pearson correlations of MoverScore-1 on WMT17. Original results are citet from \citet{zhao2019moverscore}. Bold values refer to unreproducible results.}
\label{tab:reproduction wmt17}

\vspace{15pt}

\centering
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
dataset                & \multicolumn{3}{c}{BAGEL} & \multicolumn{3}{c}{SFHOTEL} \\
criteria               & Inf     & Nat    & Qual   & Inf     & Nat     & Qual    \\ \midrule
original               & 0.285   & 0.195  & 0.158  & 0.207   & 0.270   & 0.183   \\
reproduced             & 0.244   & 0.145  & 0.092  & \textbf{0.223}   & 0.167   & 0.065   \\
reproduced (stopwords) & 0.230   & 0.135  & 0.078  & \textbf{0.208}   & 0.145   & 0.042   \\ \bottomrule
\end{tabular}%
}
\caption{\emph{Reproduction}: Original and reproduced utterance-level Spearman correlations of MoverScore-1 on BAGEL and SFHOTEL datasets. Original results are citet from \citet{zhao2019moverscore}. Bold values refer to the reproduced resutls that are better than the original.}
\label{tab:dtt reproduction}

\vspace{15pt}

\centering
\resizebox{0.7\columnwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
metric                      & \multicolumn{2}{c}{MoverScore-1} & \multicolumn{2}{c}{BERTScore-R} \\
criteria                    & M1              & M2             & M1             & M2             \\ \midrule
original                    & 0.813           & 0.810          & 0.834          & 0.783          \\
reproduced (mean)           & 0.687            & 0.674           & -              & -              \\
reproduced  (max)           & 0.690           & 0.714          & \textbf{0.851}          & \textbf{0.793}          \\
reproduced (mean+stopwords) & 0.707           & 0.709          & -              & -              \\
reproduced (max+stopwords)  & 0.686           & 0.718          & -              & -              \\ \bottomrule
\end{tabular}%
}
\caption{\emph{Reproduction}: Original and reproduced system-level Pearson correlations of MoverScore-1 and BERTScore-R on MSCOCO dataset. Original results are citet from \citet{zhao2019moverscore} and \citet{zhang2019bertscore}. Bold values refer to the reproduced resutls that are better than the original.}
\label{tab:coco reproduction}


\end{table}


\begin{table}[H]
\renewcommand{\arraystretch}{1.4}
\centering
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
                                       & Factor              & MoverScore & BERTScore \\ \hline
\multirow{3}{*}{Preprocessing-related} & subwords removal    & \Checkmark          & \XSolidBrush         \\ \cline{2-4} 
                                       & stopwords removal   & \Checkmark          & \XSolidBrush         \\ \cline{2-4} 
                                       & punctuation removal & \Checkmark         & \XSolidBrush         \\ \hline
\multirow{2}{*}{Other}                 & layer selection     & \XSolidBrush         & \Checkmark         \\ \cline{2-4} 
                                       & IDF-weighting       & \Checkmark          & \Checkmark         \\ \hline
\end{tabular}%
}
\caption{Factors considered in this work. \Checkmark/\XSolidBrush denotes whether the evaluation metric has the parameter associated with the factor.}
\label{tab:fac}
\end{table}


\begin{table}[H]
\centering
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{@{}lcccc|cccc@{}}
\toprule
\multicolumn{5}{c|}{\textbf{Segment-level}} & \multicolumn{4}{c}{\textbf{System-level}} \\
Metric & WMT17-$r$ & WMT18-$\tau$ & WMT19-$\tau$ & AVG & WMT17-$r$ & WMT18-$r$ & WMT19-$r$ & AVG \\ \midrule
Mover-1 & 2.18\% & 2.00\% & 1.42\% & 1.87\% & 0.44\% & 0.20\% & 0.12\% & 0.25\% \\
Mover-2 & 2.09\% & 2.04\% & 1.99\% & 2.04\% & 0.14\% & 0.16\% & 0.20\% & 0.17\% \\
BERT-F1 & 8.74\% & 8.18\% & 6.24\% & 7.72\% & 0.16\% & 0.48\% & 0.25\% & 0.30\% \\ \bottomrule
\end{tabular}%
}

\caption{\emph{Sensitivity to Stopwords}: Average coefficients of variation 
%per dataset and evaluation metric
%and over WMT17-19 datasets 
%of the correlations 
on WMT17-19 to-English language pairs.}
\label{tab:sw wmt all}
\end{table}


\begin{table}[hp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccc|cccc@{}}
\toprule
        & \multicolumn{4}{c|}{\textbf{Segment-level}}      & \multicolumn{4}{c}{\textbf{System-level}}  \\
Metric  & WMT17-$r$ & WMT18-$\tau$ & WMT19-$\tau$ & AVG    & WMT17-$r$ & WMT18-$r$ & WMT19-$r$ & AVG    \\ \midrule
Mover-1 & 0.13\%    & 0.67\%       & 2.56\%       & 1.12\% & 0.05\%    & 0.06\%    & 0.21\%    & 0.11\% \\
Mover-2 & 0.78\%    & 1.19\%       & 3.84\%       & 1.94\% & 0.25\%    & 0.17\%    & 0.49\%    & 0.30\% \\
BERT-F1 & 0.20\%    & 0.32\%       & 0.41\%       & 0.31\% & 0.05\%    & 0.02\%    & 0.08\%    & 0.05\% \\ \bottomrule
\end{tabular}%
}
\caption{\emph{Sensitivity to IDF-weighting}: Average coefficients of variation on WMT17-19 (CV(ori+random)).}
\label{tab:wmt idf cv}

\vspace{15pt}

\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccc|cccccc@{}}
\toprule
 & \multicolumn{6}{c|}{\textbf{Pyramid}} & \multicolumn{6}{c}{\textbf{Responsiveness}} \\
 & \multicolumn{3}{c}{{\ul TAC2008}} & \multicolumn{3}{c|}{{\ul TAC2009}} & \multicolumn{3}{c}{{\ul TAC2008}} & \multicolumn{3}{c}{{\ul TAC2009}} \\
Metric & $r$ & $\rho$ & $\tau$ & $r$ & $\rho$ & $\tau$ & $r$ & $\rho$ & $\tau$ & $r$ & $\rho$ & $\tau$ \\ \midrule
Mover-1 & 0.11\% & 0.15\% & \multicolumn{1}{c|}{0.40\%} & 0.08\% & 0.04\% & 0.43\% & 0.13\% & 0.27\% & \multicolumn{1}{c|}{0.31\%} & 0.14\% & 0.33\% & 0.37\% \\
Mover-2 & 0.13\% & 0.23\% & \multicolumn{1}{c|}{0.27\%} & 0.11\% & 0.31\% & 0.35\% & 0.19\% & 0.37\% & \multicolumn{1}{c|}{0.39\%} & 0.13\% & 0.42\% & 0.46\% \\
BERT-F1 & 0.19\% & 0.42\% & \multicolumn{1}{c|}{0.51\%} & 0.06\% & 0.24\% & 0.34\% & 0.21\% & 0.32\% & \multicolumn{1}{c|}{0.31\%} & 0.17\% & 0.21\% & 0.19\% \\ \bottomrule
\end{tabular}%
}
\caption{\emph{Sensitivity to IDF-weighting}: Coefficients of variation of correlations on TAC2008-2009 (CV(ori+random)).}
\label{tab:tac idf cv}

\end{table}



\begin{table}[H]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{@{}lcc@{}}
\toprule
Corpora & WMT18-AVG & WMT19-AVG \\
ORI & \textbf{0.355} & \textbf{0.333} \\ \midrule
Wili\_2008(117500) & 0.349 & 0.323 \\
Wikipedia(100000) & 0.350 & 0.320 \\
Wikipedia(1000000) & 0.351 & 0.320 \\
Wikipedia(2500000) & 0.351 & 0.320 \\
Wikipedia(5000000) & 0.350 & 0.320 \\
Wikipedia(7500000) & 0.351 & 0.320 \\
Wikipedia(10000000) & 0.351 & 0.320 \\
IMDB\_train(25000) & 0.347 & 0.323 \\
Wikitext(23767) & 0.350 & 0.324 \\
Wiki40b(2926536) & 0.347 & 0.324 \\ \bottomrule
\end{tabular}%
}
\caption{\emph{External IDF-weighting}: Average segment-level Kendall correlation of MoverScore-1 on WMT18-19 to-English language pairs. Bold values refer to best results. Number in bracket represents the number of documents in this corpora.}
\label{tab:external en}
\end{table}


\begin{table}[H]
\centering
\resizebox{0.5\textwidth}{!}{%
\begin{tabular}{@{}cccc|ccc@{}}
\toprule
metric  & \multicolumn{3}{c|}{BERTScore-F1} & \multicolumn{3}{c}{MoverScore-1} \\
dataset & WMT17     & WMT18     & WMT19     & WMT17     & WMT18     & WMT19    \\ \midrule
en      & 0         & 0         & 0         & 0         & 0         & 0        \\
zh      & 0         & 0         & 0         & 0         & 0         & 0        \\
de      & 0         & 0         & 0         & 0         & 0         & 0        \\
ru      & 0         & 0         & 0         & 0         & 0         & 0        \\
fi      & 0         & 0         & 0         & 0         & 0         & 229      \\
cs      & 0         & 0         & -         & 0         & 0         & -        \\
tr      & 504       & 551       & -         & 504       & 551       & -        \\ \bottomrule
\end{tabular}%
}
\caption{\emph{Comparison among Evaluated Languages}: Distribution of the best stopword settings for all tested languages on segment-level MT evaluation.}
\label{tab:sw distribution}
\end{table}


\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|cccccc|cccccc|cccc|}
\hline
\multicolumn{1}{|c|}{} & \multicolumn{6}{c|}{WMT17} & \multicolumn{6}{c|}{WMT18} & \multicolumn{4}{c|}{WMT19} \\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{de} & \multicolumn{1}{c|}{zh} & \multicolumn{1}{c|}{ru} & \multicolumn{1}{c|}{fi} & \multicolumn{1}{c|}{tr} & cs & \multicolumn{1}{c|}{de} & \multicolumn{1}{c|}{zh} & \multicolumn{1}{c|}{ru} & \multicolumn{1}{c|}{fi} & \multicolumn{1}{c|}{tr} & cs & \multicolumn{1}{c|}{de} & \multicolumn{1}{c|}{zh} & \multicolumn{1}{c|}{ru} & fi \\ \hline
first & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{\Checkmark} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\ \hline
all & \multicolumn{1}{c|}{{\ul }} & \multicolumn{1}{c|}{\Checkmark} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\Checkmark} & \multicolumn{1}{c|}{\Checkmark} & \Checkmark & \multicolumn{1}{c|}{{\ul }} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\Checkmark} & \multicolumn{1}{c|}{{\ul }} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\ \hline
ave-all & \multicolumn{1}{c|}{\Checkmark} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\Checkmark} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\Checkmark} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \Checkmark \\ \hline
first+PR* & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\Checkmark} & \multicolumn{1}{c|}{\Checkmark} &  \\ \hline
all+PR & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\Checkmark} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\Checkmark} & \Checkmark & \multicolumn{1}{c|}{\Checkmark} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\ \hline
ave-all+PR & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} &  \\ \hline
\end{tabular}%
}
\caption{\emph{Comparison among Evaluated Languages}: Distribution of the best subword and punctuation settings for tested languages.}
\label{tab:ditro}
\end{table}


\begin{table}[h]
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{@{}lccccccccc@{}}
\toprule
Metric & dropout rate & cs-en & de-en & fi-en & lv-en & ru-en & tr-en & zh-en & AVG \\ \midrule
\multicolumn{10}{c}{Cross-lingual evaluation} \\ \midrule
XMover-1 & 0 & 0.2580 & 0.3552 & \textbf{0.3973} & \textbf{0.3082} & 0.2557 & \textbf{0.4156} & \textbf{0.4728} & \textbf{0.3518} \\
 & 0.1 & 0.2826 & 0.3600 & 0.3913 & 0.2290 & 0.2818 & 0.3934 & 0.4209 & 0.3370 \\
 & 0.2 & \textbf{0.2831} & 0.3619 & 0.3913 & 0.2290 & 0.2813 & 0.3935 & 0.4213 & 0.3373 \\
 & 0.3 & 0.2823 & 0.3617 & 0.3913 & 0.2276 & \textbf{0.2819} & 0.3937 & 0.4211 & 0.3371 \\
 & 0.4 & 0.2829 & \textbf{0.3619} & 0.3912 & 0.2277 & 0.2817 & 0.3935 & 0.4201 & 0.3370 \\
 & 0.5 & 0.2831 & 0.3602 & 0.3912 & 0.2290 & 0.2814 & 0.3937 & 0.4187 & 0.3367 \\ \midrule
XMover-1+CLP & 0 & 0.3200 & 0.3673 & 0.4675 & \textbf{0.4436} & 0.2932 & 0.5029 & \textbf{0.4918} & 0.4123 \\
 & 0.1 & \textbf{0.3639} & 0.3845 & \textbf{0.5394} & 0.4369 & 0.3146 & \textbf{0.5202} & 0.4266 & \textbf{0.4266} \\
 & 0.2 & 0.3620 & \textbf{0.3865} & 0.5383 & 0.4359 & \textbf{0.3152} & 0.5197 & 0.4275 & 0.4264 \\
 & 0.3 & 0.3630 & 0.3832 & 0.5383 & 0.4370 & 0.3142 & 0.5197 & 0.4274 & 0.4261 \\
 & 0.4 & 0.3632 & 0.3826 & 0.5393 & 0.4342 & 0.3143 & 0.5197 & 0.4280 & 0.4259 \\
 & 0.5 & 0.3633 & 0.3851 & 0.5393 & 0.4331 & 0.3150 & 0.5197 & 0.4264 & 0.4260 \\ \midrule
XMover-1+CLP+LM & 0 & \textbf{0.5059} & \textbf{0.4878} & 0.6578 & \textbf{0.6708} & 0.5076 & \textbf{0.5910} & \textbf{0.5822} & \textbf{0.5719} \\
 & 0.1 & 0.5023 & 0.4867 & 0.6609 & 0.6290 & \textbf{0.5096} & 0.5484 & 0.5416 & 0.5541 \\
 & 0.2 & 0.5009 & 0.4875 & 0.6605 & 0.6290 & 0.5093 & 0.5477 & 0.5428 & 0.5540 \\
 & 0.3 & 0.5017 & 0.4854 & 0.6605 & 0.6290 & 0.5089 & 0.5477 & 0.5411 & 0.5535 \\
 & 0.4 & 0.5011 & 0.4847 & 0.6609 & 0.6277 & 0.5089 & 0.5481 & 0.5421 & 0.5534 \\
 & 0.5 & 0.5013 & 0.4863 & \textbf{0.6610} & 0.6276 & 0.5092 & 0.5476 & 0.5410 & 0.5534 \\ \midrule
\multicolumn{10}{c}{Monolingual evaluation} \\ \midrule
Mover-1 & 0 & \textbf{0.6487} & \textbf{0.6765} & 0.8101 & 0.6994 & \textbf{0.7177} & 0.7581 & \textbf{0.7363} & \textbf{0.7210} \\
 & 0.1 & 0.6430 & 0.6600 & \textbf{0.8150} & 0.7100 & 0.6930 & \textbf{0.7630} & 0.7180 & 0.7146 \\
 & 0.2 & 0.6440 & 0.6660 & 0.8130 & \textbf{0.7120} & 0.6940 & 0.7580 & 0.7190 & 0.7151 \\
 & 0.3 & 0.6430 & 0.6710 & 0.8060 & 0.7030 & 0.6870 & 0.7570 & 0.7110 & 0.7111 \\
 & 0.4 & 0.6420 & 0.6720 & 0.7990 & 0.6820 & 0.6820 & 0.7550 & 0.6950 & 0.7039 \\
 & 0.5 & 0.6220 & 0.6130 & 0.7580 & 0.6340 & 0.6440 & 0.7060 & 0.6520 & 0.6613 \\ \midrule
Mover-1 (idf) & 0 & \textbf{0.6698} & \textbf{0.7083} & 0.8214 & 0.7174 & \textbf{0.7379} & \textbf{0.7618} & \textbf{0.7442} & \textbf{0.7373} \\
 & 0.1 & 0.6585 & 0.6733 & 0.8222 & 0.7212 & 0.7043 & 0.7559 & 0.7197 & 0.7222 \\
 & 0.2 & 0.6566 & 0.6715 & \textbf{0.8229} & 0.7234 & 0.7088 & 0.7538 & 0.7217 & 0.7227 \\
 & 0.3 & 0.6576 & 0.6710 & 0.8197 & 0.7269 & 0.7073 & 0.7506 & 0.7206 & 0.7220 \\
 & 0.4 & 0.6562 & 0.6697 & 0.8128 & 0.7293 & 0.7052 & 0.7468 & 0.7169 & 0.7196 \\
 & 0.5 & 0.6516 & 0.6668 & 0.8007 & \textbf{0.7294} & 0.7012 & 0.7347 & 0.7090 & 0.7134 \\ \bottomrule
\end{tabular}%
}
\caption{\emph{Noisy Alignment Rermoval}: Pearson correlations of XMoverScore and MoverScore with segment-level human judgements on WMT17 to-English language pairs. Dropout rate 0 denotes disabling noisy alignment removal. Bold values refer to the best result of each evaluation metric.}
\label{tab:noisy}
\end{table}


\begin{table}[h]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{@{}clccc@{}}
\toprule
language & \multicolumn{1}{c}{model} & ORI & NAR(dropout\_rate=0.1) & absolute improvement \\ \midrule
\multirow{2}{*}{Turkish} & MBERT & 0.327 & 0.374 & +0.047 \\
 & Turkish BERT\tablefootnote{\url{https://huggingface.co/dbmdz/bert-base-turkish-cased}} & 0.426 & 0.461 & +0.035 \\ \midrule
\multirow{2}{*}{German} & MBERT & 0.692 & 0.697 & +0.005 \\
 & German BERT\tablefootnote{\url{https://huggingface.co/dbmdz/bert-base-german-uncased}} & 0.720 & 0.726 & +0.006 \\ \bottomrule
\end{tabular}%
}
\caption{\emph{Noisy Alignment Rermoval}: Kendall's $\tau$ of MoverScore-1 applying language-specific BERT with segment-level human judgements on WMT18.}
\label{tab: noisy language specific}
\end{table}


\begin{table}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}c|lclclc|lc@{}}
\toprule
\multirow{2}{*}{dropout\_rate} &
  metric &
  \multicolumn{1}{c|}{r} &
  metric &
  \multicolumn{1}{c|}{r} &
  metric &
  r &
  metric &
  r \\ \cmidrule(l){2-9} 
 &
  \multicolumn{6}{c|}{Cross-lingual evaluation} &
  \multicolumn{2}{c}{Monolingual evaluation} \\ \midrule
\multirow{3}{*}{0.1} &
  XMover-1 &
  \multicolumn{1}{c|}{0.3370} &
  XMover-1+CLP &
  \multicolumn{1}{c|}{0.4256} &
  XMover-1+CLP+LM &
  0.5536 &
  Mover-1 &
  \textbf{0.7146} \\
 &
  XMover-2 &
  \multicolumn{1}{c|}{0.3531} &
  XMover-2+CLP &
  \multicolumn{1}{c|}{0.4344} &
  XMover-2+CLP+LM &
  \textbf{0.5539} &
  Mover-2 &
  0.7096 \\
 &
  XMover-3 &
  \multicolumn{1}{c|}{\textbf{0.3546}} &
  XMover-3+CLP &
  \multicolumn{1}{c|}{\textbf{0.4344}} &
  XMover-3+CLP+LM &
  0.5513 &
  Mover-3 &
  0.7119 \\ \midrule
\multirow{3}{*}{0.2} &
  XMover-1 &
  \multicolumn{1}{c|}{0.3366} &
  XMover-1+CLP &
  \multicolumn{1}{c|}{0.4260} &
  XMover-1+CLP+LM &
  \textbf{0.5539} &
  Mover-1 &
  \textbf{0.7151} \\
 &
  XMover-2 &
  \multicolumn{1}{c|}{0.3536} &
  XMover-2+CLP &
  \multicolumn{1}{c|}{0.4340} &
  XMover-2+CLP+LM &
  0.5536 &
  Mover-2 &
  0.7074 \\
 &
  XMover-3 &
  \multicolumn{1}{c|}{\textbf{0.3537}} &
  XMover-3+CLP &
  \multicolumn{1}{c|}{\textbf{0.4347}} &
  XMover-3+CLP+LM &
  0.5514 &
  Mover-3 &
  0.711 \\ \midrule
\multirow{3}{*}{0.3} &
  XMover-1 &
  \multicolumn{1}{c|}{0.3367} &
  XMover-1+CLP &
  \multicolumn{1}{c|}{0.4264} &
  XMover-1+CLP+LM &
  \textbf{0.5541} &
  Mover-1 &
  \textbf{0.7111} \\
 &
  XMover-2 &
  \multicolumn{1}{c|}{0.3533} &
  XMover-2+CLP &
  \multicolumn{1}{c|}{0.4341} &
  XMover-2+CLP+LM &
  0.5536 &
  Mover-2 &
  0.705 \\
 &
  XMover-3 &
  \multicolumn{1}{c|}{\textbf{0.3540}} &
  XMover-3+CLP &
  \multicolumn{1}{c|}{\textbf{0.4347}} &
  XMover-3+CLP+LM &
  0.5516 &
  Mover-3 &
  0.7071 \\ \midrule
\multirow{3}{*}{0.4} &
  XMover-1 &
  \multicolumn{1}{c|}{0.3369} &
  XMover-1+CLP &
  \multicolumn{1}{c|}{0.4259} &
  XMover-1+CLP+LM &
  \textbf{0.5537} &
  Mover-1 &
  \textbf{0.7039} \\
 &
  XMover-2 &
  \multicolumn{1}{c|}{0.3533} &
  XMover-2+CLP &
  \multicolumn{1}{c|}{0.4339} &
  XMover-2+CLP+LM &
  0.5536 &
  Mover-2 &
  0.6947 \\
 &
  XMover-3 &
  \multicolumn{1}{c|}{\textbf{0.3541}} &
  XMover-3+CLP &
  \multicolumn{1}{c|}{\textbf{0.4344}} &
  XMover-3+CLP+LM &
  0.5511 &
  Mover-3 &
  0.6929 \\ \midrule
\multirow{3}{*}{0.5} &
  XMover-1 &
  \multicolumn{1}{c|}{0.3366} &
  XMover-1+CLP &
  \multicolumn{1}{c|}{0.4261} &
  XMover-1+CLP+LM &
  \textbf{0.5536} &
  Mover-1 &
  \textbf{0.6613} \\
 &
  XMover-2 &
  \multicolumn{1}{c|}{0.3533} &
  XMover-2+CLP &
  \multicolumn{1}{c|}{0.4333} &
  XMover-2+CLP+LM &
  0.5531 &
  Mover-2 &
  0.6554 \\
 &
  XMover-3 &
  \multicolumn{1}{c|}{\textbf{0.3543}} &
  XMover-3+CLP &
  \multicolumn{1}{c|}{\textbf{0.4350}} &
  XMover-3+CLP+LM &
  0.5513 &
  Mover-3 &
  0.6514 \\ \bottomrule
\end{tabular}%
}
\caption{\emph{Noisy Alignment Rermoval}: Pearson correlation of MoverScore and XMoverScore with segment-level human judgements on WMT17. Bold values are the best resutls applying the same dropout rate but with different n-grams.}
\label{tab:noisy-ngram}
\end{table}


\begin{table}[H]
\centering
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{@{}ccccccccc@{}}
\toprule
layer & cs-en & de-en & fi-en & lv-en & ru-en & tr-en & zh-en & AVG \\ \midrule
8 & 0.6361 & 0.6755 & 0.8134 & 0.7033 & 0.7273 & 0.7233 & 0.7175 & 0.7138 \\
9 & 0.6510 & 0.6865 & \textbf{0.8240} & 0.7107 & \textbf{0.7291} & \textbf{0.7357} & \textbf{0.7195} & 0.7224 \\
10 & 0.6605 & \textbf{0.6948} & 0.8231 & 0.7158 & 0.7363 & 0.7317 & 0.7168 & \textbf{0.7256} \\
11 & \textbf{0.6695} & 0.6845 & 0.8192 & 0.7048 & 0.7315 & 0.7276 & 0.7058 & 0.7204 \\
12 & 0.6677 & 0.6825 & 0.8194 & \textbf{0.7188} & 0.7326 & 0.7291 & 0.7064 & 0.7224 \\ \midrule
pmeans & 0.6623 & 0.6873 & 0.8234 & 0.7139 & 0.7350 & 0.7339 & 0.7192 & 0.7250 \\ \midrule
CV & 1.87\% & 0.91\% & 0.46\% & 0.85\% & 0.42\% & 0.57\% & 0.82\% & 0.54\% \\
RD(pmeans-best) & -1.08\% & -1.08\% & -0.07\% & -0.68\% & -0.18\% & -0.24\% & -0.04\% & -0.08\% \\ \bottomrule
\end{tabular}%
}
\caption{\emph{Sensitivity to Layer Selection \& Aggregation}: Pearson correlations of MoverScore-1 with segment-level human judgments on WMT17. The results are taken from \citet{zhao2019moverscore}. Bold values refer to the best results using embedding from single layer.}
\label{tab:mover layer}

\vspace{15pt}

\centering
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{@{}crrrrrrrr@{}}
\toprule
layer & \multicolumn{1}{c}{cs-en} & \multicolumn{1}{c}{de-en} & \multicolumn{1}{c}{fi-en} & \multicolumn{1}{c}{lv-en} & \multicolumn{1}{c}{ru-en} & \multicolumn{1}{c}{tr-en} & \multicolumn{1}{c}{zh-en} & \multicolumn{1}{c}{AVG} \\ \midrule
8 & 0.2579 & 0.3549 & 0.3977 & \textbf{0.3082} & 0.2559 & 0.4157 & \textbf{0.4728} & 0.3519 \\
9 & 0.2835 & 0.3555 & \textbf{0.4231} & 0.2859 & 0.2581 & \textbf{0.4239} & 0.4557 & \textbf{0.3551} \\
10 & 0.2533 & 0.3469 & 0.3926 & 0.2335 & 0.2231 & 0.4008 & 0.4283 & 0.3255 \\
11 & 0.1825 & 0.3269 & 0.2687 & 0.1381 & 0.1525 & 0.3317 & 0.3563 & 0.2509 \\
12 & 0.2058 & 0.3856 & 0.3002 & 0.2269 & \textbf{0.3251} & 0.3772 & 0.4568 & 0.3254 \\ \midrule
pmeans & 0.2357 & 0.3781 & 0.3523 & 0.2509 & 0.2763 & 0.4136 & 0.4752 & 0.3403 \\ \midrule
CV & 15.58\% & 5.34\% & 16.98\% & 24.69\% & 23.08\% & 8.49\% & 9.54\% & 11.68\% \\
RD(pmeans-best) & -16.86\% & -1.95\% & -16.72\% & -18.57\% & -15.01\% & -2.41\% & 0.51\% & -4.16\% \\ \bottomrule
\end{tabular}%
}
\caption{\emph{Sensitivity to Layer Selection \& Aggregation}: Pearson correlations of XMoverScore-1 with segment-level human judgments on WMT17. Bold values refer to the best results using embedding from single layer.}
\label{tab:xmover layer}

\vspace{15pt}

\centering
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{@{}crrrrrrrr@{}}
\toprule
layer & \multicolumn{1}{c}{cs-en} & \multicolumn{1}{c}{de-en} & \multicolumn{1}{c}{fi-en} & \multicolumn{1}{c}{lv-en} & \multicolumn{1}{c}{ru-en} & \multicolumn{1}{c}{tr-en} & \multicolumn{1}{c}{zh-en} & \multicolumn{1}{c}{AVG} \\ \midrule
8 & 0.4841 & \textbf{0.4901} & 0.6496 & \textbf{0.6447} & 0.4897 & \textbf{0.5731} & \textbf{0.5715} & 0.5575 \\
9 & 0.5073 & 0.4882 & \textbf{0.6593} & 0.6390 & \textbf{0.5004} & 0.5639 & 0.5579 & \textbf{0.5594} \\
10 & \textbf{0.5007} & 0.4867 & 0.6517 & 0.6169 & 0.4928 & 0.5469 & 0.5397 & 0.5479 \\
11 & 0.4806 & 0.4897 & 0.6279 & 0.6024 & 0.4702 & 0.5247 & 0.5115 & 0.5296 \\
12 & 0.4065 & 0.4819 & 0.5852 & 0.5568 & 0.4762 & 0.5179 & 0.5249 & 0.5071 \\ \midrule
pmeans & 0.4820 & 0.4947 & 0.6443 & 0.6336 & 0.4973 & 0.5556 & 0.5425 & 0.5500 \\ \midrule
CV & 7.58\% & 0.60\% & 4.24\% & 5.15\% & 2.28\% & 3.93\% & 4.00\% & 3.65\% \\
RD(pmeans-best) & -4.99\% & 0.94\% & -2.29\% & -1.73\% & -0.62\% & -3.04\% & -5.09\% & -1.69\% \\ \bottomrule
\end{tabular}%
}
\caption{\emph{Sensitivity to Layer Selection \& Aggregation}: Pearson correlations of XMoverScore-1+LM with segment-level human judgments on WMT17. Bold values refer to the best results using embedding from single layer.}
\label{tab:xmover LM layer}


\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[h]
\centering
%\resizebox{\textwidth}{!}
{\small %
\begin{tabular}{@{}c|lllll|llllll@{}}
\toprule
 &
  \multicolumn{5}{c|}{WMT15} &
  \multicolumn{6}{c}{WMT16} \\
 &
  metric &
  cs-en &
  de-en &
  fi-en &
  ru-en &
  cs-en &
  de-en &
  ru-en &
  fi-en &
  ro-en &
  tr-en \\ \midrule
\multirow{5}{*}{Reproduced} &
  BERT-F &
  75.0 &
  73.3 &
  75.2 &
  \textbf{74.5} &
  \textbf{74.7} &
  64.0 &
  67.2 &
  66.1 &
  \textbf{72.3} &
  68.8 \\
 &
  Mover-1 &
  73.4 &
  73.1 &
  74.3 &
  73.1 &
  74.0 &
  63.3 &
  \textbf{67.6} &
  65.5 &
  71.4 &
  69.3 \\
 &
  Bary-W &
  \textbf{75.1} &
  \textbf{73.7} &
  \textbf{77.1} &
  73.3 &
  73.1 &
  \textbf{67.3} &
  66.0 &
  \textbf{66.8} &
  71.5 &
  \textbf{70.1} \\
 &
  Mover-1$^{+}$ &
  74.5 &
  75.5 &
  77.4 &
  76.5* &
  76.5* &
  67.6 &
  69.5* &
  70.7* &
  74.2* &
  73.6 \\
 &
  Bary-W$^{+}$ &
  75.6* &
  75.6* &
  78.6* &
  76.2 &
  75.7 &
  69.9* &
  67.7 &
  70.0 &
  73.1 &
  74.9* \\ \midrule
\multirow{5}{*}{Reported} &
  BERT-F &
  \textbf{74.3} &
  72.2 &
  74.7 &
  \textbf{74.0} &
  74.1 &
  \textbf{65.3} &
  65.1 &
  65.4 &
  70.2 &
  \textbf{70.7} \\
 &
  Mover &
  68.8 &
  71.8 &
  70.0 &
  68.6 &
  67.4 &
  60.9 &
  64.4 &
  63.1 &
  64.2 &
  66.1 \\
 
 &
  Bary &
  74.2 &
  \textbf{74.1} &
  \textbf{76.6} &
  73.7 &
  \textbf{74.2} &
  64.6 &
  \textbf{67.5} &
  \textbf{67.1} &
  \textbf{72.5} &
  69.3 \\
  &
  Mover$^{+}$ &
  71.0 &
  71.1 &
  72.2 &
  67.3 &
  70.7 &
  62.4 &
  64.0 &
  64.5 &
  66.4 &
  66.3 \\
  
 & Bary$^{+}$ & 75.9* & 75.8* & 79.9* & 77.6* & 76.6* & 68.5* & 69.4* & 70.2* & 74.3* & 73.8* \\ \bottomrule
\end{tabular}%
}
\caption{Reproduction: Segment-level Pearson's r (\%) on WMT15-16 to English language pairs using evaluation script provided by \citet{colombo2021automatic}. Reported values are cited from \citet{colombo2021automatic}. $^{+}$ refers to using the finetuned bert-based-uncased model on MNLI. Bold values refer to the best results with bert-base-uncased model. Values with * denote the best reproduced/reported results.}
\label{tab: reproduction wmt1516}
\end{table*}

